Pessimism of the Will, Optimism of the Intellect: Fair Protocols with Malicious but Rational Agents

Fairness is a desirable and crucial property of many protocols that handle, for instance, exchanges of message. It states that if at least one agent engaging in the protocol is honest, then either the protocol will unfold correctly and fulfill its intended goal for all participants, or it will fail for everyone. In this work, we present a game-based framework for the study of fairness protocols, that does not define a priori an attacker model. It is based on the notion of strong secure equilibria, and leverages the conceptual and algorithmic toolbox of game theory. In the case of finite games, we provide decision procedures with tight complexity bounds for determining whether a protocol is immune to nefarious attacks from a coalition of participants, and whether such a protocol could exist based on the underlying graph structure and objectives.

==> agentsnaturev1.tex <==
\subsection{A neutral natural environment}

There is however a case where this notion of finite memory does not make sense: when the agents represent \emph{natural} entities that cannot really be malicious although they may help malicious untrusted agents in their endeavors.
An example of such ``agents'' would be an unreliable communication channel.
These nature agents can be modeled as untrusted agents with no individual goal and a wronging condition that represent the assumptions made over them.
For example an unreliable channel may delay a message for any arbitrary duration but not lose it completely.
This condition can be modeled by an LTL formula of the form $\neg\left(\globally \text{received} \Rightarrow \eventually \text{transmitted}\right)$.
We can remark that this condition can be fulfilled or not based entirely on the choice of the channel agent.
But although there are a variety of ways to construct a Mealy machine that would always satisfy this goal (say wait at most $t$ steps before transmitting the message), this cannot cover the full possibility of the plausible and correct behaviors of such agents.

One solution to this is to model nature agents specifically to capture this kind of behaviors.
Namely, nature agents:
\begin{itemize}
    \item Do not have an individual objective.
    \item Instead of a wronging condition, they have a \emph{sanity} condition\footnote{A sanity condition can be seen as the negation of the wronging condition: a nature agent is wronged if it behaves in an insane manner.}.
    \item Can always enforce their sanity condition.
\end{itemize}
In return, a protocol should not actually specify the behaviors of nature agents.
It should allow for the collective goal to be fulfilled and prevent attacks provided no nature agents behave insanely.


Definitions of protocols and what constitutes a valid protocol have to be slightly adapted to take into account the special role of nature agents.
Formally:
\Ms{Copied from version2; new names should be given\dots ``Protocol Problem in Nature''?}
\begin{defi}[Protocol challenge]\label{def:protocolProblem}
    A \emph{protocol challenge} is a tuple:
    \[\pc = \left(\Traces, \tr, \untrusted, (\behaviors_{u})_{u \in \untrusted}, (\Ind_u)_{u \in \untrusted}, (\Wrong_u)_{u \in \untrusted}, \trusted, (\behaviors_{t})_{t \in \trusted}, \nature, (\behaviors_{n})_{n \in \nature}, (\Sane_n)_{n \in \nature}, \Coll\right),\] where:

    \begin{itemize}
    \item there are three types of \emph{agents}:
    \begin{itemize}
        \item the \emph{untrusted agents} are the elements of the set $\untrusted$,

        \item the \emph{trusted agents} are the elements of the set $\trusted$,

        \item the \emph{nature agents} are the elements of the set $\nature$,
    \end{itemize}
    and we write $\agents = \untrusted \cup \trusted \cup \nature$;

    \item each agent $a$ has a set $\behaviors_a$ of available \emph{behaviors} (and for $A \subseteq \agents$, we write $\behaviors_A = \prod_{a \in A} \behaviors_a$);

    \item the set $\Traces$ is the set of \emph{traces}, and the \emph{trace mapping} $\tr: \behaviors_\agents \rightarrow \Traces$ maps each tuple of behaviors to one trace;

    \item for each untrusted agent $u$, the sets $\Ind_u, \Wrong_u \subseteq \Traces$ are respectively the \emph{individual goal} and the \emph{wronging condition} of agent $u$, and they satisfy $\Ind_u \cap \Wrong_u = \emptyset$;

    \item for each nature agent $n$, the set $\Sane_n \subseteq \Traces$ is called the \emph{sanity hypothesis} of agent $n$.
    We call \emph{sane behavior} a behavior $\beta_n$ such that $\tr(\beta_n, \bbeta_{-n}) \in \Sane_n$ for all $\bbeta_{-n}$, and we write $\Sane = \bigcap_n \Sane_n$.
    % We assume that every sane trace is compatible with sane behaviors: for every $\tau \in \Sane$, there exists $\bbeta$ such that $\tr(\bbeta) = \tau$ and that each $\beta_n$ is sane;
    We assume that every nature behavior participating in a sane trace can be considered to be sane: for every $\bbeta$ such that $\tr(\bbeta) \in \Sane$, there exists $\bbeta_\nature'$ such that $\tr(\bbeta) = \tr(\bbeta_{-\nature},\bbeta_\nature')$;

    \item the set $\Coll \in \Traces$ is called the \emph{collective goal}, and is such that for each untrusted agent $u$, we have $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$.
\end{itemize}
\end{defi}

The requirements on sanity hypotheses ensure that sanity should be always achievable by nature agents, regardless of the cooperation of others.
In a sense, it places weak enough conditions to only exclude degenerate behaviors from the nature agents.

\begin{defi}[Protocol, implementation, execution]
    A \emph{protocol} is a nonempty set $P \subseteq \behaviors_{\untrusted \cup \trusted}$.
    An \emph{implementation} of $P$ is an element $\bbeta_{\untrusted \cup \trusted}$ of $P$.
    An \emph{execution} of $\bbeta_{\untrusted \cup \trusted}$ is a trace $\tau$ such that there exists $\bbeta_\nature \in \behaviors_\nature$ with $\tau = \tr(\bbeta)$.
\end{defi}

Note that here a protocol only specifies the actions of trusted and untrusted agents; nature agents cannot be constrained beyond assuming that they do no exhibit insane behaviors.

\begin{defi}[Attack, valid protocol]
    An \emph{attack} of the \emph{alliance} $A \subseteq \untrusted$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists an implementation $\bbeta_{\untrusted \cup \trusted} \in P$ such that, for each $a \in \trusted$ or $a \in \untrusted \setminus A$, we have $\beta_a = \alpha_a$ (the trusted agents, and the untrusted ones that do not belong to $A$, are following the protocol $P$);
    
        \item we have $\tr(\balpha) \in \Sane$ (the sanity hypotheses are satisfied);
    
        \item there exists $u \in A$ such that $\tr(\balpha) \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in A$, we have $\tr(\balpha) \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    A protocol $P$ is \emph{valid} if:
    \begin{itemize}
        \item there is no attack to $P$,
        
        \item and if every implementation of $P$ has a sane execution that satisfies the collective goal.
    \end{itemize}
\end{defi}

Attacks on the protocol may benefit from ``choices'' of the nature agents.
That means that it is not possible to rely on nature agents to prevent attacks (beyond sanity assumptions).
In the absence of nature agents, the above definitions boil down to the original ones; hence nature agents are not a required feature of the modeling of all protocol challenges.

A counterpart to Theorem~\ref{thm:linkSNEvalidNoNature} can still be proved to the case with nature agents.
The payoff functions of the corresponding game $\Game$ are defined as follows:
\Ms{We \textsc{really} need different notations so that the game is know to be a general one here more easily.}
\begin{itemize}
    \item For $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \Wrong_u \\
        1 & \text{if } \tr(\bsigma) \not\in \Wrong_u \cup \Ind_u \\
        2 & \text{if } \tr(\bsigma) \in \Ind_u
    \end{cases};$$

    \item For $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Coll \\
        1 & \text{if } \tr(\bsigma) \in \Coll
    \end{cases};$$

    \item For $n\in \nature$ \emph{(nature players)}:
    $$\mu_n: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Sane_n \\
        1 & \text{if } \tr(\bsigma) \in \Sane_n
    \end{cases}.$$
\end{itemize}

We still assume that $\trusted \neq \emptyset$: if there is no trusted player, we add one that has only one available strategy.

\begin{thm}\label{thm:linkSNEvalid}
    Let $P$ be a protocol in $\pc$.
    The protocol $P$ is valid if and only if for each $\bsigma_{\untrusted \cup \trusted} \in P$, there exists a strategy profile $\bsigma_\nature$ such that the strategy profile $\bsigma$ is a strong Nash equilibrium satisfying $\mu_a(\bsigma) = 1$ for every player $a$.
\end{thm}

\begin{proof}~
    \begin{itemize}
        \item \emph{If $P$ is valid.}
        
        Let $\bsigma_{\untrusted\cup\trusted} \in P$.
        Since $P$ is valid, there exists a strategy profile $\bsigma_\nature$ such that $\tr(\bsigma) \in \Coll \cap \Sane$.
        Moreover, since by definition of a protocol challenge, every nature behavior participating in a sane trace can be assumed to be sane, we can consider that it is indeed the case and that each $\sigma_n$ is sane.
        Since $\tr(\bsigma) \in \Sane$, we have $\mu_n(\bsigma) = 1$ for every $n \in \nature$, and since $\tr(\bsigma) \in \Coll$, we have $\mu_t(\bsigma) = 1$ for each $t \in \trusted$.
        For each $u \in \untrusted$, since $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$ by definition of a protocol challenge, we have $\mu_u(\bsigma) = 1$.

        Let us now prove that $\bsigma$ is an SNE.
        Let us assume that there exists a coalition $C \subseteq \agents$, that has a profitable deviation $\bsigma'_C$.
        Let $\balpha=(\bsigma_{-C},\bsigma_C')$: we will prove that $\balpha$ is an attack to $P$.
        Only untrusted agents can achieve payoff strictly higher than $1$.
        Therefore, we have:
        
        \begin{itemize}
            \item $\mu_a(\balpha) \geq 1$ for all $a \in C$;
            
            \item and there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha) = 2$, i.e. $\tr(\balpha) \in \Ind_u$.
        \end{itemize}

        Note that $\tr(\balpha) \in \Ind_u$ implies $\tr(\balpha) \not\in \Coll$, and therefore $\mu_t(\balpha) = 0$ for every $t \in \trusted$.
        Therefore, the coalition $C$ contains no trusted player.
        Consequently, in the strategy profile $\balpha$, all trusted agents and all the untrusted agents that are not in the coalition do follow $\bsigma_{\untrusted\cup\trusted}$.
        Moreover, each agent of the alliance $A = C \cap \untrusted$ has the payoff at least $1$, i.e. is not wronged; and at least one satisfies their individual objective.

        Let us now show that $\balpha\in\Sane_n$ for all $n\in\nature$.
        If $n \in C$, then $\mu_n(\balpha) \geq  \mu_n(\bsigma)=1$, so $\balpha\in\Sane_n$.
        If $n \notin C$, since $\sigma_n$ is a sane behavior, then it ensures $\balpha \in \Sane_n$ regardless of other players' choices.

        So $\balpha$ is an attack of the alliance $A$ on $P$, which contradicts its validity.


        \item \emph{If every $\bsigma_{\untrusted \cup \trusted} \in P$ can be completed into an SNE $\bsigma$ that yields payoff $1$ to every player.}

        Then, the trace $\tr(\bsigma)$ is an execution of $\bsigma_{\untrusted \cup \trusted}$ that satisfies the collective goal, and all the sanity hypotheses: every implementation of $P$ has an execution that satisfies the collective goal.

        Now, let us assume that there is an attack $\balpha$ of the alliance $A \subseteq \untrusted$ on the protocol $P$.
        Let $\bsigma_{\untrusted \cup \trusted}$ be an implementation of $P$ such that $\balpha_{\trusted \cup \untrusted \setminus A} = \bsigma_{\trusted \cup \untrusted \setminus A}$.
        Let $\bsigma_\nature$ be a strategy profile such that $\bsigma$ is an SNE that gives every player a payoff equal to $1$.
        Consider the coalition $C = A \cup \nature$: we will prove that $\balpha_C$ is a profitable deviation of $\bsigma_C$.
        First, by definition of an attack, we have $\tr(\balpha) \in \Sane$, and therefore $\mu_n(\balpha) = 1$ for each nature player $n$.
        Moreover, for each untrusted agent $u \in A$, we have $\tr(\balpha) \notin \Wrong_u$, i.e. $\mu_u(\balpha) \geq 1$.
        Finally, there is an untrusted agent $u \in A$ such that $\tr(\balpha) \in \Ind_u$, i.e. $\mu_u(\balpha) = 2$.
       As a consequence, the strategy profile $\balpha_C$ is a profitable deviation of $\bsigma_C$, which is impossible since $\bsigma$ is an SNE: there is therefore no attack to $P$, which is a valid protocol.\qedhere
    \end{itemize}
\end{proof}

\begin{cor}
    A protocol challenge admits a valid protocol if and only if the corresponding game admits an SNE that gives every player the payoff $1$.
\end{cor}

==> agentsnaturev2.tex <==
\subsection{On rationality and insanity}

The proposed model relies on the assumption that agents (whether trusted or untrusted) are rational and therefore would always prefer to satisfy their individual objective and to avoid being wronged.
The model only then needs to take into account the possible actions of each agents, whether wise or not with respect to each agent's objectives.

In the case of games specified abstractly, this can be done explicitly.
It is however more practical to reason on a finite model, such as games played on finite graphs (see Definition~\ref{def:gameGraph}).

In that case, some behaviors that are assumed to be impossible require an infinite memory.
For example, it is a common assumption that (neutral) communication channels can delay messages for an arbitrary duration but cannot drop a message altogether.
In an infinite state system, this requirement can be simply described as is: behaviors that lead to an infinite delay between message sending and reception are not possible.
We label these behaviors as \emph{insane}.
On the other hand, on a finite graph arena, this cannot be specified unless an explicit time bound is used.
Therefore a semantic condition has to be introduced to bypass the syntactic limitation of the finite model.
Notice that the ``no dropped message'' condition\footnote{Usually called \emph{fairness} in specification and verification.} can be modeled by the LTL formula $\globally \text{received} \Rightarrow \eventually \text{transmitted}$.
It is thus a finite representation of a semantic condition that has infinitely many possible realizations.
We should also remark that this condition is clearly in the responsibility of a given channel, and not something that would require several players to cooperate in order to happen.

To limit the behaviors of the system to only these \emph{sane} behaviors, there needs to be a clear incentive not to behave insanely.
We therefore add to each untrusted agent $u$ a set $\Sane_u\subseteq \Traces$ of sane traces.
We write $\Sane = \bigcap_{a \in \untrusted} \Sane_a$ the set of traces sane for all agents (called \emph{sane} traces) and $\Sane_{-u} = \bigcap_{\substack{a \in \untrusted\\a\neq u}} \Sane_a$ the set of behaviors sane for all agents but $u$.

We call \emph{sane behavior} a behavior $\beta_u$ such that $\tr(\beta_u, \bbeta_{-u})\in \Sane_u$ for all $\bbeta_{-u}$.
%We assume that every behavior participating in a sane trace can be considered to be sane: for every $\bbeta$ such that $\tr(\bbeta) \in \Sane$, there exists $\bbeta_\untrusted'$ such that $\tr(\bbeta) = \tr(\bbeta_{-\untrusted},\bbeta_\untrusted')$.
%That ensures that sanity is always the result of one's own behavior and may not be influenced by other's behaviors.

The definition of what constitutes an attack on a protocol can therefore be updated as follows:
\begin{defi}[Attack, valid protocol (under sanity hypothesis)]~
\begin{itemize}
    \item 
    An \emph{attack under sanity hypothesis} of the \emph{alliance} $A \subseteq \untrusted$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists an implementation $\bbeta \in P$ such that, for each $a \in \trusted$ or $a \in \untrusted \setminus A$, we have $\beta_a = \alpha_a$ (the trusted agents, and the untrusted ones that do not belong to $A$, are following the protocol $P$);
    
        \item we have $\tr(\balpha) \in \Sane$ (the sanity hypotheses are satisfied);
    
        \item there exists $u \in A$ such that $\tr(\balpha) \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in A$, we have $\tr(\balpha) \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    \item A protocol $P$ is \emph{valid under sanity hypothesis} if:
    \begin{itemize}
        \item all behaviors are sane,
        \item there is no attack to $P$ under sanity hypothesis,
        \item every implementation of $P$ satisfies the collective goal.
    \end{itemize}
    
\end{itemize}
\end{defi}

The addition of sanity hypotheses does not hinder the conversion of the problem into a game.
The payoffs are defined as follows:
\begin{itemize}
    \item For $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in (\Wrong_u \setminus \Sane_{-u}) \cup \overline{\Sane_u} \\
        1 & \text{if } \tr(\bsigma) \in \overline{\Wrong_u} \cap \overline{\Ind_u} \cap \Sane \\
        2 & \text{if } \tr(\bsigma) \in \Sane_u \cap\left(\Ind_u \cup \overline{\Sane_{-u}}\right)
    \end{cases};$$

    \item For $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \overline{\Coll}\cap \Sane \\
        1 & \text{if } \tr(\bsigma) \in \Coll \cup \overline{\Sane}
    \end{cases};$$
\end{itemize}
As we will see in the formal proof, the fact that when a trace is insane for a player $u$, all other players get their maximal payoff will ensure that it is in the best interest of $u$ to play according to a sane strategy.

\begin{thm}\label{thm:linkSNEvalidWithSanity}
    Let $P$ be a protocol in $\pc$.
    The protocol $P$ is valid under sanity assumption if and only if each $\bsigma \in P$ is a strong Nash equilibrium satisfying $\mu_a(\bsigma) = 1$ for every player $a$.
\end{thm}
\begin{proof}~
\begin{description}
    \item[\fbox{$\Rightarrow$}]
    Let $P$ be a valid protocol under sanity assumption.
    Let $\bsigma\in P$, and assume, by way of contradiction that $\bsigma$ is not an SNE with all payoffs at $1$.
    Let $\tau=\tr(\<\bsigma\>)$. 
    First, because of the validity of $P$ we know the collective goal is achieved so $\tau\in\Coll$; that implies that $\tau \notin \Ind_u$ and $\tau \notin \Wrong_u$ for any untrusted player $u$.
    Moreover, as all behaviors are sane, $\tau \in \Sane$.
    Therefore $\mu_a(\bsigma)=1$ for every player $a$.

    So it must be the case that $\bsigma$ is not an SNE, i.e. there exists a profitable deviation for a coalition $C$ of players.
    For the deviation to be profitable, at least a player $a\in C$ must achieve a strictly better payoff while other players in the coalition are not decreasing their own.
    As trusted players cannot improve their payoff, they cannot strictly increase it, so an untrusted agent $u\in C\cap \untrusted$ must achieve a better payoff.
    That can be achieved in two ways:
    \begin{itemize}
        \item Either because the sanity condition of a player $u'\in \untrusted$ is violated.
        That can only happen if said player $u'$ themselves deviated from the sane strategy $\sigma_{u'}$, so $u'\in C$.
        But that means the payoff of $u'$ is now $0$ so a strict decrease, and the deviation is not profitable.
        Hence this case can be excluded.
        \item Or $u$ achieved its individual goal $\Ind_u$.
        In that case the collective goal is not achieved and so all trusted players get a payoff $0$, strictly less than with $\bsigma$, and therefore cannot be part of the coalition $C$.
        As a result $C\subseteq\untrusted$.
    \end{itemize}

    From the above we know that there must be a coalition of untrusted players who can deviate so one of them achieves their individual goal, while others are not wronged.
    This deviation corresponds to an attack on $\bsigma$, which contradicts the validity of $P$.
    
    \item[\fbox{$\Leftarrow$}]~
    Assume all profiles in $P$ are SNEs with all payoffs to $1$.
    In particular, each produced trace must be in $\Sane$, otherwise at least an untrusted player would get payoff $0$.
    As a result, every trusted player having payoff $1$ then means that the collective goal is achieved.

    Assume by way of contradiction that $P$ is not valid.
    There are, then, three possibilities.

    \begin{itemize}
        \item First possibility: one of the untrusted players, say $u$, has an insane behavior, in an implementation $\bsigma$ of $P$.
        Then, there is a deviation $\bsigma'_{-u}$ of $\bsigma_{-u}$ such that $(\sigma_u, \bsigma'_{-u}) \not\in \Sane_u$.
        Then, in the strategy profile $(\sigma_u, \bsigma'_{-u})$, every trusted player gets the payoff $1$, and every untrusted player except $u$ (there is at least one by hypothesis) gets the payoff $2$.
        Such a deviation is therefore profitable, which is impossible since $\bsigma$ is an SNE.
        \Ms{Problème ici: $\bsigma'_{-u}$ peut inclure des comportements insane et donc pas une déviation profitable pour autant.}
        \item Second possibility: there is an attack $\balpha$ on a profile $\bbeta \in P$.
    Let $C$ be the alliance of untrusted agents in the attack.
    Profile $\balpha$ is a deviation of untrusted players where:
    \begin{itemize}
        \item all sanity hypotheses are statisfied;
        \item a player $u\in C$ achieves $\Ind_u$;
        \item no player $C$ is wronged.    
    \end{itemize}
    One can check that this corresponds to a profitable deviation for players in $C$, thus contradicting the fact that $\bbeta$ is an SNE.


        \item Third possibility: an implementation $\bsigma$ of $P$ does not satisfy the collective goal.
        Then, if $t$ is a trusted player (there is at least one by hypothesis), we have $\mu_t(\bsigma) = 0$, which is impossible since every player is supposed to get the payoff $1$.
    \end{itemize}
    \qedhere
\end{description}
\end{proof}

==> algorithmsMultiValuedSNE.tex <==
%% Multivalued {parity|omega-regular} games: testing and existence of Strong Nash Equilibria
    \section{Algorithms}

In this section, we study natural decision problems on SNEs that arise from the links we have drawn with security protocols.
First, we study the SNE-checking problem, which appears when a given protocol has to be formally verified.
Second, we study the fixed-payoff SNE existence problem, which appears when one wants to know whether a valid protocol exist in a given protocol challenge.
We study those problems in two classes of games, that cover the games obtained in the examples studied above.
We give tight complexity bounds to all those problems.


        \subsection{Definition of the problems}
        
\Ms{We must use games over a finite graph arena here; what names/notations should be used in order to differentiate from general games of Definition~\ref{def:generalGame}?}

In what follows, we will use parity conditions as a succinct way to encode $\omega$-regular sets of plays.

\begin{defi}[Parity condition]
    Let $(V, E)$, and let $\kappa: V \to \NN$ be a mapping, called \emph{color mapping}.
    The set $\Parity(\kappa)$ is the set of infinite paths $\alpha$ in $(V, E)$, such that $\min_{v \in \Inf(\alpha)} \kappa(v)$ is an even integer.
\end{defi}

\begin{defi}[Parity automaton]
    A parity automaton over alphabet $X$ is a tuple $\auto=(X,S,s_0,T,\kappa)$ where $S$ is a set of states, $T:S\times X \to S$ is a deterministic transition function, and $\kappa: S \to \NN$ is a color mapping.
    Given a word $w=w_0w_1\cdots\in X^\omega$, the run of $\auto$ on $w$ is $\rho_\auto(w)=s_0 s_1 \cdots$ where for $i\in \NN$, $s_{i+1}=T(s_i,w_i)$.
    The set of infinite words accepted by $\auto$ is $\Lang(\auto)= \left\{w\in X^\omega \mmid \rho_\auto(w)\in\Parity(\kappa)\right\}$.
\end{defi}

It is well-known that the set of languages recognized by parity automata is exactly the set of $\omega$-regular languages.
Now, we consider two classes of games, that fit with the games that are in practice obtained from protocol challenges: games in which a finite number of payoffs is possible for each player, and in which the set of plays granting a given payoff to a given player is defined by a parity condition, or by a parity automaton.

\begin{defi}[Multi-valued parity game]
    A \emph{multi-valued parity game}, or \emph{MVP game} for short, is a multi-player game $\Game_{\|v_0}$ such that there exists two integers $p$ and $m$, and for each player $i$, exactly $p$ color mappings $\kappa_{i1}, \dots, \kappa_{ip}: V \to \{0, \dots, m-1\}$, such that for each play $\pi$, we have $\mu_i(\pi) = \max\{j ~|~ \pi \in \Parity(\kappa_{ij})\}$ (with the convention $\max\emptyset = 0$).
\end{defi}

\begin{defi}[Multi-valued $\omega$-regular game]
    A \emph{multi-valued $\omega$-regular game}, or \emph{MV$\omega$R game} for short, is a multi-player game $\Game_{\|v_0}$ such that there exists two integers $p$ and $m$, and for each player $i$, $p$ parity automata $\auto_{i1},\dots,\auto_{ip}$ over alphabet $V$, such that  for each play $\pi$, we have $\mu_i(\pi) = \max\{j ~|~ \pi \in \Lang(\auto_{ij})\}$ (with the convention $\max\emptyset = 0$).
\end{defi}

Remark that an MVP game is a particular case of an MV$\omega$R game, where all automata $\auto_{i1},\dots,\auto_{ip}$ have the same structure: one state $s_v$ per vertex $v$ of the game to remember the last visited vertex.
The transition function it $T(s_v,v')=s_{v'}$.
For each automaton $\auto_{ij}$, the color of $s_v$ is $\kappa_{ij}(v)$.

We must now present how we encode strategies for the players: Mealy machines.
In such a machine, the states represent the memory of the player.
At each turn, the current vertex in the game is read, firing a transition to a new state; and if the current vertex is controlled by the player using the machine, then the transition outputs a new vertex, to which the player goes.
We do not impose determinism on Mealy machines, since a protocol is often not defined itself in a deterministic way: it may be ambiguous about minor aspects, or be able to respond to different types of requests.
As we will see later, non-determinism has, in practice, no impact on complexity.

\begin{defi}[Mealy machine]
    A \emph{Mealy machine for player $i$} on a game $\Game$ is a tuple $\Mach = (Q, q_0, \Delta)$, where $Q$ is a finite set of \emph{states}, where $q_0 \in Q$ is the \emph{initial state}, and where $\Delta \subseteq (Q \times V_{-i} \times Q) \cup (Q \times V_i \times Q \times V)$ is a finite set of \emph{transitions}, such that for every $(p, u, q, v) \in \Delta$, we have $uv \in E$, and such that for every $p \in Q$ and $u \in V$, there exists a transition $(p, u, q)$ or $(p, u, q, v) \in \Delta$.
        When for each $p$ and $u$, there exists exactly one such transition, we say that the machine $\Mach$ is \emph{deterministic}.
		
		A strategy $\sigma_i$ in $\Game_{\|v_0}$ is \emph{compatible} with $\Mach$ if there exists a mapping $h \mapsto q_h$ that maps every history $h$ in $\Game_{\|v_0}$ to a state $q_h \in Q$, such that for every $hv \in \Hist_{-i} \Game_{\|v_0}$, we have $(q_h, v, q_{hv}) \in \Delta$, and for every $hv \in \Hist_i \Game_{\|v_0}$, we have $(q_h, v, q_{hv}, \sigma_i(hv)) \in \Delta$.
		The set of strategies in $\Game_{\|v_0}$ compatible with $\Mach$ is written $\Comp_{\|v_0}(\Mach)$.
		If $\Mach$ is deterministic, then there is exactly one strategy compatible with $\Mach$; we call it a \emph{finite-memory} strategy.

  
We define analogously Mealy machines that capture a set of strategy profiles for several players, including for the whole set $\Pi$.
In such a case, we simply call it \emph{machine on the game $\Game$}, with no mention of a player.
\end{defi}

We can now define the decision problem we will study.
First, the verification of a protocol amounts to decide, given the description of a strategy profile, whether all strategy profiles compatible with that description are SNEs.
Two approaches are possible regarding how the strategy profile is described: with one unique machine, or one per agent.

\begin{pb}[SNE-checking problem]
    Given an MVP game (resp. MV$\omega$R game) $\Game_{\|v_0}$ and a Mealy machine $\Mach$ on $\Game$, is every strategy profile compatible with $\Mach$ an SNE?
\end{pb}

\begin{pb}[Compositional SNE-checking problem]
    Given an MVP game (resp. MV$\omega$R game) $\Game_{\|v_0}$ and a family of Mealy machines $(\Mach_i)_{i \in \Pi}$ on $\Game$, is every strategy profile $\bsigma$, with $\sigma_i \in \Comp(\Mach_i)$ for each $i$, an SNE?
\end{pb}


Later, we will also study a more complex problem: the synthesis of valid protocol, which amounts to search for an SNE with a given outcome in a given game.

\begin{pb}[Fixed-payoff SNE existence problem]
    Given an MVP game (resp. MV$\omega$R game) $\Game_{\|v_0}$ and a payoff vector $\bx$, does there exist an SNE $\bsigma$ in $\Game_{\|v_0}$ such that $\mu\< \bsigma \> = \bx$?
\end{pb}

A possible extension of that problem is the following.

\begin{pb}[Threshold SNE existence problem]
    Given an MVP game (resp. MV$\omega$R game) $\Game_{\|v_0}$ and two payoff vectors $\bx, \by$, does there exist an SNE $\bsigma$ in $\Game_{\|v_0}$ such that $\bx \leq \mu\< \bsigma \> \leq \by$?
\end{pb}



        \subsection{SNE-checking problems}
            \subsubsection{A tool: the product graph}

Let us first present the method we will use for all the algorithms solving SNE-checking problems: construct the \emph{product graph} of the game and the Mealy machine(s), in order to search for a pair of paths (a \emph{critical pair}) that would correspond to a profitable deviation.

\begin{defi}[Product graph]\label{def:product_graph}
    Consider a graph game $\Game_{\|v_0}$, and a Mealy machine $\Mach$ on $\Game$.
    We define the product $\Game_{\|v_0} \otimes \Mach$ as the graph $(V \times S, E^\times)$ where $(u, s)(v, t) \in E^\times$ if and only if we have $uv \in E$, and if there exists $w \in V$ with $(s, u, t, w) \in \Delta$.
    If $(s, u, t, v) \in \Delta$, then the edge $(u, s)(v, t) \in E$ is called a \emph{non-deviating} edge, and otherwise, it is called an \emph{$i$-deviating} edge, where $i$ is the player controlling the vertex $u$.
    Given a path $\alpha = (u_0, s_0)(u_1, s_1) \dots$ in $\Game_{\|v_0} \otimes \Mach$, we write $\dalpha$ the projection $u_0u_1 \dots$.

    We call \emph{critical pair} in $\Game_{\|v_0} \otimes \Mach$ a pair $(\alpha, \beta)$ of paths, starting from the vertex $(v_0, s_0)$, such that:
        \begin{itemize}
            \item the path $\alpha$ has no deviating edge;

            \item if $k$ is the least index such that $\alpha_k \neq \beta_k$, then the edge $\alpha_{k-1}\beta_k$ is deviating;

            \item there is one player $i$ such that $\mu_i(\dalpha) < \mu_i(\dbeta)$;

            \item for every player $i$ such that $\beta$ contains an $i$-deviating edge, we have $\mu_i(\dalpha) \leq \mu_i(\dbeta)$.
        \end{itemize}
\end{defi}

Note that the player $i$ who has a strictly greater payoff in $\bbeta$ than in $\balpha$ is not required to actively deviate: he or she may still be part of the deviating coalition.
Then, as expected, the existence of a critical pair is equivalent to the existence of a profitable deviation in one of the strategy profiles compatible with the Mealy machine.

\begin{thm} \label{thm:product_graph}
    Let $\Game_{\|v_0}$ be a graph game, and let $\Mach$ be a Mealy machine on $\Game$.
    There exists a strategy profile $\bsigma$ compatible with the machine $\Mach$ that is not an SNE if and only if there exists a critical pair in $\Game_{\|v_0} \otimes \Mach$.
\end{thm}

\begin{proof}
    \begin{itemize}
        \item Let $(\alpha, \beta)$ be such a critical pair, let $i$ be a player such that $\mu_i(\dalpha) < \mu_i(\dbeta)$, and let $C$ be the set of players $j$ such that $\beta$ has an $j$-deviating edge, plus $i$.
        Let us write $\alpha = (\pi_0, s_0) (\pi_1, s_1) \dots$ and $\beta = (\chi_0, t_0) (\chi_1, t_1) \dots$.
        Let $k$ be the least index such that $\alpha_k \neq \beta_k$.
        Let us define a strategy profile $\bsigma \in \Comp(\Mach)$ by defining the mapping $h \mapsto q_h$ as follows: for each $\l$, we define $q_{\dalpha_{\leq \l}} = s_\l$, and $q_{\dbeta_{\leq \l}} = t_\l$.
        We define the other states $q_h$ arbitrarily.

        Then, we have $\dalpha = \< \bsigma \>$, and $\dbeta$ is compatible with the strategy profile $\bsigma_{-C}$.
        Moreover, we have $\mu_C(\dbeta) > \mu_C(\dalpha)$, hence the coalition $C$ has a profitable deviation in the strategy profile $\bsigma$.

        \item Conversely, if a given coalition $C$ has a profitable deviation $\bsigma'_C$ to a strategy profile $\bsigma \in \Comp(\Mach)$, then let $h \mapsto q_h$ be the mapping corresponding to $\bsigma$.
        Let us define $\alpha = (\pi_0, q_{\pi_0}) (\pi_1, q_{\pi_0\pi_1}) (\pi_2, q_{\pi_0\pi_1\pi_2}) \dots$, and $\beta = (\chi_0, q_{\chi_0}) (\chi_1, q_{\chi_0\chi_1}) \dots$, where $\pi = \< \bsigma \>$ and $\chi = \< \bsigma_{-C}, \bsigma'_C \>$.
        Then, since $\bsigma'_C$ is a profitable deviation to $\bsigma$, there is a player $i \in C$ that has a better payoff in $\dalpha = \pi$ than in $\dbeta = \chi$, and every player $j$ such that there is a $j$-deviating edge along $\beta$ belongs to $C$, and has therefore at least the same payoff in $\dbeta$ than in $\dalpha$.
        The path $\alpha$ has also no deviating edge, and the path $\beta$ gets separated from it with a deviating edge: the paths $\alpha$ and $\beta$ form a critical pair.
    \end{itemize}
\end{proof}



        
            \subsubsection{MVP games}

Using that preliminary result, we first provide an optimal algorithm in the case of MVP games.
That algorithm consists in guessing and checking the optimal pair in polynomial time.

\begin{thm}\label{thm:SNEcheckingMVP}
    In MVP games, the SNE-checking problem is $\coNP$-complete, even if the Mealy machine is deterministic.
\end{thm}

\begin{proof}
    \begin{itemize}
        \item \emph{Easiness.}

        By Theorem~\ref{thm:product_graph}, this problem reduces to deciding the non-existence of a critical pair in the graph $\Game_{\|v_0} \otimes \Mach$.
        We prove that if such a pair $(\alpha, \beta)$ exists, then there also exists a critical pair $(hc^\omega, h'd^\omega)$ of lassos whose sizes are polynomial in the size of $\Game_{\|v_0} \otimes \Mach$, and therefore in the size of the input.
        Let $n$ be the number of vertices in the graph $\Game_{\|v_0} \otimes \Mach$.

        Indeed, given the critical pair $(\alpha, \beta)$, let $k$ be the least index such that $\alpha_k \neq \beta_k$.
        The vertex $\alpha_{k-1}$ is accessible from $\alpha_0$: therefore, there exists a path $h_0$ from $\alpha_0$ to $\alpha_{k-1}$, with no deviating edge, that has length at most $n$.
        Then, let $m > k$ be an index such that every vertex in $\alpha_{\geq m}$ is visited infinitely often by $\alpha$.
        In particular, it is the case of the vertex $\alpha_m$, and there exists an index $\l$ such that $\alpha_\l = \alpha_m$, and $\Occ(\alpha_m \dots \alpha_{\l - 1}) = \Inf(\alpha)$.
        There is, therefore, a path from $\alpha_m$ to itself that visits all the vertices of the set $\Inf(\alpha)$ and only them, and that uses no deviating edges: therefore, there exists a path $c$ that satisfies the same properties and that has length at most $n^2$.
        Moreover, there is a path $h_1$ from $\alpha_k$ to $\alpha_m$ with no deviating edges of size at most $n$.
        Then, the lasso $\alpha' = h_0 h_1 c^\omega$ is such that $\mu(\dalpha') = \mu(\dalpha)$, and it size is at most $2n + n^2$.
        We define analogously a lasso $\beta' = h_0 h_2 d^\omega$ such that $\mu(\dbeta') = \mu(\dbeta)$, and such that for every $i$, if there is an $i$-deviating edge in $\beta'$, then there is an $i$-deviating edge in $\beta$.
        Then, the pair $(\alpha', \beta')$ is critical.

        Therefore, such a pair can be guessed and checked in polynomial time: negative instances of the SNE-checking problem can be recognized in non-deterministic polynomial time.
        
        

        \item \emph{Hardness.}
        
        We encode the negation of the satisfiability problem.
        Namely, for a propositional formula $\varphi$, we build a game $\Game$ and a machine $\Mach$ such that $\varphi$ is satisfiable if and only if there is a profile in $\Mach$ that is not an SNE.

        Let $\varphi=\bigwedge_{i=1}^k \bigvee_{j=1}^m L_{ij}$ with $L_{ij}\in \textit{Lit}=\{x_1,\neg x_1,\dots,x_n,\neg x_n\}$ be a propositional formula.
        We build a game with $2n+1$ players $\textit{Lit}\uplus\eve$ as depicted in \figurename~\ref{fig:sat2sneCheck}.
        Player $\eve$ controls circular vertices, while rectangular vertices are controlled by the player identified in the bottom right corner (if any; vertices with a single successor could belong to anyone).
        It is made of two parts: in the first part $\eve$ chooses a valuation by selecting vertices (the \emph{setting} module), and in the second part the formula is checked by traversing all clauses and selecting one literal per clause (the \emph{checking} module).
        Note that each player in $\textit{Lit}$ can, when given the opportunity to play, choose to exit a sink vertex $\blacktriangledown$ (duplicated for clarity); in that case the checking module is never reached.
        
        The coloring functions to achieve payoff $1$ are defined as follows (otherwise payoff $0$ is awarded):
        \begin{itemize}
            \item For $\ell\in\textit{Lit}$:
            \begin{itemize}
                \item $\kappa_{\ell}(\blacktriangledown)=0$;
                \item for every $L_{ij}=\neg\ell$ in the checking module, $\kappa_\ell(L_{ij})=1$;
                \item $\kappa_\ell(\checkmark)=2$.
                \item for any other vertex $v$, $\kappa_\ell(v)=3$.
            \end{itemize}
            \item For $\eve$:
            \begin{itemize}
                \item $\kappa_\eve(\blacktriangledown)=1$;
                \item $\kappa_\eve(\checkmark)=2$.
                \item for any other vertex $v$, $\kappa_\eve(v)=3$.
            \end{itemize}
        \end{itemize}
        So a player $\ell\in\textit{Lit}$ can achieve payoff $1$ by either reaching $\blacktriangledown$ or avoiding infinite visits to its negation in the checking module.
        On the other hand, $\eve$ achieves $1$ by reaching the checking module.

        Let $\Mach_{\textit{Lit}}$ be the deterministic Mealy machine with a single state that encodes the strategy profile that has all players in $\textit{Lit}$ go to $\blacktriangledown$, and Eve do arbitrary actions.
        Let $\bsigma$ be a profile defined by this machine.
        Note that with $\bsigma$ $\eve$ gets payoff $0$ while all other players get payoff $1$.
        We show that $\bsigma$ is an SNE if and only if $\varphi$ is not satisfiable.

        Assume that $\varphi$ is satisfiable.
        Then we construct a deviation to $\bsigma$.
        Let $\zeta$ be a valuation such that $\zeta \vDash \varphi$.
        Let $C$ the coalition of players made of $\eve$ and players selected by $\zeta$ as follows: if $\zeta(x_i)=\top$ then $x_i\in C$, if $\zeta(x_i)=\bot$ then $\neg x_i\in C$.
        Note that this coalition contains exactly one literal per variable.
        Let $\bsigma'$ be the profile that deviates from $\bsigma$ for players in $C$ as follows:
        \begin{itemize}
            \item for $x_i$ (resp. $\neg x_i$) $\in \textit{Lit} \cap C$, from $x_i^s$ (resp. $\neg x_i^s$) choose $?x_{i+1}$ (or $C_1$ if $i=n$)
            \item from $?x_i$ $\eve$ chooses $x_i^s$ if $\zeta(x_i)=\top$ and $\neg x_i^s$ if $\zeta(x_i)=\bot$.
            \item from $C_i$, $\eve$ chooses a literal that is $\top$ in $\zeta$; since $\zeta\vDash \varphi$, this is always possible.
        \end{itemize}
        Note that with this profile no player outside of $C$ actually plays, so the $\blacktriangledown$ vertex is not reached.
        As a result, $\bsigma'$ yields payoff $1$ for $\eve$.
        In addition, no negation of a literal in $C$ is ever reached in the checking module, so all players in $C$ still get payoff $1$.
        Therefore the deviation $\bsigma'$ is profitable for coalition $C$ and $\bsigma$ is not an SNE.

        Now assume that $\varphi$ is not satisfiable.
        Let $C$ be a coalition of players and $\bsigma'$ a profile that deviates for players in $C$.
        Since only $\eve$ can improve its payoff, any coalition without $\eve$ cannot have a profitable deviation.
        So $\eve\in C$.
        Furthermore, if for a variable $x_i$, neither player $x_i$ nor $\neg x_i$ are in $C$, then the play reaches $\blacktriangledown$ and the payoff remains the same for all players.
        So for the deviation to be profitable, at least one player per variable must be in $C$, and the corresponding vertex must be reached in the setting module (by decision of $\eve$) and they must actually deviate to avoid $\blacktriangledown$.
        Now since $\varphi$ is not satisfiable, in every loop of the checking module there must be at least a literal and its negation that are visited, so for some $i$ both $x_i$ and $\neg x_i$ see a color $1$ in this loop.
        As there are infinitely many turns of loops in the checking module, there is an index $i$ for which both players $x_i$ and $\neg x_i$ get payoff $0$.
        Since (at least) one of them is in the coalition $C$, the deviation is not profitable.
        Therefore $\bsigma$ is an SNE.\qedhere        
    \end{itemize}
\end{proof}
\begin{figure}
    \centering
    
    \begin{subcaptionblock}{\textwidth}
    \centering
    \begin{tikzpicture}[node distance=50pt]
        % Setting the valuation
        \node[solverState,initial] at (0,0) (q1) {$?x_1$};
        \node[literalState=$x_1$,above right of=q1] (p1) {$x_1^s$};
        \node[literalState=$\neg x_1$,below right of=q1] (n1) {$\neg x_1^s$};
        \node[solverState,below right of=p1] (q2) {$?x_2$};
        \node[literalState=$x_2$,above right of=q2] (p2) {$x_2^s$};
        \node[literalState=$\neg x_2$,below right of=q2] (n2) {$\neg x_2^s$};
        \node[below right of=p2] (q3) {$\cdots$};
        \node[literalState=$x_n$,above right of=q3] (pn) {$x_n^s$};
        \node[literalState=$\neg x_n$,below right of=q3] (nn) {$\neg x_n^s$};

        % Checking all the clauses
        \node[solverState,below right of=pn] (c1) {$C_1$};
        \node[nobodyState,above right of=c1] (l11) {$L_{1,1}$}; %\cobuchiLabel[inner sep=0pt,cloud puff arc=95]{l11}{$\neg L_{1,1}$}
        \node[nobodyState,below right of=c1] (l1m1) {$L_{1,m_1}$};  %\cobuchiLabel[inner sep=0pt,cloud puff arc=95]{l1m1}{$\neg L_{1,m_1}$}
        \node (c1dots) at (barycentric cs:l11=1,l1m1=1) {$\myvdots$};
        \node[solverState,below right of=l11] (c2) {$C_2$};
        \node[above right of=c2] (l21) {$\myiddots$};
        \node[below right of=c2] (l2m2) {$\myddots$};
        \node (c2dots) at (barycentric cs:l21=1,l2m2=1) {$\myvdots$};
        \node[right of=l21,node distance=2.5cm] (lp1) {$\myddots$};
        \node[right of=l2m2,node distance=2.5cm] (lpmp) {$\myiddots$};
        \node (cpdots) at (barycentric cs:lp1=1,lpmp=1) {$\myvdots$};
        \node[yshift=7pt] (ldots1) at (barycentric cs:l21=1,lp1=1) {$\cdots$};
        \node[yshift=-7pt] (ldotsm) at (barycentric cs:l2m2=1,lpmp=1) {$\cdots$};
        \node (ldots) at (barycentric cs:ldots1=1,ldotsm=1) {$\cdots$};
        \node[nobodyState,below right of=lp1] (ph) {$\checkmark$}; %\cobuchiLabel[fill=green!80!black]{ph}{$\eve$}

        % Sink state
        \node[nobodyState,above of=p2] (sinkTop) {$\blacktriangledown$}; %\cobuchiLabelTop{sinkTop}{$\eve$}
        \node[nobodyState,below of=n2] (sinkBot) {$\blacktriangledown$}; %\cobuchiLabelBot{sinkBot}{$\eve$}

        \begin{pgfonlayer}{arrows}
            \path[->] (q1) edge (p1) edge (n1);
            \path[->] (p1) edge (q2) edge[bend left,out=-30] (sinkTop);
            \path[->] (n1) edge (q2) edge[bend right,out=30] (sinkBot);
            \path[->] (q2) edge (p2) edge (n2);
            \path[->] (p2) edge (q3) edge (sinkTop);
            \path[->] (n2) edge (q3) edge (sinkBot);
            \path[->] (q3) edge (pn) edge (nn);
            \path[->] (pn) edge (c1) edge[bend right,out=30] (sinkTop);
            \path[->] (nn) edge (c1) edge[bend left,out=-30] (sinkBot);
    
            \path[->] (c1) edge (l11) edge (c1dots) edge (l1m1);
            \path[<-] (c2) edge (l11) edge (c1dots) edge (l1m1);
            \path[->] (c2) edge (l21) edge (c2dots) edge (l2m2);
            \path[<-] (ph) edge (lp1) edge (cpdots) edge (lpmp);

            \path[->] (ph) edge[out=-90,in=-90,distance=4cm] (c1);
    
            \path[->] (sinkTop) edge[loop above] (sinkTop);
            \path[->] (sinkBot) edge[loop below] (sinkBot);
            \end{pgfonlayer}
    \end{tikzpicture}
    \caption{Game $\Game_\varphi$ to encode the satisfiability of propositional formula $\varphi$ into a game.}
    \label{fig:sat2sneCheckArena}
    \end{subcaptionblock}
    
    \begin{subcaptionblock}{0.4\textwidth}
    \centering
    \begin{tikzpicture}
        \node[state,initial] (q) {};
        \path[->] (q) edge [loop above] node {$x_i^s | \blacktriangledown$} (q);
        \path[->] (q) edge [loop below] node {$\neg x_i^s | \blacktriangledown$} (q);
        \path[->] (q) edge [loop right] node {else$| \ast$} (q);
    \end{tikzpicture}
    \caption{Mealy machine $\Mach_{\textit{Lit}}$.}
    \label{fig:sat2sneCheckMachine}
    \end{subcaptionblock}
    \caption{Encoding of SAT into an MVP SNE-checking problem.}
    \label{fig:sat2sneCheck}
\end{figure}


        \subsubsection{MV\texorpdfstring{$\omega$}{ω}R games}

In the case of MV$\omega$R games, the existence of a critical pair with a polynomial description is no longer guaranteed in negative instances.
The critical pair must therefore be guessed step by step, yielding a $\PSpace$ algorithm.

\begin{thm}\label{thm:SNEcheckingMVoR}
    In MV$\omega$R games, the SNE-checking problem is $\PSpace$-complete.
\end{thm}


\begin{proof}
    \begin{itemize}
        \item \emph{Easiness.}

        We give a non-deterministic algorithm that decides the SNE-checking problem using polynomial space.
        By Theorem~\ref{thm:product_graph}, that problem reduces to search for a critical pair of paths in the product graph $\Game_{\|v_0} \otimes \Mach$.
        If such a pair $(\alpha, \beta)$ exists, then there also exists a critical pair $(h c^\omega, h' d^\omega)$ of lassos.
        Indeed, let $m$ be an index such that $\alpha_{\leq m} \neq \beta_{\leq m}$, and such that every vertex in $\alpha_{\geq m}$ is visited infinitely often by that path.
        Then, in particular, there is an index $n$ such that $\alpha_n = \alpha_m$.
        Let us then define $h = \alpha_{< m}$ and $c = \alpha_m \dots \alpha_{n-1}$, and let us define similarly $h'$ and $d$.
        Since the projections of $hc^\omega$ and $h' d^\omega$ in $\Game_{\|v_0}$ give to all players the same payoffs as $\alpha$ and $\beta$, respectively, the pair $hc^\omega, h'd^\omega)$ is also critical.
        Let us therefore present an algorithm searching for such lassos.

        That algorithm can, then, guess those lassos "on the fly", as follows:
        
        \begin{itemize}
            \item guess, vertex by vertex, the common prefix of $h$ and $h'$, with only non-deviating edges, and while doing so, run the automata $\auto_{ij}$ (memorize nothing but the current vertex, and the current state in each $\auto_{ij}$);

            \item guess the time of the first deviation: then, guess a non-deviating edge (to $u$) and a deviating edge (to $v$), and memorize $v$, and the current states of each automaton $\auto_{ij}$ when reaching $v$;

            \item guess the end of $hc^\omega$: from $u$, guess vertex by vertex a path with no deviating edges, then guess which of those vertex will be repeated, memorize it, and guess the path from it to itself, still without deviating edge, and memorizing which states of each $\auto_{ij}$ are visited while doing so;

            \item proceed similarly to guess the end of $h'd^\omega$ from $v$, using also deviating edges, and also memorizing which players deviate;

            \item then, use the data that has been memorized to compute $\mu_i(hc^\omega)$ and $\mu_i(h'd^\omega)$ for each $i$, and then check whether the pair $(hc^\omega, h'd^\omega)$ is critical.
        \end{itemize}

    
        \item \emph{Hardness.}

        We proceed by reduction from the following $\PSpace$-hard problem~\cite{Kozen77}: given $n$ deterministic finite automata $\auto_1, \dots, \auto_n$ on the alphabet $\{a, b\}$, is the intersection $\bigcap_i \Lang(\auto_i)$ empty?
        Given $n$ such finite automata, we construct a MV$\omega$R game $\Game_{\|v_0}$ and a Mealy machine $\Mach$ such that every strategy profile compatible with $\Mach$ is an SNE in $\Game_{\|v_0}$ if and only if $\bigcap_i \Lang(\auto_i) = \emptyset$.

        The game $\Game_{\|v_0}$ has $n+1$ players, namely players $1, \dots, n$ and \emph{Solver}, written $\SS$.
        For each $i \in \{1, \dots, n\}$, there is a vertex $i$ controlled by player $i$, with two outgoing edges: one to the sink vertex $\btd$, and one to the vertex $i+1$ (or $c$ if $i=n$).
        Solver controls two vertices, named $a$ and $b$, each of them having three outgoing edges: one to $a$, one to $b$, and one to a last sink vertex $\bt$.
        The vertices $\btd$ and $\bt$ have both only one outgoing edge, a self-loop.
        The initial vertex is $v_0 = 1$.
        That game is depicted by Figure~\ref{fig:MVoR_checking_hardness_arena}: each square vertex belong to the number player indicated on the vertex, and the round vertices belong to Solver.

        Each player has two possible payoffs, $0$ and $1$ --- we will therefore use the words \emph{win} and \emph{lose} to say that a player gets either of those.
        The parity automata that recognize the winning plays of each player are depicted by Figures~\ref{fig:MVoR_checking_hardness_solver} and~\ref{fig:MVoR_checking_hardness_i}.
        The number inside each state is its color.
        In Figure~\ref{fig:MVoR_checking_hardness_i}, each state of the automaton $\auto_i$ is given the color $1$, and an outgoing transition with label $\bt$ is added to each of them: to the sink state of color $0$ if it is an accepting state, to the sink state of color $1$ otherwise.
        Thus, Solver wins if and only if the vertex $c$ is reached; and each player $i$ wins if and only if either the vertex $\btd$ is reached, or the vertex $c$ is reached, Solver writes a word that is accepted by $\auto_i$, and then goes to $\bt$.

        Finally, the Mealy machine $\Mach$ is the deterministic one-state machine that makes all the number players go to the vertex $\btd$, and that makes Solver do arbitrary actions.


\begin{figure}
    \centering

\begin{subcaptionblock}{0.9\textwidth}
    \centering
    \begin{tikzpicture}[node distance=2cm]
        \node[literalState=$1$,initial] (1) at (0,0) {$1$};
        \node[literalState=$2$,right of=1] (2) {$2$};
        \node[right of=2] (dots) {$\cdots$};
        \node[literalState=$n$,right of=dots] (n) {$n$};
        \node[state, below right of=n] (a) {$a$};
        \node[nobodyState, below right of=a] (bt) {$\bt$};
        \node[state, above right of=bt] (b) {$b$};
        \node[nobodyState,below of=dots] (btd) {$\btd$};
        \node[state, above right of=a] (c) {$c$};
\begin{pgfonlayer}{arrows}
        \path[->] (1) edge (2);
        \path[->] (2) edge (dots);
        \path[->] (dots) edge (q);
        \path[->] (n) edge (c);
        \path[->] (c) edge[bend right] (a);
        \path[->] (c) edge[bend left] (b);
        \path[->] (a) edge[bend right] (b);
        \path[->] (b) edge[bend right] (a);
        \path[->] (a) edge[loop left] (a);
        \path[->] (b) edge[loop right] (b);
        \path[->] (1) edge[bend right] (btd);
        \path[->] (2) edge[bend right, in=150] (btd);
        \path[->] (n) edge[bend left] (btd);
        \path[->] (btd) edge[loop below] (btd);
        \path[->] (a) edge[bend right] (bt);
        \path[->] (b) edge[bend left] (bt);
        \path[->] (bt) edge[loop below] (bt);
        \end{pgfonlayer}
    \end{tikzpicture}
    \caption{The arena.}
    \label{fig:MVoR_checking_hardness_arena}
    \end{subcaptionblock}

    
    \begin{subcaptionblock}{0.35\textwidth}
    \centering
    \begin{tikzpicture}[auto,node distance=3cm]
        \node[automatonState,initial] (init) at (0,0) {$1$};
        \node[automatonState,right of=init] (win) {$0$};
        \path[->] (init) edge[loop above] node{$1,\dots,n,\btd$} (init);
        \path[->] (init) edge node{$c$} (win);
        \path[->] (win) edge[loop above] node{$a,b,\bt$} (win);
    \end{tikzpicture}
    \caption{The parity automaton $\auto_{\SS 1}$.}
    \label{fig:MVoR_checking_hardness_solver}
    \end{subcaptionblock}
    
    
    \hfill
    
    \begin{subcaptionblock}{0.7\textwidth}
    \centering
    \begin{tikzpicture}[auto,node distance=3cm]
        \node[automatonState,initial] (init) at (0,0) {$1$};
        \node[automatonState,below right of=init] (win) {$0$};
        \node[automatonState,rectangle,rounded corners=7pt,dotted,minimum size=3cm,above right of=win] (autom) {$\auto_{i}$};
        \node[automatonState,double] (qacc) at (3.5, -1) {1};
        \node[automatonState] (someq) at (5, -1) {1};
        \node[automatonState,below right of=autom] (lose) {$1$};
        
        
        \path[->] (init) edge[loop above] node{$1,\dots,n$} (init);
        \path[->] (init) edge node{$c$} (autom);
        \path[->] (init) edge node{$\btd$} (win);
        \path[->] (qacc) edge node{$\bt$} (win);
        \path[->] (someq) edge node{$\bt$} (lose);
        \path[->] (win) edge[loop below] node{$*$} (win);
        \path[->] (lose) edge[loop below] node{$*$} (lose);
    \end{tikzpicture}
    \caption{The parity automaton $\auto_{i1}$ for player $i \in \{1, \dots, n\}$}
    \label{fig:MVoR_checking_hardness_i}
    \end{subcaptionblock}

    \caption{Encoding of the intersection emptiness problem into an MV$\omega$R SNE-checking problem.}
    \label{fig:MVoR_checking_hardness}
\end{figure}

Thus, let us assume that there is a strategy profile $\bsigma$ that is compatible with $\Mach$, and that is not an SNE.
The play $\< \bsigma \>$ reaches the vertex $\btd$, and is therefore won by all the players, except Solver: a profitable deviation must therefore be won by Solver, i.e. reach the vertex $c$.
To do so, a deviating coalition must necessarily include all the number players; otherwise the player that would not be included would still go to the vertex $\btd$.
Consequently, a profitable deviation $\bsigma'$ of $\bsigma$ is necessarily a deviation of all the players, and must generate a play that is won by all of them.
Such a play must have the form $\< \bsigma' \> = 1 2 \dots n w \bt^\omega$, where $w$ is a word accepted by every automaton: the intersection $\bigcap_i \Lang (\auto_i)$ is then nonempty.

Conversely, if that intersection is nonempty, then a profitable deviation for the coalition of all the players consists in going to the vertex $c$, writing a word $w \in \bigcap_i \Lang (\auto_i)$, and then going to the sink vertex $\bt$.

Thus, the emptiness problem of the intersection of finite automata reduces to the SNE-checking problem in MV$\omega$R games, with a deterministic Mealy machine: that problem is therefore $\PSpace$-hard.
    \end{itemize}
\end{proof}




\subsection{Compositional SNE-checking problems}

We now study the same problem, but where the strategy profile of the players is described \emph{compositionally}, that is, with one machine per player.
In many cases, that description is more succinct: it is therefore not surprising that the complexity is higher in the case of MVP games.
Interestingly, it is not the case in MV$\omega$R, where we can use the same algorithm as before.



    \subsubsection{In MV\texorpdfstring{$\omega$}{ω}R games}

\begin{thm} \label{thm:compCheckingMVoR}
    In MV$\omega$R games, the compositional SNE-checking problem is $\PSpace$-complete, even when the Mealy machines are deterministic.
\end{thm}

\begin{proof}
    \begin{itemize}
        \item \emph{Easiness.}

        Given a machine profile $(\Mach_i)_{i \in \Pi}$, let us consider the product machine $\Mach$ whose state space is the product of the $\Mach_i$'s state spaces, and whose transitions are naturally defined in order to have $\Comp(\Mach) = \prod_{i \in \Pi} \Comp(\Mach_i)$.

        Then, deciding the compositional SNE-checking problem on the input $\Game_{\|v_0}, (\Mach_i)_i$ is equivalent to decide the SNE-checking problem on the input $\Game_{\|v_0}, \prod_i \Mach_i$.
        That can be done using the same algorithm that was presented in the proof of Theorem~\ref{thm:SNEcheckingMVoR}, which does not require the effective construction of $\Game_{\|v_0} \otimes \Mach$, nor the construction of $\Mach$ itself.


        \item \emph{Hardness.}

        The proof of hardness that was given in the proof of Theorem~\ref{thm:SNEcheckingMVoR} is still functional, provided that the Mealy machine $\Mach$ is replace by a family of (deterministic) machines $\Mach_1, \dots, \Mach_n$ (which all go to the vertex $\btd$) and an arbitrary one-state deterministic machine $\Mach_\SS$.
    \end{itemize}
\end{proof}



    \subsubsection{In MVP games}

In MVP games, the situation is quite similar: the complexity that was brought by the multiplicity of automata in MV$\omega$R games is now imposed by the Mealy machines.

\begin{thm}
    In MVP games, the compositional SNE-checking problem is $\PSpace$-complete, even when the Mealy machines are deterministic.
\end{thm}

\begin{proof}
    \begin{itemize}
        \item \emph{Easiness.}

        Every MVP game is an MV$\omega$R game (with one-state parity automata), hence the $\PSpace$-easiness is an immediate consequence of Theorem~\ref{thm:compCheckingMVoR}.

        \item \emph{Hardness.}

        We proceed, once again, by reduction from the emptiness problem of the intersection of $n$ deterministic finite automata.
        Let $\auto_1, \dots, \auto_n$ be $n$ such automata on the alphabet $\{a, b\}$.

        Let $\Game_{\|a}$ be the game depicted by Figure~\ref{fig:compParity_checking_hardness_arena}.
        The players are Solver, controlling the round vertices, and $1, \dots, n$, controlling the square vertices (the player controlling each square vertex is indicated in its bottom right corner).
        All the player have only two possible payoffs, $0$ and $1$ --- we will therefore use the words \emph{lose} and \emph{win}.
        The color mappings $\kappa_{11}, \dots, \kappa_{n1}, \kappa_{\SS 1}$ are defined so that Solver wins if and only if the vertex $\bt$ is reached, and each number player wins if and only if the vertex $\bt$ is \emph{not} reached.
        

        \begin{figure}
    \centering

\begin{subcaptionblock}{0.9\textwidth}
    \centering
    \begin{tikzpicture}[node distance=2cm]
        \node[state, initial, initial above] (a) at (0,0) {$a$};
        \node[state, right of=a] (b) {$b$};
        \node[literalState=$1$,below of=b] (1) {$1$};
        \node[literalState=$2$,right of=1] (2) {$2$};
        \node[right of=2] (dots) {$\cdots$};
        \node[literalState=$n$,right of=dots] (n) {$n$};
        \node[nobodyState, right of=n] (bt) {$\bt$};
        \node[nobodyState,below of=dots] (btd) {$\btd$};
\begin{pgfonlayer}{arrows}
        \path[->] (1) edge (2);
        \path[->] (2) edge (dots);
        \path[->] (dots) edge (n);
        \path[->] (n) edge (bt);
        \path[->] (a) edge[bend right] (b);
        \path[->] (b) edge[bend right] (a);
        \path[->] (a) edge[bend right] (1);
        \path[->] (b) edge (1);
        \path[->] (a) edge[loop left] (a);
        \path[->] (b) edge[loop right] (b);
        \path[->] (1) edge[bend right] (btd);
        \path[->] (2) edge[bend right, in=150] (btd);
        \path[->] (n) edge[bend left] (btd);
        \path[->] (btd) edge[loop below] (btd);
        \path[->] (n) edge (bt);
        \path[->] (bt) edge[loop right] (bt);
        \end{pgfonlayer}
    \end{tikzpicture}
    \caption{The arena.}
    \label{fig:compParity_checking_hardness_arena}
    \end{subcaptionblock}

    
    \begin{subcaptionblock}{0.35\textwidth}
    \centering
    \begin{tikzpicture}[auto,node distance=3cm]
        \node[automatonState,initial] (init) at (0,0) {$1$};
        \path[->] (init) edge[loop above] node{$a|a, b|b, *$} (init);
    \end{tikzpicture}
    \caption{The machine $\Mach_{\SS}$.}
    \label{fig:compParity_checking_hardness_solver}
    \end{subcaptionblock}
    
    
    \begin{subcaptionblock}{0.7\textwidth}
    \centering
    \begin{tikzpicture}[auto,node distance=3cm]
        \node[automatonState,rectangle,rounded corners=7pt,dotted,minimum size=3cm,initial] (autom) {$\auto_{i}$};
        \node[automatonState,double] (qacc) at (1, 1) {\phantom{b}};
        \node[automatonState] (someq) at (1, -1) {\phantom{b}};
        \node[automatonState,right of=qacc] (1) {\phantom{b}};
        \node[right of=1] (dots) {$\dots$};
        \node[automatonState,right of=dots] (i) {\phantom{b}};
        \node[automatonState,right of=someq] (1b) {\phantom{b}};
        \node[right of=1b] (dotsb) {$\dots$};
        \node[automatonState,right of=dotsb] (ib) {\phantom{b}};
        
        
        \path[->] (qacc) edge node{$1$} (1);
        \path[->] (1) edge node{$2$} (dots);
        \path[->] (dots) edge node{$i|i+1$} (i);
        \path[->] (i) edge[loop right] node{$*$} (i);
        \path[->] (someq) edge node{$1$} (1b);
        \path[->] (1b) edge node{$2$} (dotsb);
        \path[->] (dotsb) edge node{$i|\btd$} (ib);
        \path[->] (ib) edge[loop right] node{$*$} (ib);
    \end{tikzpicture}
    \caption{The machine $\Mach_i$ for player $i \in \{1, \dots, n\}$}
    \label{fig:compParity_checking_hardness_i}
    \end{subcaptionblock}

    \caption{Encoding of the intersection emptiness problem into a compositional MV$\omega$R SNE-checking problem.}
    \label{fig:compParity_checking_hardness}
\end{figure}


    Now, the deterministic Mealy machine $\Mach_\SS$ is depicted by Figure~\ref{fig:compParity_checking_hardness_solver}: it captures a strategy that consists in looping on the vertex $a$ forever.
    Similarly, for each player $i \in \{1, \dots, n\}$, the Mealy machine $\Mach_i$ is depicted by Figure~\ref{fig:compParity_checking_hardness_i} (when $i=n$, the reader should identify $i+1$ with $\bt$).
    It captures a strategy that consists in always going to the vertex $\btd$, except if the word constructed by the actions of Solver was a word recognized by the automaton $\auto_i$.

    Those Mealy machines define a strategy profile $\bsigma$.
    Let us prove that $\bsigma$ is an SNE if and only if the intersection $\bigcap_i \Lang(\auto_i)$ is empty.

    \begin{itemize}
        \item \emph{If $\bsigma$ is not an SNE.}

        Then, some coalition has a profitable deviation: since the only player who does not win the play $\< \bsigma \>$ is Solver, that coalition must include Solver; and since a play won by Solver is necessarily a play lost by all the other players, it can actually only be the singleton $\{\SS\}$.

        There is, then, a play $\pi$ that is compatible with the strategy profile $\bsigma_{-\SS}$, and that is won by Solver: that play has necessarily the form $w12\dots n \bt^\omega$, where $w \in \{a, b\}^*$.
        Moreover, for that play to be compatible with each strategy $\sigma_i$, the word $w$ must be accepted by the automaton $\auto_i$.
        Then, the intersection $\bigcap_i \Lang(\auto_i)$ is nonempty.


        \item \emph{If the intersection $\bigcap_i \Lang(\auto_i)$ is nonempty.}

        Then, let $w \in \bigcap_i \Lang(\auto_i)$: the play $\pi = w 12 \dots n \bt^\omega$ is compatible with the strategy profile $\bsigma_{-\SS}$ and won by Solver, hence the coalition $\{\SS\}$ has a profitable deviation. \qedhere
    \end{itemize}
    \end{itemize}
\end{proof}



    

\subsection{Fixed-payoff SNE existence problem}

We now switch to the fixed-payoff SNE existence problem.
Unsurprisingly, that problem is often harder to solve: while the SNE-checking problems amounted to search for a profitable deviation, that problem consists in searching for a strategy profile that admit \emph{no} such deviation.


        \subsubsection{A tool: the deviator game}

Instead of the product game, we need a new tool to solve that problem: it will take the form of a new game structure, in which one player, \emph{Prover}, tries to prove that an SNE generating the desired payoff exists, while another one, \emph{Challenger}, tries to prove that the strategy profile she constructs is actualy not an SNE.
That game is the \emph{deviator game}, very similar to a construction with the same name proposed in~\cite{DBLP:conf/fossacs/Brenguier16}, in a slightly different context.

\begin{defi}[Deviator game]
    Let $\Game_{\|v_0}$ be a graph game, and let $\bx$ be a payoff vector.
    The \emph{deviator game} is the initialized graph game:
    $$\ConDev_{\bx} \Game_{\|v_0} = \left( \{\PP, \CC\}, V^\cd, E^\cd, \left(V^\cd_\PP, V^\cd_\CC\right), \mu^\cd\right)_{\|v_0^\cd},$$
    where:

     \begin{itemize}
         \item the player $\PP$ is called \emph{Prover}, and the player $\CC$ \emph{Challenger}.

         \item Prover controls the set $V^\cd_\PP = V \times 2^\Pi$, and Challenger the set $V^\cd_\CC = E \times 2^\Pi$.

         \item The initial vertex is $v_0^\cd = (v_0, \emptyset)$.

         \item The edge set $E^\cd$ is defined as follows: from the vertex $(u, D)$, Prover can go to every vertex of the form $(uv, D) \in E$ (she \emph{proposes} the edge $uv$).
         From the vertex $(uv, D)$, Challenger can go to the vertex $(v, D)$ (he \emph{accepts} the edge $uv$), or to every vertex $(w, D \cup \{i\})$, with $w \neq v$ and $uw \in E$, and where $i$ is the player controlling $u$ (he \emph{deviates} from Prover's proposal).

         \item Given a play $\chi$ is this game, we write $\dchi$ the play in $\Game$ constructed by the actions of Prover and Challenger: if $\chi = (u_0, D_0)(u_0v_0, D_0)(u_1, D_1) (u_1v_1, D_1) \dots$, then we define $\dchi = u_0 u_1 \dots$.
         We also define $\D(\chi) = \bigcup_k D_k$, the set of players who deviated along the play $\chi$.

         \item Then, $\mu^\cd$ is the Boolean payoff function defined as follows. A play $\chi$ is won by Challenger if and only if either:
         \begin{itemize}
             \item we have $\D(\chi) = \emptyset$ and $\mu(\dchi) \neq \bx$;

             \item or for every player $i \in \D(\chi)$, we have $\mu_i(\dchi) \geq x_i$, and there exists a player $j \in \Pi$ such that $\mu_j(\dchi) > x_j$.
         \end{itemize}
     \end{itemize}
\end{defi}

\Ma{BLABLA (explication du "non-reset")}

\begin{thm} \label{thm_condev}
    Prover has a winning strategy in the game $\ConDev_{\bx} \Game_{\|v_0}$ if and only if there exists an SNE $\bsigma$ in $\Game_{\|v_0}$ with $\mu\< \bsigma \> = \bx$.
\end{thm}

\Le{Est-ce qu'il faut une preuve pour ça ?}


        \subsubsection{In MVP games}

Let us first consider the case of MVP games: then, similarly to what was done in~\cite{DBLP:conf/fossacs/Brenguier16}, a cautious way to solve the deviator game leads to an algorithm that uses only polynomial space.

\begin{thm}\label{thm:sneExistencePspaceEasy}
    In MVP games, the fixed-payoff SNE existence problem is $\PSpace$-complete.
\end{thm}

\begin{proof}
    \begin{itemize}
        \item \emph{Easiness.}
    
    By Theorem~\ref{thm_condev}, deciding the fixed-payoff SNE existence problem amounts to deciding which player, among Prover and Challenger, has a winning strategy in the corresponding deviator game.
    That game has an exponential size, but has a specific shape that makes it possible to solve it region by region, without using exponential space.

    Indeed, let us define recursively an algorithm that decides, given $\Game_{\|v_0}$, $\bx$ and a vertex $(u_0, D)$ of the game $\ConDev_{\bx} \Game$, whether Prover has a winning strategy from that vertex.
    First, construct the game $\Gameb^D_{\|(u_0, D)}$ as follows: construct the region of $\ConDev_{\bx} \Game$ that is made of vertices of the form $(u, D)$ or $(uv, D)$.
    Define on that region the color mappings so that player $i$'s payoff, in that region, is always equal to their payoff in the corresponding play in $\Game$, plus $1$: i.e., for all $i \in \Pi$ and $j \in \{1, \dots, p, p+1, p+2\}$, define $\kappa'_{ij}(uv, D) = m$, and $\kappa'_{ij}(u, D) = \kappa_{i(j-1)}(u)$, or $1$ if $j=1$ or $p+2$.
    
    For each edge $(uv, D)(w, D \cup \{i\})$ that leaves that region, add to the constructed game the edge $(uv, D)(w, D \cup \{i\})$ and the loop $(w, D \cup \{i\})(w, D \cup \{i\})$, and decide recursively whether Prover has a winning strategy from the vertex $(w, D \cup \{i\})$.
    If she does, call the vertex $(w, D \cup \{i\})$ a \emph{Prover's leaf}, and define the color mappings so that player $i'$'s payoff, on that loop, is equal to $0$: for each $i' \in \Pi$ and every $j > 0$, define $\kappa'_{i'j}(w, D \cup \{i\}) = 1$.
    If she does not, call the vertex $(w, D \cup \{i\})$ a \emph{Challenger's leaf}, and define the color mappings so that player $i'$'s payoff, on that loop, is equal to $p+1$: for each $i'$, define $\kappa'_{i'(p+2)}(w, D \cup \{i\}) = 2$ (the color $\kappa'_{i'j}(w, D \cup \{i\})$ can be defined arbitrarily for any other $j$).
    
    Now, define the (Boolean) payoff functions as follows.
    If $D \neq \emptyset$, then a play $\pi$ is won by Challenger if and only if:
    $$\pi \in \left( \bigcup_{i \in \Pi} \bigcup_{j > x_i+1} \Parity(\kappa'_{ij}) \right) \cap \left( \bigcap_{i \in D} \bigcup_{j \geq x_i+1} \Parity(\kappa'_{ij}) \right)$$
    (i.e., if $\pi$ gives to at least one player $i$ a payoff greater than $x_i$, and to every player who deviated at least the same payoff as in $\bx$).
    If $D = \emptyset$, then a play $\pi$ is won by Challenger if and only if:
    $$\pi \in \bigcup_{i \in \Pi} \bigcup_{j \neq x_i+1} \Parity(\kappa'_{ij})$$
    \Ms{Cette histoire de shift n'est pas 100\% claire pour moi; j'ai changé les $x_i$ en $x_i+1$ mais il faudra sans doute revérifier (et peut être expliquer l'intuition de ce shift).}
    (i.e., if the payoff vector generated by Prover, without any deviation, is not equal to $\bx$).
    Note that in both cases, Challenger wins if he reaches a Challenger's leaf, and loses if he reaches a Prover's leaf.
    
    Prover has a winning strategy in the game $\Gameb^D_{\|(u_0, D)}$ if and only if she has a winning strategy from the vertex $(u_0, D)$ in the game $\ConDev_{\bx} \Game$.
    Indeed, if Prover has a winning strategy in $\Gameb^D_{\|(u_0, D)}$, then she can follow that strategy in $\ConDev_{\bx} \Game$.
    Then, she either stays in the region where the deviating coalition is $D$, or she reaches a vertex of the form $(w, D \cup \{i\})$ from which she has a winning strategy, that she can then follow.
    Conversely, if she has a winning strategy from $(u_0, D)$ in $\ConDev_{\bx} \Game$, she can follow it in $\Gameb^D_{\|(u_0, D)}$: she will then either stay in the region where the deviating coalition is $D$, or reach a Prover's leaf (since the strategy she is following afterwards in $\ConDev_{\bx} \Game$ is still winning), which makes her win.

    This game can be seen as an Emerson-Lei game~\cite{EmersonLei87}: Prover's and Challenger's winning conditions are Boolean combinations of Büchi conditions.
    Indeed, if $\B(v^\cd)$ denotes, for each vertex $v^\cd$, the set of plays that visit infinitely often the vertex $v^\cd$, then we have the equality:
    $$\Parity(\kappa'_{ij}) = \bigcup_{2k < m} \left(\bigcup_{\kappa'_{ij}(v^\cd) = 2k} \B(v^\cd) \cap \neg \bigcup_{\l < 2k} \bigcup_{\kappa'_{ij}(w^\cd) = \l} \B(w^\cd)\right).$$
    It was shown in~\cite{HunterDawar05} that such games can be solved using a space polynomial in the size of the game and of the objectives.
    Here, both are themselves polynomial in the size of $\Game$.
    Thus, the last step of our recursive algorithm consists in solving $\Gameb^D_{\|(u_0, D)}$.

    Then, applying this recursive algorithm from the vertex $(v_0, \emptyset)$ solves our problem: there is an SNE $\bsigma$ in $\Game_{\|v_0}$ such that $\mu\< \bsigma \> = \bx$ if and only if Prover has a winning strategy from that vertex.
    Moreover, that algorithm uses polynomial space: each recursive call does, and the recursion stack has size at most $\card \Pi$, i.e. polynomial.
    Therefore, the fixed-payoff SNE existence problem in MVP games is $\PSpace$-easy.



        \item \emph{Hardness.}

        We reduce the Quantified Satisfaction Problem (QSAT).
    Let \[\varphi=\exists x_1 \forall x_2  \cdots \exists x_{n-1} \forall x_n \bigwedge_{i=1}^p \bigvee_{j=1}^{m_i} L_{i,j}\] be an instance of QSAT in conjunctive normal form where for all $i,j$, $L_{i,j}$ is a literal of the form $x_k$ or $\neg x_k$ for some $k\in\{1,\dots,n\}$.
    We write $\psi(x_1,\dots,x_n)=\bigwedge_{i=1}^p \bigvee_{j=1}^{m_i} L_{i,j}$ the non-quantified part of the formula.
    \medskip
    
    We construct a game with $2n+2$ players: one for each literal and two extra players $\solver$ (solver) and $\opponent$ (opponent) as depicted in \figurename~\ref{fig:qsat2sneGame}.
    Round states belong to $\solver$, hexagonal states belong to $\opponent$, rectangular states belong to the literal indicated in the bottom right corner (if any), some states only have a single outgoing edge and therefore could belong to anyone without loss of generality.
    Red clouds indicate the list of players for which a given state is in the co-B\"uchi set: infinitely many visits to these states means losing (also written as obtaining payoff $0$) while only finitely many visits means winning (payoff $1$).
    
    It is composed of three parts: in the first part, the \emph{setting} module, a valuation can be chosen by visiting $x_i$ (setting $x_i=\top$) or $\neg x_i$ (setting $x_i=\bot$), the choice belonging to $\solver$ if $x_i$ is existentially quantified and to $\opponent$ if it is universally quantified.
    When the value of a variable is chosen, the corresponding literal player can choose to go to a sink state $\blacktriangledown$ (duplicated in the figure for clarity) where player $\solver$ loses as it belongs to the co-B\"uchi set for this player.
    
    If that does not happen then the game moves into the second part, the \emph{checking} module, where the formula is ``checked'': each disjunctive clause $C_i$ has a state owned by $\solver$ who must choose a literal $L_{i,j}$ from the clause.
    State $L_{i,j}$ is in the co-B\"uchi set of the player $\neg L_{i,j}$, and would lose if said state was visited infinitely often.
    When this ``checking'' is done, the last part, called \emph{punishing} module, visits the co-B\"uchi set of one literal per variable, the choice of which being left to $\solver$.

    The game continues back to the checking module.
    As the last state of these modules is in the co-B\"uchi set of $\opponent$, it will lose if the game enters these modules.
    Also remark that, dually, if the game enters the checking module then no state of the co-B\"uchi set for $\solver$ can be reached, so it will win.
    \medskip

    We will show that when $\varphi$ holds, there can be no SNE with payoff vector $(1,\dots,1,0,1)$ as a coalition made of $\solver$ and all true literals can deviate to make $\solver$ win while not penalizing the other players in the coalition.
    \medskip

    First, assume $\varphi$ does not hold.
    Let $\bsigma$ be the following profile of strategies: each literal goes to $\blacktriangledown$ whenever possible in the setting module, $\solver$ plays any strategy, and $\opponent$ plays the optimal strategy in response to $\solver$'s choice of valuation so that $\psi(x_1,\dots,x_n)$ is false.
    The outcome of this profile is either path $?x_1\cdot x_1^s \cdot\blacktriangledown^\omega$ or $?x_1\cdot\neg x_1^s\cdot\blacktriangledown^\omega$, both with payoff vector $(1,\dots,1,0,1)$ as only $\solver$ loses.
    
    Let's prove that it is an SNE.
    Let $C$ be a coalition of players and assume that there exists a profitable deviation for this coalition.
    If $\solver\notin C$, then no one in the coalition can improve their payoff, so no deviation can be profitable.
    Therefore $\solver\in C$.
    And since it is the player with a strict increase of payoff, that means that to be profitable for the coalition, any deviation must make $\solver$ win, so it must reach the checking module.
    Because that means that $\opponent$ would then lose, $\opponent$ cannot be in the coalition.
    For each variable $x_i$, players $x_i$ and $\neg x_i$ cannot be both in the coalition as (at least) one of them loses through the infinite visits in the punishing module.
    To actually reach the checking module, all literal players whose state was visited in the setting module must have deviated from $\bsigma$, therefore are in the coalition.
    As a result the coalition is made of $\solver$ and exactly one literal per variable, defining a valuation.
    Because $\opponent$ played optimally, that valuation does not satisfy $\psi(x_1,\dots,x_n)$, so there is a clause $C_i$ where all literals $L_{i,1}, \dots, L_{i,m_i}$ are false, meaning that the player corresponding to their negation are all in the coalition.
    The choice by $\solver$ of any of these literals therefore enforces a visit to the co-B\"uchi set of (at least) one player in the coalition.
    As this choice is infinitely repeated, that makes this player lose and the deviation is not profitable.
    So $\bsigma$ is an SNE.
    \medskip

    Now assume that $\varphi$ holds.
    Let $\bsigma$ be a strategy profile with payoff $(1,\dots,1,0,1)$.
    As noted above, that payoff requires the outcome of $\bsigma$ to end in the $\blacktriangledown$ state.
    Consider the following strategy for $\solver$: in the setting module, choose the literal that ensures satisfaction of $\psi(x_1,\dots,x_n)$, based on the already known choices of $\opponent$.
    This is possible since $\varphi$ holds.
    Let $C$ be the coalition made of $\solver$ and all literal players corresponding to states $x_i^s$ or $\neg x_i^s$ visited in the setting module.
    These players deviate by reaching state $?x_{i+1}$ (or $C_1$ if $i=n$) instead of going to $\blacktriangledown$.
    The valuation thus built ensures that $\psi(x_1,\dots,x_n)$ is satisfied, so in the checking module, for every clause there is a true literal.
    The strategy of $\solver$ consists in consistently choosing the state for these literals.
    Note that that means visiting a co-B\"uchi set for a player that is not in the coalition.
    In the punishing module, $\solver$ visits states corresponding to players in the coalition (i.e. the exact same one that were visited in the setting module: if $x_i^s$ was visited, consistently choose $x_i^p$, if $\neg x_i^s$ was visited, consistently choose $\neg x_i^p$.
    This ensures that the co-B\"uchi set of no player in the coalition $C$ is ever visited, hence all players in this coalition win, including $\solver$, therefore the deviation is profitable and $\bsigma$ is not an SNE.
\begin{figure}
    \centering
    \begin{tikzpicture}[node distance=50pt]
        % Setting the valuation
        \node[solverState,initial] at (0,0) (q1) {$?x_1$};
        \node[literalState=$x_1$,above right of=q1] (p1) {$x_1^s$};
        \node[literalState=$\neg x_1$,below right of=q1] (n1) {$\neg x_1^s$};
        \node[opponentState,below right of=p1] (q2) {$?x_2$};
        \node[literalState=$x_2$,above right of=q2] (p2) {$x_2^s$};
        \node[literalState=$\neg x_2$,below right of=q2] (n2) {$\neg x_2^s$};
        \node[below right of=p2] (q3) {$\cdots$};
        \node[literalState=$x_n$,above right of=q3] (pn) {$x_n^s$};
        \node[literalState=$\neg x_n$,below right of=q3] (nn) {$\neg x_n^s$};

        % Checking all the clauses
        \node[solverState,below right of=pn] (c1) {$C_1$};
        \node[nobodyState,above right of=c1] (l11) {$L_{1,1}$}; \cobuchiLabel[inner sep=0pt,cloud puff arc=95]{l11}{$\neg L_{1,1}$}
        \node[nobodyState,below right of=c1] (l1m1) {$L_{1,m_1}$};  \cobuchiLabel[inner sep=0pt,cloud puff arc=95]{l1m1}{$\neg L_{1,m_1}$}
        \node (c1dots) at (barycentric cs:l11=1,l1m1=1) {$\myvdots$};
        \node[solverState,below right of=l11] (c2) {$C_2$};
        \node[above right of=c2] (l21) {$\myiddots$};
        \node[below right of=c2] (l2m2) {$\myddots$};
        \node (c2dots) at (barycentric cs:l21=1,l2m2=1) {$\myvdots$};
        \node[right of=l21,node distance=2.5cm] (lp1) {$\myddots$};
        \node[right of=l2m2,node distance=2.5cm] (lpmp) {$\myiddots$};
        \node (cpdots) at (barycentric cs:lp1=1,lpmp=1) {$\myvdots$};
        \node[yshift=7pt] (ldots1) at (barycentric cs:l21=1,lp1=1) {$\cdots$};
        \node[yshift=-7pt] (ldotsm) at (barycentric cs:l2m2=1,lpmp=1) {$\cdots$};
        \node (ldots) at (barycentric cs:ldots1=1,ldotsm=1) {$\cdots$};
        \node[nobodyState,below right of=lp1] (ph) {};

        % Punition of literals
        \node[solverState,below of=ph,node distance=4cm] (v1) {$x_1?$};
        \node[nobodyState,above left of=v1] (vp1) {$x_1^p$}; \cobuchiLabel{vp1}{$\neg x_1$}
        \node[nobodyState,below left of=v1] (vn1) {$\neg x_1^p$}; \cobuchiLabel{vn1}{$x_1$}
        \node[solverState,below left of=vp1] (v2) {$x_2?$};
        \node[nobodyState,above left of=v2] (vp2) {$x_2^p$}; \cobuchiLabel{vp2}{$\neg x_2$}
        \node[nobodyState,below left of=v2] (vn2) {$\neg x_2^p$}; \cobuchiLabel{vn2}{$x_2$}
        \node[below left of=vp2] (vn) {$\cdots$};
        \node[nobodyState,above left of=vn] (vpn) {$x_n^p$};  \cobuchiLabel{vpn}{$\neg x_n$}
        \node[nobodyState,below left of=vn] (vnn) {$\neg x_n^p$}; \cobuchiLabel{vnn}{$x_n$}
        \node[nobodyState,below left of=vpn] (ph2) {}; \cobuchiLabelLeft{ph2}{$\opponent$}

        % Sink state
        \node[nobodyState,above of=p2] (sinkTop) {$\blacktriangledown$}; \cobuchiLabelTop{sinkTop}{$\solver$}
        \node[nobodyState,below of=n2] (sinkBot) {$\blacktriangledown$}; \cobuchiLabelBot{sinkBot}{$\solver$}

        \begin{pgfonlayer}{arrows}
            \path[->] (q1) edge (p1) edge (n1);
            \path[->] (p1) edge (q2) edge[bend left,out=-30] (sinkTop);
            \path[->] (n1) edge (q2) edge[bend right,out=30] (sinkBot);
            \path[->] (q2) edge (p2) edge (n2);
            \path[->] (p2) edge (q3) edge (sinkTop);
            \path[->] (n2) edge (q3) edge (sinkBot);
            \path[->] (q3) edge (pn) edge (nn);
            \path[->] (pn) edge (c1) edge[bend right,out=30] (sinkTop);
            \path[->] (nn) edge (c1) edge[bend left,out=-30] (sinkBot);
    
            \path[->] (c1) edge (l11) edge (c1dots) edge (l1m1);
            \path[<-] (c2) edge (l11) edge (c1dots) edge (l1m1);
            \path[->] (c2) edge (l21) edge (c2dots) edge (l2m2);
            \path[<-] (ph) edge (lp1) edge (cpdots) edge (lpmp);

            \path[->] (ph) edge (v1);

            \path[->] (v1) edge (vp1) edge (vn1);
            \path[<-] (v2) edge (vp1) edge (vn1);
            \path[->] (v2) edge (vp2) edge (vn2);
            \path[<-] (vn) edge (vp2) edge (vn2);
            \path[->] (vn) edge (vpn) edge (vnn);
            \path[<-] (ph2) edge (vpn) edge (vnn);

            \path[->] (ph2) edge (c1);
    
            \path[->] (sinkTop) edge[loop above] (sinkTop);
            \path[->] (sinkBot) edge[loop below] (sinkBot);
            \end{pgfonlayer}
    \end{tikzpicture}
    \caption{Game to encode QSAT  instance $\exists x_1 \forall x_2  \cdots \exists x_{n-1} \forall x_n \bigwedge_{i=1}^p \bigvee_{j=1}^{m_i} L_{i,j}$ into the existence of an SNE with payoff $(1,\dots,1,0,1)$. Round states belong to $\solver$, hexagonal states belong to $\opponent$, rectangular states belong to the literal indicated in the bottom right corner (if any). The red cloud lists the set of players for which this state is in the co-B\"uchi condition.}
    \label{fig:qsat2sneGame}
\end{figure}
\end{itemize}
\end{proof}




\subsubsection{In MV\texorpdfstring{$\omega$}{ω}R games}

When the payoff functions are defined by parity automata, those ones must be incorporated in the arena of the game, entailing an exponential blowup.
However, there is no exponential blowup in the formula that defines the winning conditions of Prover and Challenger, hence the game can be solved by using algorithms that exists in the literature, in exponential time.

% \begin{thm}
%     The fixed-payoff SNE existence problem for multi-valued $\omega$-regular games is in $\ExpSpace$.
% \end{thm}

% \begin{proof}
%     Let $\Game_{\|v_0}$ be an MV$\omega$R game, and let $\bx \in \NN$.
%     We first define the game $\Game^*_{\|v_0^*} = \left(\Pi, V^*, E^*, (V^*_i)_i, \mu^*\right)$ as follows:
%     \begin{itemize}
%         \item the players are the same as in $\Game$;

%         \item the vertex set controlled by each player $i$ is $V^*_i = V_i \times \prod_{i \in \Pi} \prod_{j = 1}^p Q_i$;

%         \item from each vertex $(u, (s_{ij})_{i,j}) \in V^*$ and every edge $uv \in E$, the set $E^*$ contains the edge $(u, (s_{ij})_{i, j})(v, (t_{ij})_{i,j})$ where for each $i$ and $j$, we have $T_{ij}(s_{ij}, u) = t_{ij}$;

%         \item the payoff function $\mu^*$ is the MVP payoff function defined by the color mappings $\kappa^*_{ij}: (u, (s_{i'j'})_{i'j'}) \mapsto \kappa_{ij}(s_{ij})$;

%         \item the initial vertex is $v_0^* = (v_0, (s_{ij0})_{i,j})$.
%     \end{itemize}
    
%     In other words, the game $\Game^*_{\|v_0^*}$ is the game $\Game_{\|v_0}$, where the automata have been incorporated in the vertex set, which makes it an MVP game.
%     By construction, there is an SNE with payoff vector $\bx$ in $\Game_{\|v_0}$ if and only if there is one in $\Game^*_{\|v_0^*}$.
%     According to Theorem~\ref{thm:sneExistencePspaceEasy}, that can be decided using a space that is polynomial in the size of $\Game^*_{\|v_0^*}$, i.e. exponential in the size of $\Game_{\|v_0}$.
% \end{proof}

\begin{thm}
    In MV$\omega$R games, the fixed-payoff SNE existence problem is $\ExpTime$-complete.
\end{thm}

\begin{proof}
    \begin{itemize}
        \item \emph{Easiness.}

    % A \emph{multi-valued $\omega$-regular game}, or \emph{MV$\omega$R game} for short, is a multi-player game $\Game_{\|v_0}$ such that there exists two integers $p$ and $m$, and for each player $i$, $p$ parity automata $\auto_{i1},\dots,\auto_{ip}$ over alphabet $V$, such that  for each play $\pi$, we have $\mu_i(\pi) = \max\{j ~|~ \pi \in \Lang(\auto_{ij})\}$ (with the convention $\max\emptyset = 0$).
Let $\Game_{\|v_0}$ be an MV$\omega$R game, and let $\bx \in \NN$.
Let $\left(\auto_{ij}\right)_{i\in\Pi, 1\leq j\leq p}$ be the parity automata defining the payoff over $\Game_{\|v_0}$.
Let $S_{ij}$ (resp. $T_{ij}$, $\kappa_{ij}$) be the set of states (resp. transition function, coloring mapping) of $\auto_{ij}$.
We assume all these automata use at most $k$ priorities, i.e. the co-domain of every $\kappa_{ij}$ is included in $\{0,\dots,k\}$.
We identify $\Pi$ with the set $\{1,\dots,n\}$ for simplicity in this proof.
Let \[m=\max\left(2,|V|,\max_{\substack{i\in\Pi\\1\leq j\leq p}}\left|Q_{ij}\right|\right)\] be the maximal size of the graph/automata provided as input (assumed to be at least 2 for complexity purposes).

We build the Extended Deviator Game as the product of the Deviator Game with all automata $\auto_{ij}$.
Formally:
    The \emph{extended deviator game} is the initialized graph game:
    \[\EConDev_{\bx} \Game_{\|v_0} = \left( \{\PP, \CC\}, V^\ecd, E^\ecd, \left(V^\ecd_\PP, V^\ecd_\CC\right), \mu^\ecd\right)_{\|v_0^\ecd},\]
    where:

     \begin{itemize}
         \item the player $\PP$ is called \emph{Prover}, and the player $\CC$ \emph{Challenger}.

         \item Prover controls the set $V^\ecd_\PP$ and Challenger the set $V^\ecd_\CC$ with
         \begin{mathpar}
             V^\ecd_\PP = V \times 2^\Pi \times \prod_{\substack{i\in\Pi\\1\leq j\leq p}} Q_{ij}
             \and\text{and}\and
             V^\ecd_\CC= E \times 2^\Pi \times \prod_{\substack{i\in\Pi\\1\leq j\leq p}} Q_{ij}
         \end{mathpar}
         \Ms{Le choix de $\Pi$ pour les players n'est pas très heureux quand on a des produits\dots}
         In the sequel we write $\bs=s_{11},\dots,s_{np}$ for elements of $\prod_{\substack{i\in\Pi\\1\leq j\leq p}} Q_{ij}$.

         \item The initial vertex is $v_0^\ecd = (v_0, \emptyset, s_{0,11},\dots,s_{0,np})=(v_0,\emptyset,\bs_0)$.

         \item The edge set $E^\ecd$ is defined as follows: from the vertex $(u, D, s_{11},\dots, s_{np})$, Prover can go to every vertex of the form $(uv, D, s_{11},\dots, s_{np})$ with $uv \in E$ (she \emph{proposes} the edge $uv$).
         From the vertex $(uv, D, s_{11},\dots, s_{np})$, Challenger can go to the vertex $(v, D, s_{11}',\dots, s_{np}')$ where $s_{ij}'=T_{ij}(s_{ij},v)$ (he \emph{accepts} the edge $uv$), or to every vertex $(w, D \cup \{\eta\}, s_{11}',\dots, s_{np}')$, with $w \neq v$, $uw \in E$, and $s_{ij}'=T_{ij}(s_{ij},w)$, and where $\eta$ is the player controlling $u$ (he \emph{deviates} from Prover's proposal).
         
         \item We define the coloring functions $\kappa'_{ij}$ for $i\in \Pi$ and $1\leq j\leq p$ as $\kappa'_{ij}(u, D, s_{11},\dots, s_{np})=\kappa_{i,j}(s_{ij})$ and $\kappa'_{ij}(uv, D, s_{11},\dots, s_{np})=k+1$ (thus effectively ignoring proposition vertices).

         \item Given a play $\chi=(u_0, D_0, \bs_0)(u_0v_0, D_0,\bs_0)(u_1, D_1,\bs_1) (u_1v_1, D_1,\bs_1)\dots$ is this game, we write $\D(\chi) = \bigcup_k D_k$, the set of players who deviated along the play $\chi$.
         % $\hchi$ the play in $\Game$ constructed by the actions of Prover and Challenger: if $\chi =  \dots$, then we define $\dchi = u_0 u_1 \dots$.

         \item Then, $\mu^\ecd$ is the Boolean payoff function defined as follows. A play $\chi$ is won by Challenger if and only if either:
    If $D(\chi) \neq \emptyset$, then a play $\chi$ is won by Challenger if and only if:
    \[\chi \in \left( \bigcup_{i \in \Pi} \bigcup_{j > x_i} \Parity(\kappa'_{ij}) \right) \cap \left( \bigcap_{i \in D(\chi)} \bigcup_{j \geq x_i} \Parity(\kappa'_{ij}) \right)\]
    (i.e., if $\chi$ gives to at least one player $i$ a payoff greater than $x_i$, and to every player who deviated at least the same payoff as in $\bx$).
    If $D(\chi) = \emptyset$, then a play $\chi$ is won by Challenger if and only if:
    \[\chi \in \bigcup_{i \in \Pi} \bigcup_{j \neq x_i} \Parity(\kappa'_{ij})\]
    \end{itemize}
    Note that we can convert all parity conditions into a chain of Rabin conditions: for $i\in \Pi, 1\leq j\leq p, 0\leq c \leq k$, let
    \[\Xi^{ij}_c=\left\{(u, D, s_{11},\dots, s_{np})\mmid \kappa_{ij}(s_{ij})\leq c\right\}.\]
    Then $\Parity(\kappa'_{ij})=\bigcup_{\substack{0\leq c \leq k\\c \text{ is even}}} \Inf(\Xi^{ij}_c) \cap \Fin(\Xi^{ij}_{c-1})$ is the set of runs where $\Xi^{ij}_c$ appears infinitely often and $\Xi^{ij}_{c-1}$ only finitely often for an even color $c$.
    Remark that we can (and do) ignore here the color $k+1$ added to ignore intermediate proposing vertices.
    We add an extra set \[\noDev=\left\{(u, \emptyset, \bs)\mmid u\in V, \bs \in \prod_{\substack{i\in\Pi\\1\leq j\leq p}} Q_{ij}\right\}\] that tracks whether there was a deviation.
    The winning condition for Challenger therefore become:
    \begin{mathpar}
       \left(\Fin(\noDev) \cap \left( \bigcup_{i \in \Pi} \bigcup_{j > x_i} \bigcup_{\substack{0\leq c \leq k\\c \text{ is even}}} \Inf(\Xi^{ij}_c) \cap \Fin(\Xi^{ij}_{c-1}) \right) \cap \left( \bigcap_{i \in D} \bigcup_{j \geq x_i} \bigcup_{\substack{0\leq c \leq k\\c \text{ is even}}} \Inf(\Xi^{ij}_c) \cap \Fin(\Xi^{ij}_{c-1}) \right) \right)
        \cup \left(\Inf(\noDev) \cap \bigcup_{i \in \Pi} \bigcup_{j \neq x_i} \bigcup_{\substack{0\leq c \leq k\\c \text{ is even}}} \Inf(\Xi^{ij}_c) \cap \Fin(\Xi^{ij}_{c-1})\right)
    \end{mathpar}

The extended deviator game therefore has $2\cdot m\cdot 2^n \cdot m^{n}=O(m^n)$ vertices and a winning condition that is provided by an Emerson-Lei condition with $n\cdot p\cdot k$ colors, and a formula of size polynomial in $n$, $p$, and $k$.
Solving this game with the $\PSpace$ algorithm used in the proof of Theorem~\ref{thm:sneExistencePspaceEasy} would provide an $\ExpSpace$ algorithm.
However, using the algorithm from~\cite[Corollary 24]{HausmannLehautPiterman23}, this game can be solved in $O((n\cdot p\cdot k)!\cdot (m^n)^{n\cdot p\cdot k+2})=O((n\cdot p\cdot k)!\cdot m^{n^2\cdot p\cdot k+2n})$.
As a result the fixed-payoff SNE existence problem for multi-valued $\omega$-regular games is in $\ExpTime$

    \item \emph{Hardness.}

    We reduce the problem of existence of a winning strategy for two player zero-sum games with winning condition defined by a conjunction of parity automata~\cite{?}.
    Let $\Game_{\|v_0}=(V,E)$ be a two player game for players Adam ($\adam$) and Eve ($\eve$): $V=V_\adam \uplus V_\eve$.
    Let $\auto_1,\dots,\auto_n$ be $n$ parity automata over alphabet $V$.
    A play $\pi$ is winning for $\eve$ if for $i\in \{1,\dots,n\}$, $\pi\in\Lang(\auto_i)$.

    We build the $n+2$-player game $\Game^\dagger$ that has an SNE with payoff $(1,\dots,1,1,0)$ if and only if $\adam$ has a winning strategy in $\Game$.
    The $n+2$ players are $\{1,\dots,n,\adam,\eve\}$ (used in that order for payoff description).
    The game arena consists of the original game $\Game_{\|v_0}$ with a prepended path where each player from $1$ to $n$ can either choose to continue or reach a sink state $\blacktriangledown$.
    Players $i$ gets payoff $1$ if either they win in in $\Game_{\|v_0}$ or the play ends up in $\blacktriangledown$; otherwise they get payoff $0$.
    This is ensured in $\auto^\dagger_{i1}$ by adding two states to $\auto_i$ to take into account this prefix (see \figurename~\ref{fig:conjParity2sneAutomataRegular}).
    % The automaton $\auto^\dagger_{i0}$ (not depicted), the complement of $\auto^\dagger_{i1}$, is obtained by adding $1$ to every priority.
    Player $\adam$ gets payoff $1$ if the play ends up in $\blacktriangledown$ and gets $0$ if it reaches $\Game_{\|v_0}$; the situation is opposite for $\eve$ who gets $0$ in $\blacktriangledown$ and $1$ in $\Game_{\|v_0}$.

    Assume that $\adam$ has a winning strategy in $\Game_{\|v_0}$.
    Let $\bsigma$ be the following profile in $\Game^\dagger$: for $i\in \{1,\dots,n\}$, from $q_i$ go to $\blacktriangledown$; $\adam$ plays his winning strategy in $\Game_{\|v_0}$, and $\eve$ play an arbitrary strategy.
    Since $\blacktriangledown$ is reached in the play induced by $\bsigma$, the payoff vector is $(1,\dots,1,1,0)$.
    We will show that $\bsigma$ is an SNE.

    Let $C$ be a coalition of players and assume $\bsigma'$ is a profitable deviation from players in $C$.
    First, only $\eve$ can strictly profit from a deviation (all others have reached the maximal payoff), so for the deviation to be profitable, we must have $\eve\in C$.
    In addition, if one of the players $i\in\{1,\dots,n\}$ does not effectively deviate, then the play ends up in $\blacktriangledown$ and the payoff vector does not change; therefore all of these players must be in $C$.
    On the other hand, if the play changes the payoff by not ending in $\blacktriangledown$, then $\adam$ strictly decreases his payoff so cannot be part of the coalition.
    Therefore, any profitable deviation must be from the coalition $C=\{1,\dots,n,\eve\}$.
    However, since $\adam$ has a winning strategy and plays it in $\Game_{\|v_0}$, the play is not accepted by (at least) one automaton $\auto_i$, so $i$ decreases their payoff.
    As a result the deviation $\bsigma'$ cannot be profitable, which is a contradiction, and $\bsigma$ is an SNE.

    Now assume that $\eve$ has a winning strategy in $\Game_{\|v_0}$.
    Let $\bsigma$ be a profile with payoff vector $(1,\dots,1,1,0)$.
    We will show this profile is not an SNE.
    For this payoff to occur, that means the play ends up in $\blacktriangledown$.
    Consider the coalition $C=\{1,\dots,n,\eve\}$ and the deviation (which may not be actually effective for some players) $\bsigma'$ defined as follows: for $i \in \{1,\dots,n\}$, from $q_i$ go to $q_{i+1}$ (or $v_0$ if $i=n$); $\eve$ plays optimally in $\Game_{\|v_0}$, i.e. a winning strategy.
    The play thus built will reach $\Game_{\|v_0}$ where the created play is accepted by all $\auto_i$, so the payoff for player $i$ remains $1$ while the payoff for $\eve$ strictly increases from $0$ to $1$.
    Therefore $\bsigma'$ is a profitable deviation and $\bsigma$ is not an SNE.    

    As a result there is an SNE with payoff $(1,\dots,1,1,0)$ if and only if $\adam$ has a winning strategy in $\Game_{\|v_0}$ for the winning condition $\bigcap_{i=1}^n \Lang(\auto_i)$.

\begin{figure}
    \centering
    \begin{tikzpicture}[node distance=2cm]
        \node[literalState=$1$,initial] (q1) at (0,0) {$q_1$};
        \node[literalState=$2$,right of=q1] (q2) {$q_2$};
        \node[right of=q2] (qdots) {$\cdots$};
        \node[literalState=$n$,right of=qdots] (qn) {$q_n$};
        \node[state,rectangle,rounded corners=7pt,dotted,minimum size=1.5cm,right of=qn,node distance=3cm] (orig) {$\Game_{\|v_0}$};
        \node[nobodyState,below of=qdots] (sink) {$\blacktriangledown$};
\begin{pgfonlayer}{arrows}
        \path[->] (q1) edge (q2);
        \path[->] (q2) edge (qdots);
        \path[->] (qdots) edge (qn);
        \path[->] (qn) edge (orig);
        \path[->] (q1) edge[bend right] (sink);
        \path[->] (q2) edge[bend right,in=150] (sink);
        \path[->] (qn) edge[bend left] (sink);
        \path[->] (sink) edge[loop below] (sink);
        \end{pgfonlayer}
    \end{tikzpicture}
    \caption{Game $\Game^\dagger$. The player owning the vertex is given in the bottom right corner of each state.}
    \label{fig:conjParity2sneGame}
\end{figure}

\begin{figure}
    \centering
    \begin{subcaptionblock}{0.9\textwidth}
    \centering
    \begin{tikzpicture}[auto,node distance=3cm]
        \node[automatonState,initial] (init) at (0,0) {$0$};
        \node[automatonState,below right of=init] (sink) {$1$};
        \node[automatonState,rectangle,rounded corners=7pt,dotted,minimum size=1.5cm,above right of=sink] (autom) {$\auto_{i}$};
        \path[->] (init) edge[loop above] node{$q_1,\dots,q_n,\blacktriangledown$} (autom);
        \path[->] (init) edge node{$v_0$} (autom);
        \path[->] (init) edge node[swap]{$v\in V\setminus\{v_0\}$} (sink);
        \path[->] (autom) edge node{$q_1,\dots,q_n,\blacktriangledown$} (sink);
        \path[->] (sink) edge[loop above] node{$*$} (sink);
    \end{tikzpicture}
    \caption{Parity automata $\auto^\dagger_{i1}$ for player $i$ to obtain payoff $1$. Numbers in state indicate the value of the coloring.}
    \label{fig:conjParity2sneAutomataRegular}
    \end{subcaptionblock}
    
    \begin{subcaptionblock}{0.4\textwidth}
    \centering
    \begin{tikzpicture}[auto,node distance=3cm]
        \node[automatonState,initial] (init) at (0,0) {$0$};
        \node[automatonState,right of=init] (lose) {$1$};
        \path[->] (init) edge[loop above] node{$q_1,\dots,q_n,\blacktriangledown,v\in V\setminus\{v_0\}$} (init);
        \path[->] (init) edge node{$v_0$} (lose);
        \path[->] (lose) edge[loop above] node{$*$} (lose);
    \end{tikzpicture}
    \caption{Parity automaton $\auto^\dagger_{\adam1}$.}
    \label{fig:conjParity2sneAutomataAdam}
    \end{subcaptionblock}
    \hfill
    \begin{subcaptionblock}{0.4\textwidth}
    \centering
    \begin{tikzpicture}[auto,node distance=3cm]
        \node[automatonState,initial] (init) at (0,0) {$1$};
        \node[automatonState,right of=init] (lose) {$0$};
        \path[->] (init) edge[loop above] node{$q_1,\dots,q_n,\blacktriangledown,v\in V\setminus\{v_0\}$} (init);
        \path[->] (init) edge node{$v_0$} (lose);
        \path[->] (lose) edge[loop above] node{$*$} (lose);
    \end{tikzpicture}
    \caption{Parity automaton $\auto^\dagger_{\eve1}$.}
    \label{fig:conjParity2sneAutomataEve}
    \end{subcaptionblock}

    \caption{Parity automata for payoffs in $\Game^\dagger$.}
    \label{fig:conjParity2sneAutomata}
\end{figure}

\end{itemize}
\end{proof}
% By Lemma~\ref{lem:EL2ParityGame}, we can transform the Emerson-Lei condition into a parity condition for a game of size $O(m^n\cdot2^{n\cdot p\cdot k})=2^{O(n\cdot p\cdot k\cdot \log(m))}$ with $O(n\cdot p\cdot k)$ colors.
% This game can be solved in time $\NP\cap\coNP$; as the game is exponential, that provides a procedure in $\NexpTime\cap\coNexpTime$.
% \end{proof}

% \begin{lm}\label{lem:EL2ParityGame}
%     A colored Emerson-Lei game over an arena of size $n$ with winning condition using $p$ colors can be transformed into a parity game of size $O(n\times 2^{p})$ with $O(p)$ colors.
% \end{lm}

% \begin{proof}
%     Let $\Game=(V,E)$ be a game arena with $V=V^{\playerOneSymb}\uplus V^{\playerTwoSymb}$.
%     Let $v_0\in V$ an initial vertex, $\colors=\{C_1, \dots, C_p\} \subseteq 2^V$ be a set of colors attached to vertices, and $\varphi$ a propositional formula over literals $\{\Inf(C_i),\Fin(C_i)\}$ (with the convention that $\neg\Inf(C)=\Fin(C)$).
%     By abuse of notation, for a set $K\subseteq \colors$, $\varphi(K)$ is the truth value of $\varphi$ where $\Inf(C)$ is set to $\top$ if and only if $C\in K$.
%     Given an infinite play $\chi=v_0v_1\cdots$, we define $K(\chi)$ as the set of colors appearing infinitely often in $\chi$: $C\in K(\chi)$ if and only if there exists an infinity of indices $k$ such that $v_k\in C$.
%     Player $\playerOneSymb$ wins if $\varphi(K(\chi))$ evaluates to $\top$.

%     First, the game can be expanded into $\hat{\Game}$ so that every vertex belongs to at most one set $C_i$: if $v\in C_{i_1} \cap \cdots C_{i_m}$ then replace $v$ by new vertices $v_1 \in C_{i_1}, \dots, v_m \in C_{i_m}$ (all belonging to the same player as $v$).
%     For $1\leq i < m$, add edges $(v_i,v_{i+1})$ to $E$, and replace all edges $(v',v) \in E$ by $(v',v_1)$, and $(v,v') \in E$ by $(v_m,v')$.
%     Since no new choice has been added to the game, the winning player remain the same (and strategies can be converted straightforwardly).
%     This creates an arena of size at most $|V|\cdot p$.

%     Let $\auto_{\mathrm{EL}}$ be the following automaton: the alphabet is $\colors \cup \emptyset$, the set of states is $\colors\cup \emptyset$, and the transition function is defined as $T(C,C')=C'$.
%     The initial state is the set $C$ such that $v_0\in C$ (or $\emptyset$ if $v_0$ is not colored).
%     This automaton reads a color and the state remembers the last color visited.
%     With the coloring of every state $C$ by color $C$ and Emerson-Lei condition $\varphi$, clearly automaton $\auto_{\mathrm{EL}}$ accepts sequences of colors that correspond to winning plays in $\hat{\Game}$.
    
%     We now transform $\auto_{\mathrm{EL}}$ into an equivalent parity automaton $\auto_{\mathrm{par}}$ using the Latest Acceptance Record (LAR) construction of McNaughton~\cite{McNaughton66}.
%     Recall that a state of $\auto_{\mathrm{par}}$ is of the form $(j,\pi)$ where $\pi$ is a permutation over a subset of $\colors$ (the LAR) and $j$ is the \emph{hit position}.
%     \Ms{Description reprise \href{https://www.mimuw.edu.pl/~bojan/20152016-2/jezyki-automaty-i-obliczenia-2/games-with-ω-regular-winning-conditions/from-muller-to-parity}{du site de Mikolaj Bojanczyk}, je ne sais pas si ni comment le citer.}
%     The priority of $(j,\pi)$ in $\auto_{\mathrm{par}}$ is defined as follows.
%     Let $\pi=C_{i_1}\cdots C_{i_m}$.
%     If $j<m$ then let $K=\{C_{i_{j+1}},\dots,C_{i_m}\}$; if $j=m$ then let $K=\{C_{i_m}\}$.
%     The set $K$ is the set of colors appearing in $\pi$ after having removed $j$ ``letters'' (except when $j=m$).
%     The priority of $(j,\pi)$ is:
%     \begin{itemize}
%         \item $2\cdot (j+1)$ if $\varphi(K)$ is true
%         \item $2\cdot j+1$ if $\varphi(K)$ is false
%     \end{itemize}
%     Note that each of these priorities can be evaluated in polynomial time by evaluating formula $\varphi$.
%     By construction of the LAR, if $j$ is the minimal index visited infinitely often, then letters in $K$ are visited infinitely often.
%     % IF two different sets $K,K'$ are visited infinitely often with the same hit position then there must have been a lower hit position in the middle, also visited infinitely often (intuition)
%     Note that if several states with the same hit position but different sets $K$ are visited infinitely often, that means there must be between these states a visit to a state with a lower hit position. \Ms{C'est vrai \c ca? C'est ce que je comprends mais ce n'est jamais dit clairement.}
%     As a result, a sequence of colors is accepted by $\auto_{\mathrm{par}}$ if and only if the colors visited infinitely often are winning for $\varphi$.
%     This automaton uses $O(p!)$ states and $O(p)$ priorities.

%     By taking the synchronized product of $\hat{\Game}$ with $\auto_{\mathrm{par}}$ over colors, one obtains a game arena of size $O(|V|\cdot p!)$ and parity winning condition with $O(p)$ priorities.
%     Indeed, a play in $\hat{\Game}$ generates an infinite sequence of colors.
%     If this sequence satisfies $\varphi$ it is accepted by $\auto_{\mathrm{par}}$.
%     The size of the product is $O(n\cdot2^p)$ and it uses $O(p)$ priorities.
% \end{proof}
% Note that the transformation of Lemma~\ref{lem:EL2ParityGame} combined with the $\NP\cap\coNP$ algorithm for parity games is not an improvement on the $\PSpace$ algorithm for Emerson-Lei games as it is exponential, but it provides a complexity that is exponential only in the number of colors used in the formula.



==> exchangeWithGuarantees.tex <==
% For safekeeping, maybe removed later
\paragraph{An untrusted trusted-third-party.}
        A more subtle approach need not require the third party to be trusted, but only to have its best interest to act honestly as a third party to $\alice$ and $\bob$.
        In this setting, the third party is a regular agent Charlie ($\charlie$) who has two items $g_1$ and $g_2$ that are of value only to him.
        These item are sent to $\alice$ and $\bob$, respectively, as a token of good faith, and are to be given back to $\charlie$ after the exchange of items has gone through between $\alice$ and $\bob$.
        Since these items are of no value to them, $\alice$ and $\bob$ have no incentive to keep them afterwards.
        The actions of all players are to send to any other player an item they currently have in their possession, starting with $\alice: \{\textit{item}_1\}$, $\bob: \{\textit{item}_2\}$, and $\charlie: \{g_1,g_2\}$.
        As before, both $\alice$ and $\bob$ would prefer to keep both items rather than proceed to the full exchange, but want to avoid being cheated in the symmetric manner.
        The third party $\charlie$ requires both $g_1$ and $g_2$ to be back in his possession at the end not to feel cheated, but would benefit from having $\textit{item}_1$ or $\textit{item}_2$ on top of $g_1,g_2$.
        One way to perform this exchange is thus for each agent to follow the following protocol:
        \begin{description}
            \item[For $\alice$:] Upon receiving $g_1$, send $\textit{item}_1$ to $\charlie$.
            When $\textit{item}_2$ is received, send $g_1$ to $\charlie$.
            \item[For $\bob$:] Upon receiving $g_2$, send $\textit{item}_2$ to $\charlie$.
            When $\textit{item}_1$ is received, send $g_2$ to $\charlie$.
            \item[For $\charlie$:] Send $g_1$ to $\alice$ and $g_2$ to $\bob$ (in no particular order).
            When both $\textit{item}_1$ and $\textit{item}_2$ have been received, send $\textit{item}_2$ to $\alice$ and $\textit{item}_1$ to $\bob$ (again with no particular order).
        \end{description}
        % \begin{multicols}{3}
        % \begin{enumerate}[nosep]
        %     \item $\charlie$ sends $g_1$ to $\alice$.
        %     \item $\charlie$ sends $g_2$ to $\bob$.
        %     \item $\alice$ sends 
        %     \item $\bob$ sends $\textit{item}_2$ to $\charlie$.
        %     \item $\charlie$ sends $\textit{item}_2$ to $\alice$.
        %     \item $\charlie$ sends $\textit{item}_1$ to $\bob$.
        %     \item $\alice$ sends $g_1$ to $\charlie$.
        %     \item $\bob$ sends $g_2$ to $\charlie$.
        % \end{enumerate}
        % \end{multicols}

        No agent here has a benefit from deviating from this protocol: $\charlie$ gathers both $\textit{item}_1$ and $\textit{item}_2$ before sending them to their rightful recipient so at no point $\alice$ or $\bob$ is in a position to get an unfair advantage.
        $\charlie$ has no incentive to keep any item since that would mean not getting $g_1$ or $g_2$ back.
        And there is no incentive for $\alice$ or $\bob$ to keep these as they have no value to them.
        It is also not rational for two of the agents to team up against the third:
        \begin{itemize}
            \item $\alice$ and $\bob$ have competing objectives so cannot team up together.
            \item $\alice$ and $\charlie$ teaming up together would mean one of them keeping $\textit{item}_2$ and retaining their original items.
            As that would mean that $\charlie$ never gets $g_2$ back, it is not rational for him to do so.
            \item $\bob$ and $\charlie$ cannot team up for similar reasons.
        \end{itemize}
        In fact, because there is no real advantage to be gained by teaming up, the role of $\charlie$ can even be taken up by $\alice$.
        She starts the process by sending an item $g$ to $\bob$, he can then send $\textit{item}_2$ to $\alice$, she replies with $\textit{item}_1$ and $\bob$ returns $g$.
        That means there is no longer a need for a dedicated third party, and the bottleneck its use would create can be mitigated by decentralizing it, under assumptions of rationality.
        

==> oldIntro.tex <==
\subsection*{Intro théorie des jeux}
\hrule
\begin{itemize}
    \item Several rationality models:
        Nash~\cite{Nas50,DBLP:conf/fossacs/Ummels08,DBLP:conf/lfcs/BrihayePS13},
        Subgame Perfect~\cite{DBLP:conf/concur/BrihayeBGRB19,BriceRaskinVandenbogaard21},
        Weak Subgame Perfect~\cite{DBLP:conf/fossacs/Bruyere0PR17,DBLP:conf/csl/BrihayeBMR15}, \Ms{J'ai des doutes sur la pertinence d'évoquer les versions (weak) subgame perfect ici puisqu'on ne s'en sert pas vraiment.}
        Secure~\cite{ChatterjeeHenzingerJurdzinski05,DBLP:conf/csl/BruyereMR14},
        Immune~\cite{DBLP:conf/fossacs/Brenguier16},
        Admissible~\cite{DBLP:journals/corr/BrenguierRS15}\dots \Ms{Pareil pour l'admissibilité}
    \item In the setting allowing coalition deviation: related to Strong Nash equilibria~\cite{Aumann60}.
    \item Contribution:
    \begin{itemize}
        \item study Strong Secure equilibria for $\omega$-regular objectives (\cite{DBLP:conf/csl/BruyereMR14} treats quantitative objectives for 2 players);
        \item meaningful application to security protocols;
        \item two variants of the problem: verification (which is a form of rational verification as we want the correctness condition to hold) and existence;
        \item tight complexity bounds, also studying fixed-parameters cases.
    \end{itemize}
\end{itemize}
\hrule
\bigskip

Modern systems are distributed among several agents who can be owned by different stakeholders.
Ensuring a correct behavior of such distributed systems can be a challenging task when no full control can be assumed on all agents.
In fact, it is often the case that any agent could disrupt the whole system on his own.
This is for example the case with a float of autonomous vehicles: if a vehicle actively tries to crash into others, it is quite impossible to avoid that, as anyone who has ever ridden in a bumper car could attest.
This behavior is however quite unlikely if it is assumed that the agent is \emph{rational}: no one actually voluntarily crashes their car.

Agents having individual interests that are distinct from simply being a nuisance to others can be captured by \emph{non zero-sum games}.
In this setting, each agent has a choice of actions from an \emph{arena}, also known as \emph{strategies}, and every outcome of the collective strategies of all agents (a \emph{profile}) are given a possibly different payoff for each player.
The central notion for these games is the one of \emph{equilibrium}: a set of behaviors from which it is not worthwhile to deviate from.
The notion of equilibrium was first defined by Nash in the 1950's~\cite{Nas50}, for the case where a single agent deviating would not increase their payoff.
Since then, several notions of equilibria have been defined to capture different \emph{models of rationality}: Aumann~\cite{Aumann60} defined Strong Nash Equilibria, where several players deviating conjointly cannot increase their payoff.
Other notions include Immune Equilibria~\cite{DBLP:conf/fossacs/Brenguier16}, where players should not be able to decrease the payoff of others by deviating, and Secure Equilibria~\cite{ChatterjeeHenzingerJurdzinski05} which contrasts from the former by requiring that any payoff decrease for others cannot decrease one's payoff at the same time.

Although these first definitions originated in economy theory, these game models have also been studied by computer scientists.
The most popular choice of arenas for the algorithmic study of games has been games on directed finite graphs~\cite{GaleStewart53}: each vertex of a graph belongs to a given player who can choose an outgoing transition, thus producing an infinite path.
The payoff of each player can be determined by a Boolean condition on this path, in which case it is a qualitative game, or given a numerical value as in quantitative games such as mean-payoff or discounted payoff games. \Ma{ref?}

In this paper, we study a Strong version of Secure Equilibria for qualitative payoffs defined by $\omega$-regular sets.
This notion generalizes secure equilibria by requiring that no coalition of players can harm any player not belonging to the coalition while (at least) maintaining the payoff obtained when not deviating.
The notion of secure equilibria was defined by~\cite{ChatterjeeHenzingerJurdzinski05} for two players in the qualitative setting and studied for quantitative games by~\cite{DBLP:conf/csl/BruyereMR14}.
The extension of the notion to multiplayer games and taking into account coalitions is a novel contribution of this paper.
We study the problems of checking whether a provided set of strategy profiles corresponds to Strong Secure Equilibria and the problem of existence of such a strategy profile.
We provide tight complexity bounds for several settings, corresponding of different manners the profiles and/or winning sets are provided, and also give complexity for the fixed-parameter case (usually the number of players involved is the fixed parameter).

Strong Secure Equilibria have a natural application to the verification of security protocol such as contract signing.
Indeed, in these protocols agents are willing to cooperate in order to obtain the signature of the contract, but even more willing to rob another participant by denying them an access to the signed document, even if that would cost them nothing.
The motivation for the study of security protocols is provided in Section~\ref{sec:motivatingExample} and the formal link between them and Strong Secure Equilibria is given in Section~\ref{sec:formalism}.
Examples of this connection are detailed in Section~\ref{sec:examples}.
Finally, the algorithms are detailed in Section~\ref{sec:algorithms}.

==> plan.tex <==

\section{Plan}
\Ms{Just for draft purposes}

\begin{enumerate}
    \item Modèles
    \begin{enumerate}
        \item Modèles de systèmes:
        \begin{enumerate}
            \item Text descriptions
            \item Process algebra like $\pi$-calculus
        \end{enumerate}
        Traduction vers Jeux sur graphe
        \item Modèle d'attaquant: Dolev-Yao (zero-sum) vs rational agents (non-zero sum)
    \end{enumerate}
    \item Protocoles
    \begin{enumerate}
        \item Needham-Shroeder
        \item Fair exchange protocols
    \end{enumerate}
    \item Algorithmes
\end{enumerate}

==> version1formalism.tex <==
    \section{General formalism v1}
        \subsection{Framework}

We consider the following general scenario: several \emph{agents} (for instance: programs, or human users) interact through \emph{behaviors} (for instance: sending some message after having received some other), and aim to reach a \emph{collective goal} (for instance, exchanging a cryptographic key, or signing a contract).
But, some of those agents are \emph{untrusted}: if they have the possibility, they may prefer an \emph{individual goal} in which they get a certain undue advantage (for instance: being able to read a message without having sent a delivery receipt, or buying an item without paying).
Some other untrusted agents may also be tempted to help that agent, as long as they avoid to be themselves \emph{wronged}.

Moreover, the possibility of achieving such an individual goal may depend on the behaviors of unpredictable \emph{natural} phenomena (for instance: unreliable communication channels that may lose a message, or spend an unpredictable time to deliver it; or an electrical network that may shut down).
Only some general conditions are guaranteed with those phenomena (for instance: a communication channel always end up delivering a message, even though it may spend time; or the electrical network is never down for more than three hours).
Those phenomena should be considered as a third type of agents: \emph{nature} agents.

In such a scenario, we wish to design, or to verify, \emph{protocols} that all those agents should follow, so that no untrusted agent, or coalition of untrusted agents, can cheat other agents to reach their individual goal, whatever the nature agents do; and so that reaching the collective goal is possible, at least if the natural agents have some good behavior (it is often impossible to ensure the collective goal whatever the nature agents do; but, at least cheating must always be impossible).

\begin{defi}[Protocol problem]\label{def:protocolProblem}
    A \emph{protocol problem} is a tuple:
    \[\pc = \left(\agents, \untrusted, (\behaviors_{u})_{u \in \untrusted}, (\Ind_u)_{u \in \untrusted}, (\Wrong_u)_{u \in \untrusted}, \trusted, (\behaviors_{t})_{t \in \trusted}, \nature, (\behaviors_{n})_{n \in \nature}, (\Sane_n)_{n \in \nature}, \Coll\right),\] where:

    \begin{itemize}
    \item there are three types of \emph{agents}:
    \begin{itemize}
        \item the \emph{untrusted agents} are the elements of the set $\untrusted$,

        \item the \emph{trusted agents} are the elements of the set $\trusted$,

        \item the \emph{nature agents} are the elements of the set $\nature$,
    \end{itemize}
    and we write $\agents = \untrusted \cup \trusted \cup \nature$;

    \item each agent $a$ has a set $\behaviors_a$ of available \emph{behaviors} (and for $A \subseteq \agents$, we write $\behaviors_A = \prod_{a \in A} \behaviors_a$);

    \item for each untrusted agent $u$, the sets $\Ind_u, \Wrong_u \subseteq \behaviors_\agents$ are respectively the \emph{individual goal} and the \emph{wronging condition} of agent $u$, and they satisfy $\Ind_u \cap \Wrong_u = \emptyset$;

    \item for each nature agent $n$, the set $\Sane_n \subseteq \behaviors_\agents$ is called the \emph{sanity hypothesis} of agent $n$, and there exists a behavior $\beta_n \in \behaviors_n$ such that for every $\bbeta_{-n} \in \behaviors_{-n}$, we have $(\beta_n, \bbeta_{-n}) \in \Sane_n$ -- such a behavior is called \emph{strongly sane};

    \item the set $\Coll \in \behaviors_\agents$ is called the \emph{collective goal}, and is such that for each untrusted agent $u$, we have $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$.
\end{itemize}
\end{defi}

\begin{defi}[Protocol, sane execution]
    A \emph{protocol} is a set $P \subseteq \behaviors_{\untrusted \cup \trusted}$. 
A \emph{sane execution} of $P$ is a tuple of behaviors $\bbeta \in \behaviors_{\agents}$ such that $\bbeta_{\untrusted \cup \trusted} \in P$, and that for each $n \in \nature$, the behavior $\beta_n$ is sane.
\end{defi}

%% Peut être pas la bonne place pour cela.
\begin{defi}[Strongly sane nature profile]
A profile $\bsigma_\nature=(\sigma_n)_{n\in\nature}$ is a \emph{strongly sane nature profile} if all strategies enforce sanity regardless of other agents' behavior: for every $n\in\nature$, for every profile $\bsigma_{-n}$ of other agents, $(\bsigma_{-n},\sigma_n)\in\Sane_n$.

The set of strongly sane nature profiles for $\pc$ is written $\strSaneNatProf{\pc}$.
\end{defi}
Note that by the assumptions of Definition~\ref{def:protocolProblem}, $\strSaneNatProf{\pc}\neq \emptyset$.

\begin{defi}[{[Strongly] sane extension}]
Let $\bbeta_{\untrusted\cup\trusted} \in \behaviors_{\agents}$ be a behavior for trusted and untrusted agents.
\begin{itemize}
\item  The \emph{sane extension} of $\bbeta_{\untrusted\cup\trusted}$ is the set of behaviors
\[\saneExt{\bbeta_{\untrusted\cup\trusted}}=\{(\bbeta_{\untrusted\cup\trusted},\bbeta_\nature) \mid \bbeta_{\nature} \in \behaviors_\nature\} \cap \bigcap_{n\in\nature}\Sane_n\]
of behaviors obtained when untrusted and trusted agents behave according to $\bbeta_{\untrusted\cup\trusted}$ and such that all sanity conditions of nature agents are satisfied.
\item The \emph{strongly sane extension} of $P$ is the set of behaviors
\[\stSaneExt{\bbeta_{\untrusted\cup\trusted}}=\{(\bbeta_{\untrusted\cup\trusted},\bbeta_\nature) \mid \bbeta_\nature \in \strSaneNatProf{\pc}\}\]
of behaviors obtained when untrusted and trusted agents behave according to $\bbeta_{\untrusted\cup\trusted}$ and nature agents behave in order to enforce their sanity conditions.
\end{itemize}

For a protocol $P$, the \emph{sane extension} (resp. \emph{strongly sane extension}) of $P$ is the set
\begin{mathpar}
    \saneExt{P} = \left\{\saneExt{\bbeta_{\untrusted\cup\trusted}} \mmid \bbeta_{\untrusted\cup\trusted}\in P\right\}
    \and
    \text{(resp. }
    \stSaneExt{P} = \left\{\stSaneExt{\bbeta_{\untrusted\cup\trusted}} \mmid \bbeta_{\untrusted\cup\trusted}\in P\right\}
    \text{)}
\end{mathpar}
\end{defi}
% \begin{defi}[{[Strongly] sane extension}]
% Let $P$ be a protocol for $\pc$.
% \begin{itemize}
% \item  The \emph{sane extension} of $P$ is the set of behaviors
% \[\saneExt{P}=\{(\bsigma_{\untrusted\cup\trusted},\bsigma_\nature) \mid \bsigma_{\untrusted\cup\trusted} \in P\} \cap \bigcap_{n\in\nature}\Sane_n\]
% of behaviors obtained when untrusted and trusted agents behave according to $P$ and such that all sanity conditions of nature agents are satisfied.
% \item The \emph{strongly sane extension} of $P$ is the set of behaviors
% \[\stSaneExt{P}=\{(\bsigma_{\untrusted\cup\trusted},\bsigma_\nature) \mid \bsigma_{\untrusted\cup\trusted} \in P, \bsigma_\nature \in \strSaneNatProf{\pc}\}\]
% of behaviors obtained when untrusted and trusted agents behave according to $P$ and nature agents behave in order to enforce their sanity conditions.
% \end{itemize}
% \end{defi}
The difference between the \emph{sane extension} and the \emph{strongly sane extension} is that in the strong version, nature agents have to behave sanely regardless of other agents' choices, while in the other the behaviors of the nature agents only have to ensure sanity for that given profile of behavior from the protocol.
Remark that if $P'\subseteq P$, then $\saneExt{P'}\subseteq\saneExt{P}$ and $\stSaneExt{P'}\subseteq\stSaneExt{P}$.
% \begin{proof}
% Let $\bsigma\in\saneExt{P'}$.
% Then $\bsigma=(\bsigma_{\unstrusted\cup\trusted},\bsigma_\nature)$ with $\bsigma_{\untrusted\cup\trusted}\in P'$ so $\bsigma_{\unstrusted\cup\trusted}\in P$.
% Therefore $\bsigma\in\saneExt(P)$ and $\saneExt{P'}\subseteq\saneExt{P}$.
% \end{proof}

\begin{defi}[Attack, valid protocol]
    An \emph{attack} of the \emph{coalition} $C \subseteq \untrusted$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists $\bbeta_{\untrusted \cup \trusted} \in P$ satisfying $\beta_a = \alpha_a$ for each $a \in \trusted$ or $a \in \untrusted \setminus C$ (the trusted agents, and the untrusted ones that do not belong to $C$, are following the protocol $P$);
    
        \item we have $\balpha \in \Sane_n$ for each $n \in \nature$ (the sanity hypotheses are satisfied);
    
        \item there exists $u \in C$ such that $\balpha \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in C$, we have $\balpha \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    % A protocol $P$ is \emph{valid} if there is no attack to $P$, and if there exists a sane execution of $P$ that belongs to the set $\Coll$. % exists exists
    A protocol $P$ is \emph{valid} if
    \begin{itemize}
        \item $P\neq \emptyset$,
        \item there is no attack to $P$,
        % \item  $\saneExt{P}\subseteq\Coll$.  % forall forall
        % \item  $\forall \bbeta\in P$, $\saneExt{\bbeta}\cap\Coll \neq \emptyset$.  % forall exists a.k.a. 4
        % \item  $\forall \bbeta\in P$, $\stSaneExt{\bbeta}\cap\Coll \neq \emptyset$.  % forall exists a.k.a. 4'
    \end{itemize}
    A protocol $P$ is \emph{valid under sanity assumption} if
    \begin{itemize}
        \item $P\neq \emptyset$,
        \item there is no attack to $P$,
        \item $\forall \beta\in P$, $\saneExt{\beta}\cap\Coll \neq \emptyset$.  % forall exists a.k.a. 4
    \end{itemize}
    A protocol $P$ is \emph{valid under strong sanity assumption} if
    \begin{itemize}
        \item $P\neq \emptyset$,
        \item there is no attack to $P$,
        \item $\forall \beta\in P$, $\stSaneExt{\beta}\cap\Coll \neq \emptyset$.  % forall exists a.k.a. 4'
    \end{itemize}
\end{defi}

Thus, modeling a concrete situation by a protocol problem can be done by defining appropriate individual goals and wronging conditions, depending on the type of attacks one wants to avoid: the individual goals capture what a successful attack is, while the wronging conditions capture what can discourage an untrusted agent from helping another one.
A protocol is valid if it provides a description of behaviors that ensure the fulfillment of the collective goal (provided the nature agents behave sanely) and are immune to attacks from untrusted agents.
Exactly how sane nature agents are expected to behave can be subject to discussion.
Clearly, since $\stSaneExt{P} \subseteq \saneExt{P}$, a protocol valid under strong sanity assumption is also valid under sanity assumption.

\begin{lm}
Let $P$ be a valid protocol for $\pc$.
Let $P'\subseteq P$ be a non-empty protocol.
% such that there exists a sane execution of $P'$ that belongs to the set $\Coll$.
Then $P'$ is valid.
\end{lm}
\begin{proof}
    Then one of the condition of validity must be violated.
    \begin{itemize}
        \item $P\neq \emptyset$ by assumption.
        \item $\saneExt{P'}\subseteq\saneExt{P}\subseteq\Coll$.
        \item Assume, by way of contradiction, that there is an attack $\balpha$ from coalition $C\subseteq\untrusted$ on $P'$.
        Agents in $\trusted\cup\untrusted\setminus C$ play according to $\bbeta\in P'$.
        By inclusion, $\bbeta\in P$ so $\balpha$ is also an attack of $P$, in contradiction with the validity of $P$.
    \end{itemize}
\end{proof}
This shows that the validity is preserved by adding further restrictions to a protocol.
% , provided it still allows a sane execution that satisfies the collective goal.


        \subsection{Valid protocols as SNEs}

\begin{defi}[Game]\label{def:generalGame}
    A \emph{game} is a tuple $\Game = \left(\Pi, (\Sigma_i)_{i \in \Pi}, (\mu_i)_{i \in \Pi}\right)$, where:
    \begin{itemize}
        \item $\Pi$ is a set of \emph{players};

        \item for each player $i$, the set $\Sigma_i \neq \emptyset$ gathers the \emph{strategies} available for player $i$;

        \item for each player $i$, the function $\mu_i: \Sigma_\Pi \to \RR^\Pi$ is the \emph{payoff function} of player $i$.
    \end{itemize}
\end{defi}

We now explain how such a protocol problem $\pc$ can be captured by a game $\Game$.

The players in $\Game$ are the agents of $\pc$.
The strategies available for each player $i$ in $\Game$ are the behaviors available for agent $a$ in $\pc$.

The payoff functions of $\Game$ are defined as follows:

\begin{itemize}
    \item For $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \bsigma \in \Wrong_u \\
        1 & \text{if } \bsigma \not\in \Wrong_u \cup \Ind_u \\
        2 & \text{if } \bsigma \in \Ind_u
    \end{cases};$$

    \item For $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \bsigma \not\in \Coll \\
        1 & \text{if } \bsigma \in \Coll
    \end{cases};$$

    \item For $n\in \nature$ \emph{(nature players)}:
    $$\mu_n: \bsigma \mapsto \begin{cases}
        0 & \text{if } \bsigma \not\in \Sane_n \\
        1 & \text{if } \bsigma \in \Sane_n
    \end{cases}.$$
\end{itemize}

We assume that $\untrusted, \trusted, \nature \neq \emptyset$: in particular, if there is no trusted player, we add one that has only one available strategy.


\begin{thm}\label{thm:linkSNEvalid}
%% Using definition:
%%      A protocol $P$ is \emph{valid} if there is no attack to $P$, and if there exists a sane execution of $P$ that belongs to the set $\Coll$.
    Let $\bsigma_{\untrusted \cup \trusted}$ be a strategy profile in $\Game$.
    The protocol $\{\bsigma_{\untrusted \cup \trusted}\}$ is valid if and only if there exists a strategy profile $\bsigma_\nature$ such that the strategy profile $\bsigma$ is a strong Nash equilibrium that satisfies $\mu_a(\bsigma) \geq 1$ for every player $a$.
\end{thm}

\begin{proof}~
    \begin{itemize}
        \item \emph{If $\bsigma$ is an SNE with $\mu_a(\bsigma) \geq 1$ for each $a\in\Pi$, then the protocol $P = \{\bsigma_{\untrusted \cup \trusted}\}$ is valid.}

        First, for each nature agent $n\in\nature$, we have $\mu_n(\bsigma) \geq 1$, i.e. $\bsigma \in \Sane_n$.
        The strategy profile $\bsigma$ is therefore a sane execution of $P$.
        Moreover, for each trusted player $t\in\trusted$, we have $\mu_t(\bsigma) \geq 1$, and therefore $\bsigma \in \Coll$.
        So, there exists a sane execution of $P$ that satisfies $\Coll$.

        Now, let $C\subseteq\untrusted$ be a coalition of untrusted agents.
        Let us assume that the coalition $C$ has an attack $\balpha$ to the protocol $P$.
        Then, we have $\alpha_a = \sigma_a$ for every $a \in \Pi \setminus (C \cup \nature)$; we have $\balpha \in \Sane_n$, i.e. $\mu_n(\balpha) = 1$, for each $n \in \nature$; we have $\balpha \in \Ind_u$, i.e. $\mu_u(\balpha) = 2$, for some $u \in C$; and we have $\balpha \not\in \Wrong_{u'}$, i.e. $\mu_{u'}(\balpha) \geq 1$, for every $u' \in C$.
        Thus, the strategy profile $\balpha_{C \cup \nature}$ is a profitable deviation to the strategy profile $\bsigma$, which is impossible since $\bsigma$ is an SNE.
        
        As a result, the protocol $P$ is valid.


        \item \emph{If $P = \{\bsigma_{\untrusted \cup \trusted}\}$ is a valid protocol, then there exists $\bsigma_\nature$ such that $\bsigma$ is an SNE satisfying $\mu_a(\bsigma) \geq 1$ for each $a\in\Pi$.}

        Since $P$ is valid, there is a sane execution of $P$ that belongs to $\Coll$.
        In other words, there is a collection $(\sigma_n)_{n \in \nature}$ of sane behaviors such that $\bsigma \in \Coll$: then, we have $\mu_n(\bsigma) = 1$ for each $n \in \nature$, because $\sigma_n$ is sane, which implies $\bsigma \in \Sane_n$; we have $\mu_t(\bsigma) = 1$ for each $t \in \trusted$ because $\bsigma \in \Coll$; and we have $\mu_u(\bsigma) = 1$ for each $u \in \untrusted$ because $\bsigma \in \Coll$ implies $\bsigma \not\in \Ind_u$ and $\bsigma \not\in \Wrong_u$.
        Let us show that such a strategy profile is an SNE.

        Let $C \subseteq \Pi$, and let us assume that there is a profitable deviation $\bsigma'_C$ of $\bsigma_C$.
        Let $\balpha = (\bsigma_{-C}, \bsigma'_C)$, and let us show that $\balpha$ is an attack to the protocol $P$.
        
        First, let us show that $\balpha \in \Sane_n$ for each $n \in \nature$.
        If $n\notin C$, then $\sigma_n$ is a sane behavior in $\pc$, i.e. $\sigma_n$ is a strategy that enforces $\Sane_n$ regardless of the other players' strategies, hence $\balpha \in \Sane_n$.
        If $n \in C$, then $\balpha \not\in \Sane_n$ would imply $\mu_n(\balpha) = 0$, and the deviation would not be profitable.
        
        Moreover, since the deviation is profitable, there is a player in $C$ who gets in $\balpha$ a payoff that is strictly greater than their payoff in $\bsigma$, i.e. $1$: that payoff is then necessarily equal to $2$, and that player can only be an untrusted player, which we will write $u$.
        Therefore, we have $\balpha \in \Ind_u$, which implies $\balpha \not\in \Coll$, and consequently $\mu_t(\balpha) = 0$ for each $t \in \trusted$.
        That implies that the coalition $C$ contains no trusted player, otherwise the deviation would not be profitable.
        Thus, in the strategy profile $\balpha$, every trusted player and every untrusted player who does not belong to $C \cap \untrusted$ is following the protocol $P$: we have $\alpha_i = \sigma_i$ for each $i \in \trusted \cup (\untrusted \setminus C)$.
        In addition, for any $u' \in C \cap \untrusted$, an untrusted agent of the coalition, since $\mu_{u'}(\balpha)\geq 1$, we have $\balpha\notin\Wrong_{u'}$.
        
        The tuple of behaviors $\balpha$ is therefore an attack of to the protocol $P$, which is impossible if that protocol is valid; there is therefore no profitable deviation to the strategy profile $\bsigma$, and that strategy profile is an SNE.
    \end{itemize}
\end{proof}

\begin{thm}\label{thm:linkSNEvalidND}
%% Using definition:
%%    A protocol $P$ is \emph{valid} if
%%    \begin{itemize}
%%        \item $P\neq \emptyset$,
%%        \item there is no attack to $P$,
%%        \item  $\saneExt{P}\subseteq\Coll$.
%%    \end{itemize}
A non-empty protocol $P$ is valid for $\pc$ if and only if $\saneExt{P}$ is a set of Strong Nash Equilibria that satisfy $\Coll$ in $\Game$.
\end{thm}
\begin{proof}~
    \begin{description}
    \item[\fbox{$\Rightarrow$}] Assume $P$ is valid.
        First, by definition, $\saneExt{P}\subseteq \Coll$.
        Let $\bsigma\in\saneExt{P}$.
        By definition of $\saneExt{P}$, for every $n\in\nature$, $\bsigma\in\Sane_n$, so $\mu_n(\bsigma)=1$ in $\Game$.
        By validity of $P$, $\bsigma\in\Coll$, so for $t\in\trusted$, $\mu_t(\bsigma)=1$.
        In addition, since for every $u\in\untrusted$, $\Coll\cap\Ind_u=\Coll\cap\Wrong_u=\emptyset$, $\mu_u(\bsigma)=1$.
        So for every player $a$, $\mu_a(\bsigma)=1$.

        Let's assume, by way of contradiction, that  $\bsigma$ is not an SNE.
        Then there exists a coalition $C\subseteq\agents$ and a profitable deviation for $C$, i.e. a strategy $\sigma_C'$ such that the resulting behavior $\balpha=(\bsigma_{-C},\bsigma_C')$ has a better payoff for members of the coalition: at least as good as the original payoff for everyone and strictly better for at least an agent $a$.
        Note that only untrusted agents can achieve payoff strictly higher than $1$.
        Therefore we have:
        \begin{itemize}
            \item For all $a\in C$, $\mu_a(\balpha)\geq \mu_a(\bsigma)$.
            \item There exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha)> \mu_u(\bsigma)$.
        \end{itemize}
        Let us show that $\balpha$ is an attack on $P$.

        First, let us show that $\balpha\in\Sane_n$ for all $n\in\nature$.
        If $n \notin C$, since $\bsigma_n$ is sane then it ensures $\balpha\in\Sane_n$ regardless of other players' choices.
        If $n\in C$, then $\mu_n(\balpha)\geq \mu_n(\bsigma)=1$, so $\balpha\in\Sane_n$.

        We will now show by contradiction that no trusted agent can be in coalition $C$.
        Assume $t\in\trusted\cap C$.
        Since the deviation is profitable, $\mu_t(\balpha)\geq \mu_t(\bsigma)=1$, so $\balpha\in\Coll$.
        Since $\Coll\cap\bigcup_{u\in\untrusted}\Ind_u=\emptyset$, then there is no agent $u\in C$ such that $\mu_u(\balpha)=2$, so no agent who has a strictly higher payoff than in $\bsigma$, which is a contradiction.

        Therefore in $\balpha$ all trusted agents and untrusted agents not in the coalition do follow $P$.
        By profitability, every $u\in C \cap \untrusted$ achieve at least payoff $1$, so none is wronged and $\balpha\notin\Wrong_u$.
        In addition, there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha)> \mu_u(\bsigma)$, so $\balpha\in\Ind_u$.
        So $\balpha$ is an attack on $P$, which contradicts its validity.
    \item[\fbox{$\Leftarrow$}] Assume $\saneExt{P}$ is a set of Strong Nash Equilibria that satisfy $\Coll$ in $\Game$.
        We only need to prove that there is no attack on $P$ to prove validity.
        Assume, by way of contradiction, that there is an attack $\balpha$ on $P$ by a coalition $C\subseteq \untrusted$.
        Let $\bbeta_{\untrusted\cup\trusted}\in P$ be a behavior such that $\bbeta_a=\balpha_a$ for $a\in\trusted\cup\untrusted\setminus C$.
        For $n\in \nature$, there exists a strongly sane behavior $\beta_n$ that ensures $\Sane_n$ regardless of other players' choices.
        Then $\bbeta=(\bbeta_{\untrusted\cup\trusted},\beta_n)\in\saneExt{P}$ is by hypothesis a Strong Nash Equilibrium that satisfies $\Coll$.
        
        Since $\balpha$ is an attack, there is $u^*\in C$ that satisfies its individual objective, so $\mu_{u^*}(\balpha)=2$.
        Since $\bbeta \in\Coll$, $\mu_{u^*}(\beta)=1$.
        The behavior $\balpha$ is a deviation of the deviation $\bbeta$ by coalition $C\cup \nature$.
        So for any $u\in C$, $\mu_u(\balpha)\leq\mu_u(\bbeta)$.
        As a result we have $2\leq 1$, which is a contradiction.
        Therefore $P$ has no attack.\qedhere
    \end{description}
\end{proof}

\begin{comment}
\begin{thm}\label{thm:linkSNEvalidND} % Weaker version, not iff; Would be iff if P\times Sane_\nature \subseteq \Coll, see corollary below
%% Using definition:
%%      A protocol $P$ is \emph{valid} if there is no attack to $P$, and if there exists a sane execution of $P$ that belongs to the set $\Coll$.
    Let $P$ be a non-empty protocol for $\pc$.
    \begin{itemize}
        \item If $P$ is valid then for every profile $\bsigma_{\untrusted \cup \trusted} \in P$ and every sane strategy profile $\bsigma_\nature$, if $\bsigma=(\bsigma_{\untrusted \cup \trusted},\bsigma_\nature)$ in game $\Game$ satisfies $\Coll$, then $\bsigma$ is a Strong Nash Equilibrium.
        \item If for every profile $\bsigma_{\untrusted \cup \trusted} \in P$ and for every sane strategy profile $\bsigma_\nature$, if $\bsigma=(\bsigma_{\untrusted \cup \trusted},\bsigma_\nature)$ in game $\Game$ satisfies $\Coll$ and is a Strong Nash Equilibrium, then $P$ is valid.
    \end{itemize}
\end{thm}
\begin{proof}~
    \begin{itemize}
        \item Assume $P$ is valid.
        Let $\bsigma_{\untrusted \cup \trusted} \in P$ and $\bsigma_\nature$ be a profile of sane strategies for the nature agents.
        Assume $\bsigma=(\bsigma_{\untrusted \cup \trusted},\bsigma_\nature)\in \Coll$.
        Let's prove $\bsigma$ is a Strong Nash Equilibrium (SNE).
        First, let's remark that for every $u\in\untrusted$ we have $\mu_u(\bsigma)=1$, because $\Coll$ is incompatible with $\Ind_u$ and $\Wrong_u$.
        Similarly, for $n\in\nature$, $\mu_n(\bsigma)=1$, because $\sigma_n$ is sane.
        And since $\bsigma\in \Coll$, for $t\in\trusted$ we have $\mu_t(\bsigma)=1$.
        So for every player $a$, $\mu_a(\bsigma)=1$.

        Let's assume, by way of contradiction, that  $\bsigma$ is not an SNE.
        Then there exists a coalition $C\subseteq\agents$ and a profitable deviation for $C$, i.e. a strategy $\sigma_C'$ such that the resulting behavior $\balpha=(\bsigma_{-C},\bsigma_C')$ has a better payoff for members of the coalition: at least as good as the original payoff for everyone and strictly better for at least an agent $a$.
        Note that only untrusted agents can achieve payoff strictly higher than $1$.
        Therefore we have:
        \begin{itemize}
            \item For all $a\in C$, $\mu_a(\balpha)\geq \mu_a(\bsigma)$.
            \item There exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha)> \mu_u(\bsigma)$.
        \end{itemize}
        Let us show that $\balpha$ is an attack on $P$.

        First, let us show that $\balpha\in\Sane_n$ for all $n\in\nature$.
        If $n \notin C$, since $\bsigma_n$ is sane then it ensures $\balpha\in\Sane_n$ regardless of other players' choices.
        If $n\in C$, then $\mu_n(\balpha)\geq \mu_n(\bsigma)=1$, so $\balpha\in\Sane_n$.

        We will now show by contradiction that no trusted agent can be in coalition $C$.
        Assume $t\in\trusted\cap C$.
        Since the deviation is profitable, $\mu_t(\balpha)\geq \mu_t(\bsigma)=1$, so $\balpha\in\Coll$.
        Since $\Coll\cap\bigcup_{u\in\untrusted}\Ind_u=\emptyset$, then there is no agent $u\in C$ such that $\mu_u(\balpha)=2$, so no agent who has a strictly higher payoff than in $\bsigma$, which is a contradiction.

        Therefore in $\balpha$ all trusted agents and untrusted agents not in the coalition do follow $P$.
        By profitability, every $u\in C \cap \untrusted$ achieve at least payoff $1$, so none is wronged and $\balpha\notin\Wrong_u$.
        In addition, there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha)> \mu_u(\bsigma)$, so $\balpha\in\Ind_u$.
        So $\balpha$ is an attack on $P$, which contradicts its validity.

        \item Assume that for every profile $\bsigma_{\untrusted \cup \trusted} \in P$ and for every sane strategy profile $\bsigma_\nature$, $\bsigma=(\bSigma_{\untrusted \cup \trusted},\bsigma_\nature)$ in game $\Game$ satisfies $\Coll$ and is a Strong Nash Equilibrium.
        Assume, by way of contradiction, that there is an attack $\balpha$ on $P$ by a coalition $C\subseteq \untrusted$.
        Let $\bbeta_{\untrusted\cup\trusted}\in P$ be a behavior such that $\bbeta_a=\balpha_a$ for $a\in\untrusted\cup\trusted\setminus C$.
        For $n\in \nature$, there exists a sane behavior $\beta_n$ that ensures $\Sane_n$ regardless of other players' choices.
        Then $\bbeta=(\bbeta_{\untrusted\cup\trusted},\beta_n)$ is by hypothesis a Strong Nash Equilibrium that satisfies $\Coll$.
        
        Since $\balpha$ is an attack, there is $u^*\in C$ that satisfies its individual objective, so $\mu_{u^*}(\balpha)=2$.
        Since $\bbeta \in\Coll$, $\mu_{u^*}(\beta)=1$.
        The behavior $\balpha$ is a deviation of the deviation $\bbeta$ by coalition $C\cup \nature$.
        So for any $u\in C$, $\mu_u(\balpha)\leq\mu_u(\bbeta)$.
        As a result we have $2\leq 1$, which is a contradiction.
        Therefore $P$ has no attack.

        Since $P$ is not empty and all sane behaviors induced by $P$ satisfy $\Coll$, it is a valid protocol.
    \end{itemize}
\end{proof}

In the above theorem, there is no equivalence because some attack (that therefore can not satisfy $\Coll$) could correspond to a Strong Nash Equilibrium.
On the other hand, including behaviors that do not satisfy $\Coll$ but still do not allow attacks do not violate the validity of a protocol, despite these behaviors not being SNEs.
Typically, runs of the protocol that are interrupted may not be used for an attack, but all parties have an incentive to change their behavior in order for the protocol to complete as intended and satisfy the collective goal.
Only by restricting protocols to only contain behaviors satisfying the common objective do we obtain an equivalence:
\begin{cor}
Let $P$ be a non-empty protocol for $\pc$ such that $\stSaneExt{P}\subseteq \Coll$.
Then $P$ is a valid protocol if and only if every profile $\bsigma\in\stSaneExt{P}$ is a Strong Nash Equilibrium in $\Game$.
\end{cor}
\begin{proof}
    The proof is direct from Theorem~\ref{thm:linkSNEvalidND}: every profile in $P$ with a sane strategy profile yields a behavior that by assumption is in $\Coll$.
    The first point then provides the left-to-right direction and the second point provides the right-to-left implication.
\end{proof}
\end{comment}

For a set of strategy profiles $S$, we write $S_C = \{\bsigma_C \mid \bsigma \in S\}$ the set of profiles for players of $C$ taken from a profile in $S$.

\begin{thm}~
    \begin{itemize}
        \item  Let $P$ be a protocol for $\pc$. If $P$ is valid under strong sanity assumption.
        Then for every behavior $\bsigma_{\untrusted\cup\trusted} \in P$ there exists a strategy profile $\bsigma_\nature$ such that $\bsigma$ is a Strong Nash Equilibrium in $\Game$ that satisfies, for every player $a$, $\mu_a(\bsigma)\geq1$.
        \item Let $S^{\geq1}$ be a non-empty set of Strong Nash Equilibria in $\Game$ that satisfy, for every $\sigma\in S^{\geq1}$ and for every player $a$, $\mu_a(\bsigma)\geq1$.
         Then the protocol $S^{\geq1}_{\untrusted\cup\trusted}$ is valid under sanity assumption.
    \end{itemize}
\end{thm}

\begin{proof}~
    \begin{itemize}
        \item Assume $P$ is valid for $\pc$under strong sanity assumption.
        Let $\bsigma_{\untrusted\cup\trusted} \in P$.
        Let $\bsigma_\nature \in\strSaneNatProf{\pc}$ be such that $\bsigma=(\bsigma_{\untrusted\cup\trusted},\bsigma_\nature)\in\Coll$.
        This profile exists because of the strong sanity assumption.

        By definition of $\strSaneNatProf{\pc}$, for every $n\in\nature$, $\bsigma\in\Sane_n$, so $\mu_n(\bsigma)=1$ in $\Game$.
        Since $\bsigma\in\Coll$, so for $t\in\trusted$, $\mu_t(\bsigma)=1$.
        In addition, since for every $u\in\untrusted$, $\Coll\cap\Ind_u=\Coll\cap\Wrong_u=\emptyset$, $\mu_u(\bsigma)=1$.
        So for every player $a$, $\mu_a(\bsigma)=1$.

        Let's assume, by way of contradiction, that $\bsigma$ is not an SNE.
        Then there exists a coalition $C\subseteq\agents$ and a profitable deviation for $C$, i.e. a strategy $\sigma_C'$ such that the resulting behavior $\balpha=(\bsigma_{-C},\bsigma_C')$ has a better payoff for members of the coalition: at least as good as the original payoff for everyone and strictly better for at least an agent $a$.
        Note that only untrusted agents can achieve payoff strictly higher than $1$.
        Therefore we have:
        \begin{itemize}
            \item For all $a\in C$, $\mu_a(\balpha)\geq \mu_a(\bsigma)$.
            \item There exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha)> \mu_u(\bsigma)$.
        \end{itemize}
        Let us show that $\balpha$ is an attack on $P$.

        First, let us show that $\balpha\in\Sane_n$ for all $n\in\nature$.
        If $n \notin C$, since $\bsigma_n$ is strongly sane then it ensures $\balpha\in\Sane_n$ regardless of other players' choices.
        If $n\in C$, then $\mu_n(\balpha)\geq \mu_n(\bsigma)=1$, so $\balpha\in\Sane_n$.

        We will now show by contradiction that no trusted agent can be in coalition $C$.
        Assume $t\in\trusted\cap C$.
        Since the deviation is profitable, $\mu_t(\balpha)\geq \mu_t(\bsigma)=1$, so $\balpha\in\Coll$.
        Since $\Coll\cap\bigcup_{u\in\untrusted}\Ind_u=\emptyset$, then there is no agent $u\in C$ such that $\mu_u(\balpha)=2$, so no agent who has a strictly higher payoff than in $\bsigma$, which is a contradiction.

        Therefore in $\balpha$ all trusted agents and untrusted agents not in the coalition do follow $P$.
        By profitability, every $u\in C \cap \untrusted$ achieve at least payoff $1$, so none is wronged and $\balpha\notin\Wrong_u$.
        In addition, there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha)> \mu_u(\bsigma)$, so $\balpha\in\Ind_u$.
        So $\balpha$ is an attack on $P$, which contradicts its validity.

        
        \item Assume that $S^{\geq1}$ is a non-empty set of Strong Nash Equilibria in $\Game$ that satisfy, for every $\sigma\in S^{\geq1}$ and for every player $a$, $\mu_a(\bsigma)\geq1$.
        
        First, $S^{\geq1}_{\untrusted\cup\trusted}$ is not empty by assumption.
        Let $\bsigma \in S^{\geq1}$; we have $\mu_a(\bsigma)\geq1$ for every $a$.
        It is the case for every $n\in\nature$; therefore $\bsigma\in\Sane_n$ and $\bsigma \in \saneExt{\bsigma_{\untrusted\cup\trusted}}$
        It is also the case for every trusted agent $t\in\trusted$; therefore $\bsigma\in \Coll$.
        So $\bsigma \in \saneExt{\bsigma_{\untrusted\cup\trusted}} \cap \Coll$, so this set is non-empty.

        Let's prove that there is no attack on $S^{\geq1}_{\untrusted\cup\trusted}$ to complete the proof of validity under sanity assumption.
        Assume, by way of contradiction, that there is an attack $\balpha$ on $S^{\geq1}_{\untrusted\cup\trusted}$ by a coalition $C\subseteq \untrusted$.
        Let $\bbeta\in S$ be a behavior such that $\bbeta_a=\balpha_a$ for $a\in\trusted\cup\untrusted\setminus C$.
        By assumption, $\bbeta$ is a Strong Nash Equilibrium in $\Game$ that satisfies, for every player $a$, $\mu_a(\bbeta)\geq1$.
        In particular, for every trusted agent $t\in \trusted$, $\mu_t(\bbeta)=1$ so $\bbeta \in\Coll$.
        
        Since $\balpha$ is an attack, there is $u^*\in C$ that satisfies its individual objective, so $\mu_{u^*}(\balpha)=2$.
        Since $\bbeta \in\Coll$, $\mu_{u^*}(\bbeta)=1$.
        The behavior $\balpha$ is a deviation from the strategy $\bbeta$ by coalition $C\cup \nature$.
        So for any $u\in C$, $\mu_u(\balpha)\leq\mu_u(\bbeta)$.
        As a result we have $2\leq 1$, which is a contradiction.
        Therefore $S^{\geq1}_{\untrusted\cup\trusted}$ has no attack.\qedhere
        
    \end{itemize}
\end{proof}

\subsection{Protocol problems for message exchange}

Protocols are described as the sequence of messages that ought to be exchanged between parties to reach the common goal of the protocol.
Several assumptions are usually done on these messages, for example \emph{perfect cryptography} is assumed: a message \emph{signature} cannot be faked, so only said agent can create such a message.
Similarly, ciphered messages are assumed to be only decipherable with the appropriate key.

The channels on which the messages are exchanged can be modeled as more or less reliable.
Perfect channels transmit the message immediately, reliable channels may delay messages but will always do so, unreliable channels may drop messages altogether.
Perfect channels need not appear as agents as they have no choice to perform.
Reliable and unreliable channels are modeled by \emph{nature} agents, with the sanity condition specifying how unreliable these can be.

The only actions that an agent can perform is to send a message to another agent.
Here we restrict the messages to the ones that conform to the syntax specified by the protocol.
All other messages are ignored by the recipient.
The set of possible actions (the sending of a messages) is denoted $\actions$.
When the agent is a communication channel, the action is the relaying of a message; therefore when a channel relays a message to its recipient, this correspond to the action of said recipient receiving the message.

Because protocols rely on messages being known by agents, the current state of the protocol run is fully determined by which a actions have been performed, that correspond to which messages are known by which agents.
From the set of messages currently known, agents have the possibility to send all messages they are allowed to based on rules describing the protocol.
This can be modeled by a game on graph $2^\actions\times\agents$: a round-robin has agents taking turn in sending messages (or just skip their turn).
From a state $(v,a)$, the sending of a set of messages $M\subseteq\actions$ from by $a$ means choosing as successor state $(v\cup M,a')$, where $a'$ is the next agent in the round-robin.
Abusively, we say that an agent ``sends messages $x,y,z$'' when $v'\setminus v=\{x,y,z\}$.
It is sometimes useful to refer to the absence of action ($v=v'$) as a special action $\noAct$.


==> version2formalism.tex <==
    \section{General formalisms}
        \subsection{Framework}
\Ms{Version du formalisme qui inclut directement les agents Nature qui sont un ajout ad hoc pour les hypothèses de fairness des canaux mais qui ne seraient pas une évidence dans le domaine des protocoles.}
We consider the following general scenario: several \emph{agents} (for instance: programs, or human users) interact through \emph{behaviors} (for instance: sending some message after having received some other), and aim to reach a \emph{collective goal} (for instance, exchanging a cryptographic key, or signing a contract).
But, some of those agents are \emph{untrusted}: if they have the possibility, they may prefer an \emph{individual goal} in which they get a certain undue advantage (for instance: being able to read a message without having sent a delivery receipt, or buying an item without paying).
Some other untrusted agents may also be tempted to help that agent, as long as they avoid to be themselves \emph{wronged}.

Moreover, the possibility of achieving such an individual goal may depend on the behaviors of unpredictable \emph{natural} phenomena (for instance: unreliable communication channels that may lose a message, or spend an unpredictable time to deliver it; or an electrical network that may shut down).
Only some general conditions are guaranteed with those phenomena (for instance: a communication channel always end up delivering a message, even though it may spend time; or the electrical network is never down for more than three hours).
Those phenomena should be considered as a third type of agents: \emph{nature} agents.

In such a scenario, we wish to design, or to verify, \emph{protocols} that all those agents should follow, so that no untrusted agent, or coalition of untrusted agents, can cheat other agents to reach their individual goal, whatever the nature agents do; and so that reaching the collective goal is possible, at least if the natural agents have some good behavior (it is often impossible to ensure the collective goal whatever the nature agents do; but, at least cheating must always be impossible).

\begin{defi}[Protocol challenge]\label{def:protocolProblem}
    A \emph{protocol challenge} is a tuple:
    \[\pc = \left(\Traces, \tr, \untrusted, (\behaviors_{u})_{u \in \untrusted}, (\Ind_u)_{u \in \untrusted}, (\Wrong_u)_{u \in \untrusted}, \trusted, (\behaviors_{t})_{t \in \trusted}, \nature, (\behaviors_{n})_{n \in \nature}, (\Sane_n)_{n \in \nature}, \Coll\right),\] where:

    \begin{itemize}
    \item there are three types of \emph{agents}:
    \begin{itemize}
        \item the \emph{untrusted agents} are the elements of the set $\untrusted$,

        \item the \emph{trusted agents} are the elements of the set $\trusted$,

        \item the \emph{nature agents} are the elements of the set $\nature$,
    \end{itemize}
    and we write $\agents = \untrusted \cup \trusted \cup \nature$;

    \item each agent $a$ has a set $\behaviors_a$ of available \emph{behaviors} (and for $A \subseteq \agents$, we write $\behaviors_A = \prod_{a \in A} \behaviors_a$);

    \item the set $\Traces$ is the set of \emph{traces}, and the \emph{trace mapping} $\tr: \behaviors_\agents \rightarrow \Traces$ maps each tuple of behaviors to one trace;

    \item for each untrusted agent $u$, the sets $\Ind_u, \Wrong_u \subseteq \Traces$ are respectively the \emph{individual goal} and the \emph{wronging condition} of agent $u$, and they satisfy $\Ind_u \cap \Wrong_u = \emptyset$;

    \item for each nature agent $n$, the set $\Sane_n \subseteq \Traces$ is called the \emph{sanity hypothesis} of agent $n$.
    We call \emph{sane behavior} a behavior $\beta_n$ such that $\tr(\beta_n, \bbeta_{-n}) \in \Sane_n$ for all $\bbeta_{-n}$, and we write $\Sane = \bigcap_n \Sane_n$.
    % We assume that every sane trace is compatible with sane behaviors: for every $\tau \in \Sane$, there exists $\bbeta$ such that $\tr(\bbeta) = \tau$ and that each $\beta_n$ is sane;
    We assume that every nature behavior participating in a sane trace can be considered to be sane: for every $\bbeta$ such that $\tr(\bbeta) \in \Sane$, there exists $\bbeta_\nature'$ such that $\tr(\bbeta) = \tr(\bbeta_{-\nature},\bbeta_\nature')$;

    \item the set $\Coll \in \Traces$ is called the \emph{collective goal}, and is such that for each untrusted agent $u$, we have $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$.
\end{itemize}
\end{defi}

The requirements on sanity hypotheses ensure that sanity should be always achievable by nature agents, regardless of the cooperation of others.
In a sense, it places weak enough conditions to only exclude degenerate behaviors from the nature agents.

\begin{defi}[Protocol, implementation, execution]
    A \emph{protocol} is a nonempty set $P \subseteq \behaviors_{\untrusted \cup \trusted}$.
    An \emph{implementation} of $P$ is an element $\bbeta_{\untrusted \cup \trusted}$ of $P$.
    An \emph{execution} of $\bbeta_{\untrusted \cup \trusted}$ is a trace $\tau$ such that there exists $\bbeta_\nature \in \behaviors_\nature$ with $\tau = \tr(\bbeta)$.
\end{defi}



\begin{defi}[Attack, valid protocol]
    An \emph{attack} of the \emph{alliance} $A \subseteq \untrusted$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists an implementation $\bbeta_{\untrusted \cup \trusted} \in P$ such that, for each $a \in \trusted$ or $a \in \untrusted \setminus A$, we have $\beta_a = \alpha_a$ (the trusted agents, and the untrusted ones that do not belong to $A$, are following the protocol $P$);
    
        \item we have $\tr(\balpha) \in \Sane$ (the sanity hypotheses are satisfied);
    
        \item there exists $u \in A$ such that $\tr(\balpha) \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in A$, we have $\tr(\balpha) \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    A protocol $P$ is \emph{valid} if:
    \begin{itemize}
        \item there is no attack to $P$,
        
        \item and if every implementation of $P$ has a sane execution that satisfies the collective goal.
    \end{itemize}
\end{defi}

Thus, modeling a concrete situation by a protocol challenge can be done by defining appropriate individual goals and wronging conditions, depending on the type of attacks one wants to avoid: the individual goals capture what a successful attack is, while the wronging conditions capture what can discourage an untrusted agent from helping another one.
A protocol is valid if it provides a description of behaviors that ensure the fulfillment of the collective goal (provided the nature agents behave sanely) and are immune to attacks from untrusted agents.


        \subsection{Valid protocols as SNEs}

\begin{defi}[Game]\label{def:generalGame}
    A \emph{game} is a tuple $\Game = \left(\Pi, (\Sigma_i)_{i \in \Pi}, (\mu_i)_{i \in \Pi}\right)$, where:
    \begin{itemize}
        \item $\Pi$ is a set of \emph{players};

        \item for each player $i$, the set $\Sigma_i \neq \emptyset$ gathers the \emph{strategies} available for player $i$;

        \item for each player $i$, the function $\mu_i: \Sigma_\Pi \to \RR^\Pi$ is the \emph{payoff function} of player $i$.
    \end{itemize}
\end{defi}

We now explain how such a protocol challenge $\pc$ can be captured by a game $\Game$.

The players in $\Game$ are the agents of $\pc$.
The strategies available for each player $i$ in $\Game$ are the behaviors available for agent $a$ in $\pc$.

The payoff functions of $\Game$ are defined as follows:

\begin{itemize}
    \item For $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \Wrong_u \\
        1 & \text{if } \tr(\bsigma) \not\in \Wrong_u \cup \Ind_u \\
        2 & \text{if } \tr(\bsigma) \in \Ind_u
    \end{cases};$$

    \item For $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Coll \\
        1 & \text{if } \tr(\bsigma) \in \Coll
    \end{cases};$$

    \item For $n\in \nature$ \emph{(nature players)}:
    $$\mu_n: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Sane_n \\
        1 & \text{if } \tr(\bsigma) \in \Sane_n
    \end{cases}.$$
\end{itemize}

We assume that $\trusted \neq \emptyset$: if there is no trusted player, we add one that has only one available strategy.


\begin{thm}\label{thm:linkSNEvalid}
%% Using definition:
%%      A protocol $P$ is \emph{valid} if there is no attack to $P$, and if there exists a sane execution of $P$ that belongs to the set $\Coll$.
    Let $P$ be a protocol in $\pc$.
    The protocol $P$ is valid if and only if for each $\bsigma_{\untrusted \cup \trusted} \in P$, there exists a strategy profile $\bsigma_\nature$ such that the strategy profile $\bsigma$ is a strong Nash equilibrium satisfying $\mu_a(\bsigma) = 1$ for every player $a$.
\end{thm}

\begin{proof}~
    \begin{itemize}
        \item \emph{If $P$ is valid.}
        
        Let $\bsigma_{\untrusted\cup\trusted} \in P$.
        Since $P$ is valid, there exists a strategy profile $\bsigma_\nature$ such that $\tr(\bsigma) \in \Coll \cap \Sane$.
        Moreover, since by definition of a protocol challenge, every nature behavior participating in a sane trace can be assumed to be sane, we can consider that it is indeed the case and that each $\sigma_n$ is sane.
        Since $\tr(\bsigma) \in \Sane$, we have $\mu_n(\bsigma) = 1$ for every $n \in \nature$, and since $\tr(\bsigma) \in \Coll$, we have $\mu_t(\bsigma) = 1$ for each $t \in \trusted$.
        For each $u \in \untrusted$, since $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$ by definition of a protocol challenge, we have $\mu_u(\bsigma) = 1$.

        Let us now prove that $\bsigma$ is an SNE.
        Let us assume that there exists a coalition $C \subseteq \agents$, that has a profitable deviation $\bsigma'_C$.
        Let $\balpha=(\bsigma_{-C},\bsigma_C')$: we will prove that $\balpha$ is an attack to $P$.
        Only untrusted agents can achieve payoff strictly higher than $1$.
        Therefore, we have:
        
        \begin{itemize}
            \item $\mu_a(\balpha) \geq 1$ for all $a \in C$;
            
            \item and there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha) = 2$, i.e. $\tr(\balpha) \in \Ind_u$.
        \end{itemize}

        Note that $\tr(\balpha) \in \Ind_u$ implies $\tr(\balpha) \not\in \Coll$, and therefore $\mu_t(\balpha) = 0$ for every $t \in \trusted$.
        Therefore, the coalition $C$ contains no trusted player.
        Consequently, in the strategy profile $\balpha$, all trusted agents and all the untrusted agents that are not in the coalition do follow $\bsigma_{\untrusted\cup\trusted}$.
        Moreover, each agent of the alliance $A = C \cap \untrusted$ has the payoff at least $1$, i.e. is not wronged; and at least one satisfies their individual objective.

        Let us now show that $\balpha\in\Sane_n$ for all $n\in\nature$.
        If $n \in C$, then $\mu_n(\balpha) \geq  \mu_n(\bsigma)=1$, so $\balpha\in\Sane_n$.
        If $n \notin C$, since $\sigma_n$ is a sane behavior, then it ensures $\balpha \in \Sane_n$ regardless of other players' choices.

        So $\balpha$ is an attack of the alliance $A$ on $P$, which contradicts its validity.


        \item \emph{If every $\bsigma_{\untrusted \cup \trusted} \in P$ can be completed into an SNE $\bsigma$ that yields payoff $1$ to every player.}

        Then, the trace $\tr(\bsigma)$ is an execution of $\bsigma_{\untrusted \cup \trusted}$ that satisfies the collective goal, and all the sanity hypotheses: every implementation of $P$ has an execution that satisfies the collective goal.

        Now, let us assume that there is an attack $\balpha$ of the alliance $A \subseteq \untrusted$ on the protocol $P$.
        Let $\bsigma_{\untrusted \cup \trusted}$ be an implementation of $P$ such that $\balpha_{\trusted \cup \untrusted \setminus A} = \bsigma_{\trusted \cup \untrusted \setminus A}$.
        Let $\bsigma_\nature$ be a strategy profile such that $\bsigma$ is an SNE that gives every player a payoff equal to $1$.
        Consider the coalition $C = A \cup \nature$: we will prove that $\balpha_C$ is a profitable deviation of $\bsigma_C$.
        First, by definition of an attack, we have $\tr(\balpha) \in \Sane$, and therefore $\mu_n(\balpha) = 1$ for each nature player $n$.
        Moreover, for each untrusted agent $u \in A$, we have $\tr(\balpha) \notin \Wrong_u$, i.e. $\mu_u(\balpha) \geq 1$.
        Finally, there is an untrusted agent $u \in A$ such that $\tr(\balpha) \in \Ind_u$, i.e. $\mu_u(\balpha) = 2$.
       As a consequence, the strategy profile $\balpha_C$ is a profitable deviation of $\bsigma_C$, which is impossible since $\bsigma$ is an SNE: there is therefore no attack to $P$, which is a valid protocol.\qedhere
    \end{itemize}
\end{proof}



\begin{cor}
    A protocol challenge admits a valid protocol if and only if the corresponding game admits an SNE that gives every player the payoff $1$.
\end{cor}

==> version3formalism.tex <==
    \section{General formalisms v3}
        \subsection{Framework}

We consider the following general scenario: several \emph{agents} (for instance: programs, or human users) interact through \emph{behaviors} (for instance: sending some message after having received some other), and aim to reach a \emph{collective goal} (for instance, exchanging a cryptographic key, or signing a contract).
But, some of those agents are \emph{untrusted}: if they have the possibility, they may prefer an \emph{individual goal} in which they get a certain undue advantage (for instance: being able to read a message without having sent a delivery receipt, or buying an item without paying).
Some other untrusted agents may also be tempted to help that agent, as long as they avoid to be themselves \emph{wronged}.

Moreover, the possibility of achieving such an individual goal may depend on the behaviors of unpredictable \emph{natural} phenomena (for instance: unreliable communication channels that may lose a message, or spend an unpredictable time to deliver it; or an electrical network that may shut down).
Only some general conditions are guaranteed with those phenomena (for instance: a communication channel always end up delivering a message, even though it may spend time; or the electrical network is never down for more than three hours).
Those phenomena should be considered as a third type of agents: \emph{nature} agents.

In such a scenario, we wish to design, or to verify, \emph{protocols} that all those agents should follow, so that no untrusted agent, or coalition of untrusted agents, can cheat other agents to reach their individual goal, whatever the nature agents do; and so that reaching the collective goal is possible, at least if the natural agents have some good behavior (it is often impossible to ensure the collective goal whatever the nature agents do; but, at least cheating must always be impossible).

\begin{defi}[Protocol challenge]\label{def:protocolProblem}
    A \emph{protocol challenge} is a tuple:
    \[\pc = \left(\Traces, \tr, \untrusted, (\behaviors_{u})_{u \in \untrusted}, (\Ind_u)_{u \in \untrusted}, (\Wrong_u)_{u \in \untrusted}, \trusted, (\behaviors_{t})_{t \in \trusted}, \nature, (\behaviors_{n})_{n \in \nature}, (\Sane_n)_{n \in \nature}, \Coll\right),\] where:

    \begin{itemize}
    \item there are three types of \emph{agents}:
    \begin{itemize}
        \item the \emph{untrusted agents} are the elements of the set $\untrusted$,

        \item the \emph{trusted agents} are the elements of the set $\trusted$,

        \item the \emph{nature agents} are the elements of the set $\nature$,
    \end{itemize}
    and we write $\agents = \untrusted \cup \trusted \cup \nature$;

    \item each agent $a$ has a set $\behaviors_a$ of available \emph{behaviors} (and for $A \subseteq \agents$, we write $\behaviors_A = \prod_{a \in A} \behaviors_a$);

    \item the set $\Traces$ is the set of \emph{traces}, and the \emph{trace mapping} $\tr: \behaviors_\agents \rightarrow \Traces$ maps each tuple of behaviors to one trace;

    \item for each untrusted agent $u$, the sets $\Ind_u, \Wrong_u \subseteq \Traces$ are respectively the \emph{individual goal} and the \emph{wronging condition} of agent $u$, and they satisfy $\Ind_u \cap \Wrong_u = \emptyset$;

    \item for each nature agent $n$, the set $\Sane_n \subseteq \Traces$ is called the \emph{sanity hypothesis} of agent $n$.
    We call \emph{sane behavior} a behavior $\beta_n$ such that $\tr(\beta_n, \bbeta_{-n}) \in \Sane_n$ for all $\bbeta_{-n}$, and we write $\Sane = \bigcap_n \Sane_n$.
    %We assume that every sane trace is compatible with sane behaviors: for every $\tau \in \Sane$, there exists $\bbeta$ such that $\tr(\bbeta) = \tau$ and that each $\beta_n$ is sane;

    \item the set $\Coll \in \Traces$ is called the \emph{collective goal}, and is such that for each untrusted agent $u$, we have $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$.
\end{itemize}
\end{defi}

The requirements on sanity hypotheses ensure that sanity should be always achievable by nature agents, regardless of the cooperation of others.
In a sense, it places weak enough conditions to only exclude degenerate behaviors from the nature agents.

\begin{defi}[Protocol]
    A \emph{protocol} is a nonempty set $P \subseteq \behaviors_\agents$.
\end{defi}



\begin{defi}[Attack, valid protocol]
    An \emph{attack} of the \emph{coalition} $C \subseteq \untrusted$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists $\bbeta \in P$ satisfying $\beta_a = \alpha_a$ for each $a \in \trusted$ or $a \in \untrusted \setminus C$ (the trusted agents, and the untrusted ones that do not belong to $C$, are following the protocol $P$);
    
        \item we have $\tr(\balpha) \in \Sane$ (the sanity hypotheses are satisfied);
    
        \item there exists $u \in C$ such that $\tr(\balpha) \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in C$, we have $\tr(\balpha) \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    A protocol $P$ is \emph{valid} if there is no attack to $P$, and if every $\bbeta \in P$ is such that $\tr(\bbeta) \in \Coll$, and each $\beta_n$ for $n \in \nature$ is a sane behavior.
\end{defi}

Thus, modelling a concrete situation by a protocol challenge can be done by defining appropriate individual goals and wronging conditions, depending on the type of attacks one wants to avoid: the individual goals capture what a successful attack is, while the wronging conditions capture what can discourage an untrusted agent from helping another one.
A protocol is valid if it provides a description of behaviors that ensure the fulfillment of the collective goal (provided the nature agents behave sanely) and are immune to attacks from untrusted agents.


        \subsection{Valid protocols as SNEs}

\begin{defi}[Game]\label{def:generalGame}
    A \emph{game} is a tuple $\Game = \left(\Pi, (\Sigma_i)_{i \in \Pi}, (\mu_i)_{i \in \Pi}\right)$, where:
    \begin{itemize}
        \item $\Pi$ is a set of \emph{players};

        \item for each player $i$, the set $\Sigma_i \neq \emptyset$ gathers the \emph{strategies} available for player $i$;

        \item for each player $i$, the function $\mu_i: \Sigma_\Pi \to \RR^\Pi$ is the \emph{payoff function} of player $i$.
    \end{itemize}
\end{defi}

We now explain how such a protocol challenge $\pc$ can be captured by a game $\Game$.

The players in $\Game$ are the agents of $\pc$.
The strategies available for each player $i$ in $\Game$ are the behaviors available for agent $a$ in $\pc$.

The payoff functions of $\Game$ are defined as follows:

\begin{itemize}
    \item For $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \Wrong_u \\
        1 & \text{if } \tr(\bsigma) \not\in \Wrong_u \cup \Ind_u \\
        2 & \text{if } \tr(\bsigma) \in \Ind_u
    \end{cases};$$

    \item For $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Coll \\
        1 & \text{if } \tr(\bsigma) \in \Coll
    \end{cases};$$

    \item For $n\in \nature$ \emph{(nature players)}:
    $$\mu_n: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Sane_n \\
        1 & \text{if } \tr(\bsigma) \in \Sane_n
    \end{cases}.$$
\end{itemize}

We assume that $\trusted \neq \emptyset$: if there is no trusted player, we add one that has only one available strategy.


\begin{thm}\label{thm:linkSNEvalid}
%% Using definition:
%%      A protocol $P$ is \emph{valid} if there is no attack to $P$, and if there exists a sane execution of $P$ that belongs to the set $\Coll$.
    Let $P$ be a protocol for $\pc$.
    The protocol $P$ is valid if and only if each $\bsigma \in P$ is a strong Nash equilibrium satisfying $\mu_a(\bsigma) = 1$ for every player $a$.
\end{thm}

\begin{proof}~
    \begin{itemize}
        \item \emph{If $P$ is valid.}
        
        Let $\bsigma \in P$.
        Since $P$ is valid, we have $\tr(\bsigma) \in \Coll$, and each $\sigma_n$ is a sane behavior.
        Thus, we have $\tr(\bsigma) \in \Sane$, i.e. $\mu_n(\bsigma) = 1$ for every $n \in \nature$, and since $\tr(\bsigma) \in \Coll$, we have $\mu_t(\bsigma) = 1$ for each $t \in \trusted$, and for each $u \in \untrusted$, since $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$ by definition of a protocol challenge, we have $\mu_u(\bsigma) = 1$.

        Let us now prove that $\bsigma$ is an SNE.
        Assume that there exists a coalition $C \subseteq \agents$, that has a profitable deviation $\bsigma'_C$.
        Let $\balpha=(\bsigma_{-C},\bsigma_C')$: we will prove that $\balpha$ is an attack to $P$.
        Only untrusted agents can achieve payoffs strictly higher than $1$.
        Therefore, we have:
        
        \begin{itemize}
            \item for all $a \in C$, $\mu_a(\balpha) \geq 1$.
            
            \item there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha) = 2$, i.e. $\tr(\balpha) \in \Ind_u$.
        \end{itemize}

        Note that $\tr(\balpha) \in \Ind_u$ implies $\tr(\balpha) \not\in \Coll$, and therefore $\mu_t(\balpha) = 0$ for every $t \in \trusted$.
        Therefore, the coalition $C$ contains no trusted player.
        Therefore, in the strategy profile $\balpha$, all trusted agents and all the untrusted agents that are not in the coalition do follow $P$.
        Every untrusted agent that belongs to $C$ has at least the payoff $1$, i.e. is not wronged; and at least one satisfies their individual objective.

        Let us now show that $\balpha\in\Sane_n$ for all $n\in\nature$.
        If $n \in C$, then $\mu_n(\balpha) \geq  \mu_n(\bsigma)=1$, so $\balpha\in\Sane_n$.
        If $n \notin C$, since $\sigma_n$ is a sane behavior, then it ensures $\balpha \in \Sane_n$ regardless of other players' choices.

        So $\balpha$ is an attack on $P$, which contradicts its validity.


        \item \emph{If every $\bsigma \in P$ is an SNE that gives every player the payoff $1$.}

        Thus, the trace $\tr(\bsigma)$ satisfies the collective goal, and all the sanity hypotheses.

        Now, let us assume that there is an attack $\balpha$ of the coalition $C$ to the protocol $P$.
        Let $\bsigma \in P$ be such that $\balpha_{\trusted \cup \untrusted \setminus C} = \bsigma_{\trusted \cup \untrusted \setminus C}$.
        We will prove that $\balpha_{\nature \cup C}$ is a profitable deviation of $\bsigma_{\nature \cup C}$.
        First, by definition of an attack, we have $\tr(\balpha) \in \Sane$, and therefore $\mu_n(\balpha) = 1$ for each nature player $n$.
        Moreover, for each untrusted agent $u \in C$, we have $\tr(\balpha) \notin \Wrong_u$, i.e. $\mu_u(\balpha) \geq 1$.
        Finally, there is an untrusted agent $u \in C$ such that $\tr(\balpha) \in \Ind_u$, i.e. $\mu_u(\balpha) = 2$.
       As a consequence, the strategy profile $\balpha_{\nature \cup C}$ is a profitable deviation of $\bsigma_{\nature \cup C}$, which is impossible since $\bsigma$ is an SNE: there is therefore no attack to $P$, which is a valid protocol.\qedhere
    \end{itemize}
\end{proof}



\begin{cor}
    A protocol challenge admits a valid protocol if and only if the corresponding game admits an SNE that gives every player the payoff $1$.
\end{cor}

==> version4formalism.tex <==
    \section{General formalisms}

        \subsection{Motivating example}
        Consider the problem of the swap of two item between two agents through a postal service.
        The agents performing this exchange may not trust each other, and neither wants to fulfill their end of the deal if they do not obtain the other in exchange.
        On the other hand, getting the other agent's item while still keeping their own is not only acceptable but even preferred (albeit morally dubious).
        
        The normal protocol to follow would be that they both send the item to the other and they should both end up with their end of the bargain fulfilled.
        This however is open to cheating from either party who can not send their item and be rewarded.
        A third party can be used an an intermediary to which both parties send their item.
        They are then transferred to the intended recipient only when both items have been received (or returned to the original owner after a predefined amount of time).
        This idea works only if it is assumed that the third party is always honest: a corrupted third party could well transmit both items to a single agent, violating the security of the exchange protocol.
        Assuming honesty on the part of the third party is akin to specifying that his preference is towards the completion of the bargain rather than one agent gaining unfair advantage.

        With only two agents $\alice$ and $\bob$ (no third party), the status of each item $\{\textit{item}_1,\textit{item}_2\}$ can be in possession of $\alice$, $\bob$, or in transit.
        When an agent possesses an item, it can be sent to the other, in which case it becomes in transit.
        The possible behaviors of $\alice$ and $\bob$ are as follow: send the item immediately, wait for reception of the item to send the item, never send the item (and all interleavings of these actions taken by each agent).
        From these possibility, is it possible to find a fair and secure way to exchange the items?

        A similar model can be devised with the additional third party: each items can now be sent to this third party $\ttp$ instead of the other agent.
        Is it possible to find a exchange protocol in that case?
        Do we have to specify that this third party is honest or can we do without this hypothesis?

        In this paper we propose a formal framework for these questions, and relate it to the notion of multiplayer games and more specifically Strong Nash Equilibria.
        
        \subsection{Framework}
\Ms{Version du formalisme sans les agents Nature.}

We consider the following general scenario: several \emph{agents} (for instance: programs, or human users) interact through \emph{behaviors} (for instance: sending some message after having received some other), and aim to reach a \emph{collective goal} (for instance, exchanging a cryptographic key, or signing a contract).
But, some (or all) of those agents are \emph{untrusted}: if they have the possibility, they may prefer an \emph{individual goal} in which they get a certain undue advantage (for instance: being able to read a message without having sent a delivery receipt, or buying an item without paying).
Some other untrusted agents may also be tempted to help that agent, as long as they avoid to be themselves \emph{wronged}.

In such a scenario, we wish to design, or to verify, \emph{protocols} that all those agents should follow, so that the collective goal is achieved, and moreover no untrusted agent, or coalition of untrusted agents, can cheat other agents to reach their individual goal.

\Le{A priori, la notion de trace est inutile.}

\begin{defi}[Protocol challenge]\label{def:protocolProblemNoNature}
    A \emph{protocol challenge} is a tuple:
    \[\pc = \left(\untrusted, (\behaviors_{u})_{u \in \untrusted}, \trusted, (\behaviors_{t})_{t \in \trusted}, \Traces, \tr, (\Ind_u)_{u \in \untrusted}, (\Wrong_u)_{u \in \untrusted}, \Coll\right),\] where:

    \begin{itemize}
    \item there are two types of \emph{agents}:
    \begin{itemize}
        \item the \emph{untrusted agents} are the elements of the set $\untrusted$,

        \item the \emph{trusted agents} are the elements of the set $\trusted$,
    \end{itemize}
    and we write $\agents = \untrusted \cup \trusted$;

    \item each agent $a$ has a set $\behaviors_a\neq \emptyset$ of available \emph{behaviors} (and for $A \subseteq \agents$, we write $\behaviors_A = \prod_{a \in A} \behaviors_a$);

    \item the set $\Traces$ is the set of \emph{traces}, and the \emph{trace mapping} $\tr: \behaviors_\agents \rightarrow \Traces$ maps each tuple of behaviors to one trace;

    \item for each untrusted agent $u$, the sets $\Ind_u, \Wrong_u \subseteq \Traces$ are respectively the \emph{individual goal} and the \emph{wronging condition} of agent $u$, and they satisfy $\Ind_u \cap \Wrong_u = \emptyset$;

    \item the set $\Coll \in \Traces$ is called the \emph{collective goal}, and is such that for each untrusted agent $u$, we have $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$.
\end{itemize}
\end{defi}

\begin{defi}[Protocol, implementation, execution]
    A \emph{protocol} is a nonempty set $P \subseteq \behaviors_\agents$.
    An \emph{implementation} of $P$ is an element $\bbeta$ of $P$.
    The \emph{execution} of $\bbeta$ is the trace $\tau = \tr(\bbeta)$.
\end{defi}



\begin{defi}[Attack, valid protocol]
    An \emph{attack} of the \emph{alliance} $A \subseteq \untrusted$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists an implementation $\bbeta \in P$ such that, for each $a \in \trusted$ or $a \in \untrusted \setminus A$, we have $\beta_a = \alpha_a$ (the trusted agents, and the untrusted ones that do not belong to $A$, are following the protocol $P$);
        
        \item there exists $u \in A$ such that $\tr(\balpha) \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in A$, we have $\tr(\balpha) \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    A protocol $P$ is \emph{valid} if:
    \begin{itemize}
        \item there is no attack to $P$,
        
        \item the execution of all implementation of $P$ satisfies the collective goal: $\tr(P)\subseteq \Coll$.
    \end{itemize}
\end{defi}

Thus, modeling a concrete situation by a protocol challenge can be done by defining appropriate individual goals and wronging conditions, depending on the type of attacks one wants to avoid: the individual goals capture what a successful attack is, while the wronging conditions capture what can discourage an untrusted agent from helping another one.
A protocol is valid if it provides a description of behaviors that ensure the fulfillment of the collective goal and are immune to attacks from untrusted agents.
%%%

        \subsection{Valid protocols as SNEs}

\begin{defi}[Game]\label{def:generalGame}
    A \emph{game} is a tuple $\Game = \left(\Pi, (\Sigma_i)_{i \in \Pi}, (\mu_i)_{i \in \Pi}\right)$, where:
    \begin{itemize}
        \item $\Pi$ is a set of \emph{players};

        \item for each player $i$, the set $\Sigma_i \neq \emptyset$ gathers the \emph{strategies} available for player $i$;

        \item for each player $i$, the function $\mu_i: \Sigma_\Pi \to \RR$ is the \emph{payoff function} of player $i$.
    \end{itemize}
\end{defi}

We now explain how such a protocol challenge $\pc$ can be captured by a game $\Game$.

The players in $\Game$ are the agents of $\pc$.
The strategies available for each player $i$ in $\Game$ are the behaviors available for agent $a$ in $\pc$.

The payoff functions of $\Game$ are defined as follows:

\begin{itemize}
    \item For $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \Wrong_u \\
        1 & \text{if } \tr(\bsigma) \not\in \Wrong_u \cup \Ind_u \\
        2 & \text{if } \tr(\bsigma) \in \Ind_u
    \end{cases};$$

    \item For $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Coll \\
        1 & \text{if } \tr(\bsigma) \in \Coll
    \end{cases};$$
\end{itemize}

We assume that the protocol challenge contains at least one trusted agent, and two untrusted agents --- if that is not the case, one can add additional players with only one available strategy.


\begin{thm}\label{thm:linkSNEvalidNoNature}
    Let $P$ be a protocol in $\pc$.
    The protocol $P$ is valid if and only if for each $\bsigma \in P$ is a strong Nash equilibrium satisfying $\mu_a(\bsigma) = 1$ for every player $a$.
\end{thm}

\begin{proof}~
    \begin{itemize}
        \item \emph{If $P$ is valid.}
        
        Let $\bsigma \in P$.
        Since $\tr(\bsigma) \in \Coll$, we have $\mu_t(\bsigma) = 1$ for each $t \in \trusted$.
        For each $u \in \untrusted$, since $\Coll \cap \Ind_u = \Coll \cap \Wrong_u = \emptyset$ by definition of a protocol challenge, we have $\mu_u(\bsigma) = 1$.

        Let us now prove that $\bsigma$ is an SNE.
        Let us assume that there exists a coalition $C \subseteq \agents$, that has a profitable deviation $\bsigma'_C$.
        Let $\balpha=(\bsigma_{-C},\bsigma_C')$: we will prove that $\balpha$ is an attack to $P$.
        Only untrusted agents can achieve payoff strictly higher than $1$.
        Therefore, we have:
        
        \begin{itemize}
            \item $\mu_a(\balpha) \geq 1$ for all $a \in C$;
            
            \item and there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha) = 2$, i.e. $\tr(\balpha) \in \Ind_u$.
        \end{itemize}

        Note that $\tr(\balpha) \in \Ind_u$ implies $\tr(\balpha) \not\in \Coll$, and therefore $\mu_t(\balpha) = 0$ for every $t \in \trusted$.
        Therefore, the coalition $C$ contains no trusted player.
        Consequently, in the strategy profile $\balpha$, all trusted agents and all the untrusted agents that are not in the coalition do follow $\bsigma$.
        Moreover, each agent of the alliance $A = C \cap \untrusted$ has the payoff at least $1$, i.e. is not wronged; and at least one satisfies their individual objective.

        So $\balpha$ is an attack of the alliance $A$ on $P$, which contradicts its validity.


        \item \emph{If every $\bsigma \in P$ is an SNE that yields payoff $1$ to every player.}

        Then, since $\trusted\neq\emptyset$, $\tr(\bsigma)$, the execution of $\bsigma$, satisfies the collective goal.

        Now, let us assume that there is an attack $\balpha$ of the alliance $A \subseteq \untrusted$ on the protocol $P$.
        Let $\bsigma$ be an implementation of $P$ such that $\balpha_{\agents \setminus A} = \bsigma_{\agents \setminus A}$.
        By assumption, $\bsigma$ is an SNE that gives every player a payoff equal to $1$.
        Consider the coalition $A$: we will prove that $\balpha_A$ is a profitable deviation of $\bsigma_A$.
        For each untrusted agent $u \in A$, we have $\tr(\balpha) \notin \Wrong_u$, i.e. $\mu_u(\balpha) \geq 1$.
        Finally, there is an untrusted agent $u \in A$ such that $\tr(\balpha) \in \Ind_u$, i.e. $\mu_u(\balpha) = 2$.
       As a consequence, the strategy profile $\balpha_A$ is a profitable deviation of $\bsigma_A$, which is impossible since $\bsigma$ is an SNE: there is therefore no attack to $P$, which is a valid protocol.\qedhere
    \end{itemize}
\end{proof}



\begin{cor}
    A protocol challenge admits a valid protocol if and only if the corresponding game admits an SNE that gives every player the payoff $1$.
\end{cor}

\subsection{Finite models of protocols}
Modeling and verifying protocols through games is only possible when available behaviors are generated from a finite object; the most frequent underlying game model being \emph{games on graph}, where players navigate a finite graph, the choice of the edge being taken being given to the player owning the vertex.
\begin{defi}[Game on graph]\label{def:gameGraph}
    A \emph{game on graph} is a tuple $\Game=\left(\Pi,V,E,\left(\mu_i\right)_{i\in\Pi}\right)$ where:
    \begin{itemize}
        \item $\Pi$ is a set of players;
        \item $V = \biguplus_{i\in\Pi} V_i$ is the set of vertices, partitioned according to which player owns a given vertex;
        \item $E\subseteq V\times V$ is the set of edges, which is assumed to create no sink vertex: $\forall v\in V, \exists v'\in V, (v,v')\in E$;
        \item for each player $i$, the function $\mu_i:V^\omega\rightarrow\RR$ is the payoff function of player $i$.
    \end{itemize}
    A game is initialized by specifying an initial vertex $v_0\in V$.
    Game $\Game$ initialized in $v_0$ is denoted $\Game_{\|v_0}$.
\end{defi}
We sometimes abusively identify the set of players with $\{1,\dots,|\Pi|\}$ and write $\mu: V^\omega\rightarrow\RR^\Pi$ the payoff vector function defined by $\mu(\rho)=\left(\mu_1(\rho),\dots,\mu_{|\Pi|}(\rho)\right)$ for $\rho\in V^\omega$.

The strategies available for player $i$ is the set of functions $\sigma_i:V^*V_i\rightarrow V$ such that for any $w\in V^*$, $(v,\sigma_i(wv))\in E$.
From an initial vertex $v_0$, a strategy profile $\bsigma=\left(\sigma_1,\dots,\sigma_{|\Pi|}\right)$ (a strategy for each player) generates a single infinite path $\rho \in V^\omega$: $\rho=v_0v_1\cdots$ such that for every $j\in \NN$, if $v_j\in V_i$, then $v_{j+1} = \sigma_i(v_0\cdots v_j)$.
Path $\rho$, called the \emph{outcome} of profile $\bsigma$ and written $\rho=\outcome{\bsigma}$ defines the payoff vector: $\mu(\bsigma)=\mu(\outcome{\bsigma})$.
Hence an initialized game on graph is a particular case of a game.
\bigskip

\Le{On donne plus loin une définition qui colle au formalisme utilisé dans les preuves, peut-être supprimer celle-ci ?}

In turn, the protocol themselves ought to be provided in a finite way in order to be implementable by a program.
That corresponds to strategies with finite memory, which are usually provided by Mealy machines.
\begin{defi}[Mealy machine]\label{def:Mealy_game}
A \emph{Mealy machine} for game on graph $(V,E)$ is a tuple $\M=\left(S,T,s_0\right)$ where $S$ is a set of states, $T: S\times V \rightarrow 2^{E\times S}$ is the transition relation  such that $T(s,v)\subseteq \left\{((v,v'),s') \mmid (v,v')\in E, s'\in S\right\}\neq \emptyset$. \Ma{on est sûr que c'est ça qu'on veut ? ça a l'air de clasher avec la définition \ref{def:product_graph}}

A Mealy machine is deterministic if the image of $T$ is only made of singletons.\Ms{Do we use determninistic ones?}
% A \emph{deterministic Mealy machine} for game on graph $(V,E)$ is a tuple $\M=\left(S,T,s_0\right)$ where $S$ is a set of states, $T: S\times V \rightarrow E\times S$ is the transition function such that $T(s,v)=((v,v'),s')$ that gives from a given state and vertex an edge in the graph and a successor internal state.
% We write $T_1$ for the first component of $T$ (the \emph{output}) and $T_2$ for the second component (the \emph{update}).
\end{defi}
% A deterministic Mealy machine can be converted into a profile of strategies by setting the choice of the next vertex to be provided by the edge given as an output of the transition in the machine:
% $\bsigma(v_0\cdots v_n)=v'$ where $(v,v')=T_1(T_2(\cdots T_2(s_0,v_0),v_1)\cdots)$.
A Mealy machine can be converted into a set of strategy profiles: the choices available to players are only the ones corresponding to a path in the machine.
Namely a profile $\bsigma$ is generated by a machine $\M$ if the path $\rho=\outcome{\bsigma}=v_0 v_1 \cdots$ is such that there exists a path $s_0 s_1 \cdots$ in $\M$ where for every $i\in \NN$, $((v_{i},v_{i+1}),s_{i+1}) \in T(s_i,v_i)$.
\bigskip

It is possible to specify rectangular profiles of strategies by providing a separate Mealy machine per player: $M_1,\dots,\M_n$.
In that case the machine $\M_i\left(S_i,T_i,s_{0,i}\right)$ for player $i$ has a transition function that only specifies the next vertex if the current vertex belongs to $V_i$, and uses a special $\star$ symbol otherwise: $T_i: S_i\times V \rightarrow 2^{(E\uplus\star)\times S_i}$ is such that for $v\in V_i$, $T(s,v)\subseteq \left\{((v,v'),s') \mmid (v,v')\in E, s'\in S_i\right\}$ and for $v\in V\setminus V_i$, $T_i(s,v)\subseteq \left\{(\star,s') \mmid s'\in S_i\right\}$.
A Mealy machine for all players can then be computed as the synchronized product of the machines $M_1,\dots,\M_n$.
For every $v$, only a single machine has transitions with an actual edge (not $\star$), and this edge is used as the output edge of the product machine.
\Ms{L'information imparfaite peut intervenir ici de manière ad hoc, mais pas tellement de manière syntaxique car on n'a pas de modèle très clair de l'information détenue par chaque joueur: notre modèle est très général donc très flou de ce point de vue.}

% Furthermore, imperfect information can be modeled on these Mealy machines by using a projection $\pi_i: V \rightarrow Y_i$ where $Y_i$ is the set of vertices as seen by player $i$.
% Then the Mealy machine $\M_i$ gets elements of $Y_i$ as an input.

%\input{agentsnaturev1}
\input{agentsnaturev2}


==> version5formalism.tex <==
    \section{General formalisms}

        \subsection{Motivating example}\label{sec:motivatingExample}
        \input{motivatingExample}
        
        \subsection{Framework}
\Le{Version du formalisme avec un seul agent Infrastructure.}

We consider the following general scenario: several \emph{agents} (for instance: programs, or human users) interact through \emph{behaviors} (for instance: sending some message after having received some other), and aim to reach a \emph{correctness condition} (for instance, exchanging a cryptographic key, or signing a contract).
But, some (or all) of those agents are \emph{untrusted}: if they have the possibility, they may prefer an \emph{individual goal} in which they get a certain undue advantage (for instance: being able to read a message without having sent a delivery receipt, or buying an item without paying).
Some other untrusted agents may also be tempted to help that agent, as long as they avoid to be themselves \emph{wronged}.
Finally, there is also one specific agent: the Infrastructure, which has no individual goal but various possible behaviors.

In such a scenario, we wish to design, or to verify, \emph{protocols} that all those agents should follow, so that the correctness condition is achieved, and moreover no untrusted agent, or coalition of untrusted agents, can cheat other agents to reach their individual goal, whatever the Infrastructure does.



\begin{defi}[Protocol challenge]\label{def:protocolProblemNoInfrastructure}
    A \emph{protocol challenge} is a tuple:
    \[\pc = \left(\untrusted, (\behaviors_{u})_{u \in \untrusted}, \trusted, (\behaviors_{t})_{t \in \trusted}, \Traces, \tr, (\Ind_u)_{u \in \untrusted}, (\Wrong_u)_{u \in \untrusted}, \Corr\right),\] where:

    \begin{itemize}
    \item there are three types of \emph{agents}:
    \begin{itemize}
        \item the \emph{untrusted agents} are the elements of the set $\untrusted$,

        \item the \emph{trusted agents} are the elements of the set $\trusted$,

        \item the agent \emph{Infrastructure}, written $\II$, is neither trusted nor untrusted,
    \end{itemize}
    and we write $\agents = \untrusted \cup \trusted \cup \{\II\}$;

    \item each agent $a$ has a set $\behaviors_a\neq \emptyset$ of available \emph{behaviors} (and for $A \subseteq \agents$, we write $\behaviors_A = \prod_{a \in A} \behaviors_a$);

    \item the set $\Traces$ is the set of \emph{traces}, and the \emph{trace mapping} $\tr: \behaviors_\agents \rightarrow \Traces$ maps each tuple of behaviors to one trace;

    \item for each untrusted agent $u$, the sets $\Ind_u, \Wrong_u \subseteq \Traces$ are respectively the \emph{individual goal} and the \emph{wronging condition} of agent $u$, and they satisfy $\Ind_u \cap \Wrong_u = \emptyset$;

    \item the set $\Corr \in \Traces$ is called the \emph{correctness condition}, and is such that for each untrusted agent $u$, we have $\Corr \cap \Ind_u = \Corr \cap \Wrong_u = \emptyset$.
\end{itemize}
\end{defi}

\begin{defi}[Protocol, implementation]
    A \emph{protocol} is a nonempty set $P \subseteq \behaviors_\agents$.
    An \emph{implementation} of $P$ is an element $\bbeta$ of $P$.
    %The \emph{execution} of $\bbeta$ is the trace $\tau = \tr(\bbeta)$.
\end{defi}

\begin{exa} \label{ex:protocol}
In the example described in Section~\ref{sec:motivatingExample} and depicted in \figurename~\ref{fig:ongoingExampleWithTTPandInfra}, there are two untrusted agents, $\alice$ and $\bob$, one trusted agent $\ttp$, and the infrastructure $\II$.

The available behaviors for each agent are given by the choice, at any given moment\footnote{At this abstract level we are not too concerned about concurrency; a simple solution to avoid race condition is to assume each state is actually partitioned in $|\agents|$ and a round robin is performed between players who can \emph{pass} or act.}, to perform (or not) any of their own action whenever enabled.
The behaviors of $\II$ are further restricted by prohibiting behaviors that infinitely choose not to perform any action while infinitely enabled, to model the resilience of the channels.

For untrusted agents, Alice (or Bob) is wronged if she (he) remains indefinitely in a state where she has neither items, and achieves her individual goal if she indefinitely remains in a state where she has both items.
Regarding the correctness condition, it could consist simply in exchanging the items.
However, we choose here to add the condition that the exchange goes on without any intervention of the TTP, as such an intervention is in practice costly and should be used parsimoniously.

An example of a protocol is the set of behaviors defined as the product of the sets of following behaviors:
\begin{description}
    \item[For $\alice$:] Wait between 1 and 7 time units before sending $\textit{item}_1$. Then wait between 22 and 28 time units.
    If $\textit{item}_2$ has not been received by then, alert $\ttp$.
    \item[For $\bob$:] Wait between 3 and 12 time units before sending $\textit{item}_2$. Then wait between 20 and 30 time units.
    If $\textit{item}_1$ has not been received by then, alert $\ttp$.
    \item[For $\ttp$:] When alerted, immediately force the other party to send the item.
    \item[For $\II$:] Each received item is transmitted within 6 time units.
\end{description}
One can check that this allows the exchange to be fully performed, without any TTP intervention, in under 18 time units, so the correctness condition is achieved for any tuple of behaviors in this protocol.
Note that that is true only if the Infrastructure behaves as planned by the protocol: in practice, no one controls it, and an item delivery may last (much) more than 6 time units.
In such a case, the correctness condition is no longer guaranteed, because the TTP may be called; but that is acceptable in light of another requirement to protocols, the immunity against attacks, which must be guaranteed even if the Infrastructure helps the attacking agents.
\end{exa}


\begin{defi}[Attack, valid protocol]
    An \emph{attack} of the \emph{alliance} $A \subseteq \untrusted \cup \{\II\}$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists an implementation $\bbeta \in P$ such that, for each $a \in \agents \setminus A$, we have $\beta_a = \alpha_a$ (the agents that do not belong to $A$, are following the protocol $P$);
        
        \item there exists $u \in A\cap \untrusted$ such that $\tr(\balpha) \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in A\cap \untrusted$, we have $\tr(\balpha) \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    A protocol $P$ is \emph{valid} if:
    \begin{itemize}
        \item there is no attack to $P$,
        
        \item every implementation of $P$ satisfies the correctness condition: $\tr(P)\subseteq \Corr$.
    \end{itemize}
\end{defi}

Thus, modeling a concrete situation by a protocol challenge can be done by defining appropriate individual goals and wronging conditions, depending on the type of attacks one wants to avoid: the individual goals capture what a successful attack is, while the wronging conditions capture what can discourage an untrusted agent from helping another one.
A protocol is valid if it provides a description of behaviors that ensure the fulfillment of the correctness condition and are immune to attacks from untrusted agents.
%%%


\begin{exa}
    If we consider again the previous example, it appears that every implementation satisfies the correctness condition.
    Moreover, there is no attack to the protocol: the only ways for Alice to satisfy her individual objective are to be helped by the TTP, which is not possible, or by Bob; but then, Bob is wronged --- and symmetrically for Bob.

    On the other hand, consider again the protocol challenge given by Figure~\ref{fig:ongoingExampleTwoPlayers} (without the trusted third party).
    Then, there is no valid protocol in that case: if the correctness condition is satisfied, then either the alliance $\{\alice\}$, or the alliance $\{\bob\}$ has an attack, by refusing to send the item.
\end{exa}


        \subsection{Valid protocols as SNEs}

\begin{defi}[Game]\label{def:generalGame}
    A \emph{game} is a tuple $\Game = \left(\Pi, (\Sigma_i)_{i \in \Pi}, (\mu_i)_{i \in \Pi}\right)$, where:
    \begin{itemize}
        \item $\Pi$ is a set of \emph{players};

        \item for each player $i$, the set $\Sigma_i \neq \emptyset$ gathers the \emph{strategies} available for player $i$;

        \item for each player $i$, the function $\mu_i: \Sigma_\Pi \to \RR$ is the \emph{payoff function} of player $i$.
    \end{itemize}
\end{defi}

We now explain how such a protocol challenge $\pc$ can be captured by a game $\Game$.

The players in $\Game$ are the agents of $\pc$.
The strategies available for each player $i$ in $\Game$ are the behaviors available for agent $a$ in $\pc$.

The payoff functions of $\Game$ are defined as follows:

\begin{itemize}
    \item for $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \Wrong_u \\
        1 & \text{if } \tr(\bsigma) \not\in \Wrong_u \cup \Ind_u \\
        2 & \text{if } \tr(\bsigma) \in \Ind_u
    \end{cases};$$

    \item for $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \not\in \Corr \\
        1 & \text{if } \tr(\bsigma) \in \Corr
    \end{cases};$$

    \item for Infrastructure:
    $$\mu_\II: \bsigma \mapsto 1.$$
\end{itemize}

We assume that the protocol challenge contains at least one trusted and one untrusted agent --- if that is not the case, one can add a player with only one available strategy.


\begin{thm}\label{thm:linkSNEvalidNoInfrastructure}
    Let $P$ be a protocol in $\pc$.
    The protocol $P$ is valid if and only if for each $\bsigma \in P$ is a strong Nash equilibrium satisfying $\mu_a(\bsigma) = 1$ for every player $a$.
\end{thm}

\begin{proof}~
    \begin{itemize}
        \item \emph{If $P$ is valid.}
        
        Let $\bsigma \in P$.
        Since $\tr(\bsigma) \in \Corr$, we have $\mu_t(\bsigma) = 1$ for each $t \in \trusted$.
        For each $u \in \untrusted$, since $\Corr \cap \Ind_u = \Corr \cap \Wrong_u = \emptyset$ by definition of a protocol challenge, we have $\mu_u(\bsigma) = 1$.
        In the case of Infrastructure, we have $\mu_\II(\bsigma) = 1$ because it is the only possible payoff.

        Let us now prove that $\bsigma$ is an SNE.
        Let us assume that there exists a coalition $C \subseteq \agents$, that has a profitable deviation $\bsigma'_C$.
        Let $\balpha=(\bsigma_{-C},\bsigma_C')$: we will prove that $\balpha$ is an attack to $P$.
        Only untrusted agents can achieve payoff strictly higher than $1$.
        Therefore, we have:
        
        \begin{itemize}
            \item $\mu_a(\balpha) \geq 1$ for all $a \in C$;
            
            \item and there exists $u\in C\cap\untrusted$ such that $\mu_u(\balpha) = 2$, i.e. $\tr(\balpha) \in \Ind_u$.
        \end{itemize}

        Note that $\tr(\balpha) \in \Ind_u$ implies $\tr(\balpha) \not\in \Corr$, and therefore $\mu_t(\balpha) = 0$ for every $t \in \trusted$.
        Therefore, the coalition $C$ contains no trusted player.
        Consequently, in the strategy profile $\balpha$, all trusted agents and all the untrusted agents that are not in the coalition do follow $\bsigma$.
        Moreover, each agent of the alliance $C$ has the payoff at least $1$, i.e. is not wronged; and at least one satisfies their individual objective.

        So $\balpha$ is an attack of the alliance $C$ on $P$, which contradicts its validity.



        \item \emph{If every $\bsigma \in P$ is an SNE that yields payoff $1$ to every player.}

        Then, since $\trusted\neq\emptyset$, the trace $\tr(\bsigma)$ satisfies the correctness condition.
        As $\Corr$ is incompatible with any $\Ind_u$ and $\Wrong_u$, this implies that each player receives payoff $1$.

        Now, let us assume that there is an attack $\balpha$ of the alliance $A \subseteq \untrusted \cup \{\II\}$ on the protocol $P$.
        Let $\bsigma$ be an implementation of $P$ such that $\balpha_{\agents \setminus A} = \bsigma_{\agents \setminus A}$.
        By assumption, $\bsigma$ is an SNE that gives every player a payoff equal to $1$.
        Consider the coalition $A$: we will prove that $\balpha_A$ is a profitable deviation of $\bsigma_A$.
        For each untrusted agent $u \in A$, we have $\tr(\balpha) \notin \Wrong_u$, i.e. $\mu_u(\balpha) \geq 1$.
        Moreover, we always have $\mu_\II(\balpha) = 1$.
        Finally, there is an untrusted agent $u \in A$ such that $\tr(\balpha) \in \Ind_u$, i.e. $\mu_u(\balpha) = 2$.
       As a consequence, the strategy profile $\balpha_A$ is a profitable deviation of $\bsigma_A$, which is impossible since $\bsigma$ is an SNE: there is therefore no attack to $P$, which is a valid protocol.\qedhere
    \end{itemize}
\end{proof}



\begin{cor}
    A protocol challenge admits a valid protocol if and only if the corresponding game admits an SNE that gives every player the payoff $1$.
\end{cor}

\subsection{Finite models of protocols}

Modeling and verifying protocols through games is only possible when available behaviors are generated from a finite object; the most frequent underlying game model being \emph{games on graph}, where players navigate a finite graph, the choice of the edge being taken being given to the player owning the vertex.

\begin{defi}[Game on graph]\label{def:gameGraph}
    A \emph{game on graph} is a tuple $\Game=\left(\Pi,V,E,\left(\mu_i\right)_{i\in\Pi}\right)$ where:
    \begin{itemize}
        \item $\Pi$ is a set of players;
        \item $V = \biguplus_{i\in\Pi} V_i$ is the set of vertices, partitioned according to which player owns a given vertex;
        \item $E\subseteq V\times V$ is the set of edges, which is assumed to create no sink vertex: $\forall v\in V, \exists v'\in V, (v,v')\in E$;
        \item for each player $i$, the function $\mu_i:V^\omega\rightarrow\RR$ is the payoff function of player $i$.
    \end{itemize}
    A game is initialized by specifying an initial vertex $v_0\in V$.
    Game $\Game$ initialized in $v_0$ is denoted $\Game_{\|v_0}$.
\end{defi}
We sometimes abusively identify the set of players with $\{1,\dots,|\Pi|\}$ and write $\mu: V^\omega\rightarrow\RR^\Pi$ the payoff vector function defined by $\mu(\rho)=\left(\mu_1(\rho),\dots,\mu_{|\Pi|}(\rho)\right)$ for $\rho\in V^\omega$.

The strategies available for player $i$ is the set of functions $\sigma_i:V^*V_i\rightarrow V$ such that for any $w\in V^*$, $(v,\sigma_i(wv))\in E$.
From an initial vertex $v_0$, a strategy profile $\bsigma=\left(\sigma_1,\dots,\sigma_{|\Pi|}\right)$ (a strategy for each player) generates a single infinite path $\rho \in V^\omega$: $\rho=v_0v_1\cdots$ such that for every $j\in \NN$, if $v_j\in V_i$, then $v_{j+1} = \sigma_i(v_0\cdots v_j)$.
Path $\rho$, called the \emph{outcome} of profile $\bsigma$ and written $\rho=\outcome{\bsigma}$ defines the payoff vector: $\mu(\bsigma)=\mu(\outcome{\bsigma})$.
Hence an initialized game on graph is a particular case of a game.
\bigskip

% \Le{On donne plus loin une définition qui colle au formalisme utilisé dans les preuves, peut-être supprimer celle-ci ?}

% In turn, the protocol themselves ought to be provided in a finite way in order to be implementable by a program.
% That corresponds to strategies with finite memory, which are usually provided by Mealy machines.
% \begin{defi}[Mealy machine]\label{def:Mealy_game}
% A \emph{Mealy machine} for game on graph $(V,E)$ is a tuple $\M=\left(S,T,s_0\right)$ where $S$ is a set of states, $T: S\times V \rightarrow 2^{E\times S}$ is the transition relation  such that $T(s,v)\subseteq \left\{((v,v'),s') \mmid (v,v')\in E, s'\in S\right\}\neq \emptyset$. \Ma{on est sûr que c'est ça qu'on veut ? ça a l'air de clasher avec la définition \ref{def:product_graph}}

% A Mealy machine is deterministic if the image of $T$ is only made of singletons.\Ms{Do we use determninistic ones?}
% % A \emph{deterministic Mealy machine} for game on graph $(V,E)$ is a tuple $\M=\left(S,T,s_0\right)$ where $S$ is a set of states, $T: S\times V \rightarrow E\times S$ is the transition function such that $T(s,v)=((v,v'),s')$ that gives from a given state and vertex an edge in the graph and a successor internal state.
% % We write $T_1$ for the first component of $T$ (the \emph{output}) and $T_2$ for the second component (the \emph{update}).
% \end{defi}
% % A deterministic Mealy machine can be converted into a profile of strategies by setting the choice of the next vertex to be provided by the edge given as an output of the transition in the machine:
% % $\bsigma(v_0\cdots v_n)=v'$ where $(v,v')=T_1(T_2(\cdots T_2(s_0,v_0),v_1)\cdots)$.
% A Mealy machine can be converted into a set of strategy profiles: the choices available to players are only the ones corresponding to a path in the machine.
% Namely a profile $\bsigma$ is generated by a machine $\M$ if the path $\rho=\outcome{\bsigma}=v_0 v_1 \cdots$ is such that there exists a path $s_0 s_1 \cdots$ in $\M$ where for every $i\in \NN$, $((v_{i},v_{i+1}),s_{i+1}) \in T(s_i,v_i)$.
% \bigskip

% It is possible to specify rectangular profiles of strategies by providing a separate Mealy machine per player: $M_1,\dots,\M_n$.
% In that case the machine $\M_i\left(S_i,T_i,s_{0,i}\right)$ for player $i$ has a transition function that only specifies the next vertex if the current vertex belongs to $V_i$, and uses a special $\star$ symbol otherwise: $T_i: S_i\times V \rightarrow 2^{(E\uplus\star)\times S_i}$ is such that for $v\in V_i$, $T(s,v)\subseteq \left\{((v,v'),s') \mmid (v,v')\in E, s'\in S_i\right\}$ and for $v\in V\setminus V_i$, $T_i(s,v)\subseteq \left\{(\star,s') \mmid s'\in S_i\right\}$.
% A Mealy machine for all players can then be computed as the synchronized product of the machines $M_1,\dots,\M_n$.
% For every $v$, only a single machine has transitions with an actual edge (not $\star$), and this edge is used as the output edge of the product machine.
% \Ms{L'information imparfaite peut intervenir ici de manière ad hoc, mais pas tellement de manière syntaxique car on n'a pas de modèle très clair de l'information détenue par chaque joueur: notre modèle est très général donc très flou de ce point de vue.}

% Furthermore, imperfect information can be modeled on these Mealy machines by using a projection $\pi_i: V \rightarrow Y_i$ where $Y_i$ is the set of vertices as seen by player $i$.
% Then the Mealy machine $\M_i$ gets elements of $Y_i$ as an input.

%\input{agentsInfrastructurev1}
%\input{agentsInfrastructurev2}


\subsection{Compliance of the Infrastructure}

The proposed model relies on the assumption that agents (and in particular untrusted agents) are rational and therefore would always prefer to satisfy their individual objective and to avoid being wronged.
The case of Infrastructure is slightly different: Infrastructure may do anything, and to be valid, a protocol must realize the correctness condition for some of her behaviors (the ones planned by the protocol), but it must resist to attacks whatever she does.
Of course, those hypotheses can be relaxed by excluding some limit behaviors --- for example, it is a common assumption that (neutral) communication channels can delay messages for an arbitrary duration, but cannot drop a message altogether.
In the case of protocol challenges and games specified abstractly, this can be done explicitly: the set $\behaviors_\II$ does not contain those behaviors.
It is however more practical to reason on a finite model, such as games played on finite graphs (see Definition~\ref{def:gameGraph}).
In that case, some behaviors that are assumed to be impossible cannot be excluded by the game structure itself: they must be included in it, but the payoff function must be designed in a way that guarantees that they will never be used.
We label these behaviors as \emph{non-compliant}.

We therefore define a set $\Com \subseteq \Traces$ of \emph{compliant} traces, and we call \emph{compliant behavior} a behavior $\beta_\II$ such that $\tr(\beta_\II, \bbeta_{-\II})\in \Com$ for all $\bbeta_{-\II}$.
%We assume that every behavior participating in a compliant trace can be considered to be compliant: for every $\bbeta$ such that $\tr(\bbeta) \in \Com$, there exists $\bbeta_\untrusted'$ such that $\tr(\bbeta) = \tr(\bbeta_{-\untrusted},\bbeta_\untrusted')$.
%That ensures that compliance is always the result of one's own behavior and may not be influenced by other's behaviors.

The definition of what constitutes an attack on a protocol can therefore be updated as follows:
\begin{defi}[Attack, valid protocol (under compliance hypothesis)]~
\begin{itemize}
    \item 
    An \emph{attack under compliance hypothesis} of the \emph{alliance} $A \subseteq \untrusted \cup \{\II\}$ to the protocol $P$ is a tuple of behaviors $\balpha$, such that:
    \begin{itemize}
        \item there exists an implementation $\bbeta \in P$ such that, for each $a \in \agents \setminus A$, we have $\beta_a = \alpha_a$ (the trusted agents, and the untrusted ones that do not belong to $A$, are following the protocol $P$);
    
        \item we have $\tr(\balpha) \in \Com$ (the compliance hypothesis is satisfied);
    
        \item there exists $u \in A$ such that $\tr(\balpha) \in \Ind_u$ (at least one of the attacking agents achieves their individual goal);
    
        \item and for every $u' \in A$, we have $\tr(\balpha) \not\in \Wrong_{u'}$ (none of the attacking agents is wronged).
    \end{itemize}

    \item A protocol $P$ is \emph{valid under compliance hypothesis} if:
    \begin{itemize}
        \item all behaviors of Infrastructure are compliant,
        \item there is no attack to $P$ under compliance hypothesis,
        \item every implementation of $P$ satisfies the correctness condition.
    \end{itemize}
\end{itemize}
\end{defi}

\begin{exa}
    In our running example, consider the following deviation to our protocol: the Infrastructure delivers $\textit{item}_2$ to Alice, but keeps $\textit{item}_1$ forever.
    Then, Alice gets her individual goal satisfied (without even effectively deviate), and Bob is wronged: even when he calls the TTP, she cannot arrange the situation, since Alice has already sent $\textit{item}_1$.
    However, in such a scenario, the compliance hypothesis is no longer satisfied, hence it is not an attack under compliance hypothesis.
\end{exa}

\emph{Why is the Infrastructure not considered as an untrusted agent?}
Intuitively, it may seem a natural abstraction to consider that the Infrastructure is an agent who can join alliances, but who has no individual goal (or an empty one).
Then, one could define its wronging condition as the negation of its compliance hypothesis: the Infrastructure can then help any agent who tries to deviate from the protocol in order to satisfy his or her individual goal, as long as the compliance hypothesis is maintained.
However, the compliance hypothesis cannot fit such a formalism: the wronging condition is what an agent cannot \emph{accept} to help other agents, while non-compliance is what the Infrastructure cannot \emph{do}.
A protocol can perfectly be valid if, in a scenario in which some untrusted agent, say Bob, deviates, some other untrusted agent, say Alice, abandons her individual goal to prevent an attack.
There can also be scenarii in which Alice cannot avoid to be wronged.
In contrast, the Infrastructure must always guarantee her compliance hypothesis whatever the other agents do.

The addition of the compliance hypothesis does not hinder the conversion of the problem into a game.
The payoffs are defined as follows:
\begin{itemize}
    \item for $u\in\untrusted$ \emph{(untrusted players)}:
    $$\mu_u: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \Wrong_u \cap \Com \\
        1 & \text{if } \tr(\bsigma) \in \overline{\Wrong_u} \cap \overline{\Ind_u} \cap \Com \\
        2 & \text{if } \tr(\bsigma) \in \Ind_u \cup \overline{\Com}
    \end{cases};$$

    \item for $t\in\trusted$ \emph{(trusted players)}:
    $$\mu_t: \bsigma \mapsto \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \overline{\Corr}\cap \Com \\
        1 & \text{if } \tr(\bsigma) \in \Corr \cup \overline{\Com}
    \end{cases};$$

    \item for Infrastructure:
    $$\mu_\II: \begin{cases}
        0 & \text{if } \tr(\bsigma) \in \overline{\Com} \\
        1 & \text{if } \tr(\bsigma) \in \Com
    \end{cases}.$$
\end{itemize}
As we will see in the formal proof, the fact that when a trace is non-compliant, all other players get their maximal payoff will ensure that it is in the best interest of $\II$ to play according to a compliant strategy.

\begin{thm}\label{thm:linkSNEvalidWithSanity}
    Let $P$ be a protocol in $\pc$.
    The protocol $P$ is valid under compliance assumption if and only if each $\bsigma \in P$ is a strong Nash equilibrium satisfying $\mu_a(\bsigma) = 1$ for every player~$a$.
\end{thm}

\begin{proof}~
\begin{description}
    \item[\fbox{$\Rightarrow$}]
    Let $P$ be a valid protocol under compliance assumption.
    Let $\bsigma\in P$, and let us prove that $\bsigma$ is an SNE with all payoffs equal to $1$.
    Let $\tau=\tr(\<\bsigma\>)$. 
    First, because of the validity of $P$ we know the correctness condition is achieved so $\tau\in\Corr$; that implies that $\tau \notin \Ind_u$ and $\tau \notin \Wrong_u$ for each untrusted player $u$.
    Moreover, as all behaviors are compliant, we have $\tau \in \Com$.
    Therefore, we have $\mu_a(\bsigma)=1$ for every player $a$.

    Let us now assume that $\bsigma$ is not an SNE, i.e. there exists a profitable deviation for a coalition $C$ of players.
    For the deviation to be profitable, at least a player $a\in C$ must achieve a strictly better payoff while other players in the coalition are not decreasing their own.
    As trusted players cannot improve their payoff, they cannot strictly increase it, so an untrusted agent $u \in C \cap \untrusted$ must achieve a better payoff.
    That can be achieved in two ways:
    \begin{itemize}
        \item either because the compliance condition $\Com$ is violated.
        Since the behavior $\sigma_\II$ is compliant, that can only happen if Infrastructure deviated from it, i.e. if $\II \in C$.
        But that means its payoff is now $0$, and the deviation is not profitable.
        Hence this case can be excluded.
        
        \item The other possibility is that $u$ achieved his or her individual goal $\Ind_u$.
        In that case, the correctness condition is not achieved and so all trusted players get a payoff $0$, strictly less than with $\bsigma$, and therefore cannot be part of the coalition $C$.
        As a result $C \subseteq \untrusted \cup \{\II\}$.
        Moreover, all the players in $C$ get at least the payoff $1$, which means that in particular, no untrusted player in $C$ is wronged; and from the above, we know that $\tau$ satisfies the compliance condition.
        Such a deviation is therefore an attack to the protocol $P$, which contradicts its validity.
    \end{itemize}
    
    \item[\fbox{$\Leftarrow$}]~
    Assume all profiles in $P$ are SNEs with all payoffs to $1$.
    In particular, each produced trace must be in $\Com$, otherwise Infrastructure player would get payoff $0$.
    Moreover, every trusted player having payoff $1$ then means that the correctness condition is achieved.

    Assume by way of contradiction that $P$ is not valid.
    There are, then, three possibilities.

    \begin{itemize}
        \item First possibility: Infrastructure's behavior is non-compliant.
        Then, there is a deviation $\bsigma'_{-\II}$ of $\bsigma_{-\II}$ such that $(\sigma_\II, \bsigma'_{-\II}) \not\in \Com$.
        Then, in the strategy profile $(\sigma_\II, \bsigma'_{-\II})$, every trusted player gets the payoff $1$, and every untrusted player except $\II$ (there is at least one by hypothesis) gets the payoff $2$.
        Such a deviation is therefore profitable, which is impossible since $\bsigma$ is an SNE.
        
        \item Second possibility: there is an attack $\balpha$ of some alliance $A \subseteq \untrusted \cup \{\II\}$ on an implementation $\bbeta \in P$.
    The profile $\balpha_A$ is a deviation of $\bsigma_A$:
    \begin{itemize}
        \item the compliance hypothesis is statisfied, and therefore Infrastructure keeps the payoff $1$;
        \item a player $u \in A$ achieves $\Ind_u$, and therefore gets the payoff $2$;
        \item no untrusted player in $A$ is wronged, and therefore all of them get at least the payoff $1$.
    \end{itemize}
    This is therefore a profitable deviation for the coalition $A$, thus contradicting the fact that $\bbeta$ is an SNE.


        \item Third possibility: an implementation $\bsigma$ of $P$ does not satisfy the correctness condition.
        Then, if $t$ is a trusted player (there is at least one by hypothesis), we have $\mu_t(\bsigma) = 0$, which is impossible since every player is supposed to get the payoff $1$.
    \qedhere
    \end{itemize}
\end{description}
\end{proof}
